Optimizing the growth conditions of Al mirrors for superconducting nanowire single-photon detectors

We investigate the growth conditions for thin (less than 200 nm) sputtered aluminum (Al) films. These coatings are needed for various applications, e.g. for advanced manufacturing processes in the aerospace industry or for nanostructures for quantum devices. Obtaining high-quality films, with low roughness, requires precise optimization of the deposition process. To this end, we tune various sputtering parameters such as the deposition rate, temperature, and power, which enables 50 nm thin films with a root mean square (RMS) roughness of less than 1 nm and high reflectivity. Finally, we confirm the high quality of the deposited films by realizing superconducting single-photon detectors integrated into multi-layer heterostructures consisting of an aluminum mirror and a silicon dioxide dielectric spacer. We achieve an improvement in detection efficiency at 780 nm from 40 % to 70 % by this integration approach.

==> latexmkrc <==
## Sometimes when the references is very near the end of a page/column, latexmk fails to recognise when bibtex needs to be run. This rule forces bibtex to be run everytime.
$pdflatex = 'pdflatex --shell-escape %O %S; bibtex %R';



###############################
# Post processing of pdf file #
###############################

# assume the jobname is 'output' for Overleaf v2
my $ORIG_PDF_AGE = -M "output.pdf"; # get age of existing pdf if present

END {
    my $NEW_PDF_AGE = -M "output.pdf";
    return if !defined($NEW_PDF_AGE); # bail out if no pdf file
    return if defined($ORIG_PDF_AGE) && $NEW_PDF_AGE == $ORIG_PDF_AGE; # bail out if pdf was not updated
    my $QPDF = "/usr/bin/qpdf";
    return if ! -x $QPDF; # check that qpdf exists
    my $status = system($QPDF, "--linearize", "output.pdf", "output.pdf.opt");
    my $exitcode = ($status >> 8);
    print "qpdf exit code=$exitcode\n";
    # qpdf returns 0 for success, 3 for warnings (output pdf still created)
    return if !($exitcode == 0 || $exitcode == 3);
    print "Renaming optimised file to output.pdf\n";
    rename("output.pdf.opt", "output.pdf");
}

##############
# Glossaries #
##############
add_cus_dep( 'glo', 'gls', 0, 'glo2gls' );
add_cus_dep( 'acn', 'acr', 0, 'glo2gls');  # from Overleaf v1
sub glo2gls {
	system("makeglossaries $_[0]");
}

#############
# makeindex #
#############
@ist = glob("*.ist");
if (scalar(@ist) > 0) {
        $makeindex = "makeindex -s $ist[0] %O -o %D %S";
}

################
# nomenclature #
################
add_cus_dep("nlo", "nls", 0, "nlo2nls");
sub nlo2nls {
	system("makeindex $_[0].nlo -s nomencl.ist -o $_[0].nls -t $_[0].nlg");
}

#########
# Knitr #
#########
my $root_file = $ARGV[-1];

add_cus_dep( 'Rtex', 'tex', 0, 'rtex_to_tex');
sub rtex_to_tex {
    do_knitr("$_[0].Rtex");
}

sub do_knitr {
    my $dirname = dirname $_[0];
    my $basename = basename $_[0];
    system("Rscript -e \"library('knitr'); setwd('$dirname'); knit('$basename')\"");
}

my $rtex_file = $root_file =~ s/\.tex$/.Rtex/r;
unless (-e $root_file) {
	if (-e $rtex_file) {
		do_knitr($rtex_file);
	}
}

##########
# feynmf #
##########
push(@file_not_found, '^feynmf: Files .* and (.*) not found:$');
add_cus_dep("mf", "tfm", 0, "mf_to_tfm");
sub mf_to_tfm { system("mf '\\mode:=laserjet; input $_[0]'"); }

push(@file_not_found, '^feynmf: Label file (.*) not found:$');
add_cus_dep("mf", "t1", 0, "mf_to_label1");
sub mf_to_label1 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t1"); }
add_cus_dep("mf", "t2", 0, "mf_to_label2");
sub mf_to_label2 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t2"); }
add_cus_dep("mf", "t3", 0, "mf_to_label3");
sub mf_to_label3 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t3"); }
add_cus_dep("mf", "t4", 0, "mf_to_label4");
sub mf_to_label4 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t4"); }
add_cus_dep("mf", "t5", 0, "mf_to_label5");
sub mf_to_label5 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t5"); }
add_cus_dep("mf", "t6", 0, "mf_to_label6");
sub mf_to_label6 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t6"); }
add_cus_dep("mf", "t7", 0, "mf_to_label7");
sub mf_to_label7 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t7"); }
add_cus_dep("mf", "t8", 0, "mf_to_label8");
sub mf_to_label8 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t8"); }
add_cus_dep("mf", "t9", 0, "mf_to_label9");
sub mf_to_label9 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t9"); }

##########
# feynmp #
##########
push(@file_not_found, '^dvipdf: Could not find figure file (.*); continuing.$');
add_cus_dep("mp", "1", 0, "mp_to_eps");
sub mp_to_eps {
    system("mpost $_[0]");
    return 0;
}

#############
# asymptote #
#############
sub asy {return system("asy --offscreen '$_[0]'");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

#############
# metapost  #  # from Overleaf v1
#############
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
  my $file = $_[0];
  my ($name, $path) = fileparse($file);
  pushd($path);
  my $return = system "mpost $name";
  popd();
  return $return;
}

##########
# chktex #
##########
unlink 'output.chktex' if -f 'output.chktex';
if (defined $ENV{'CHKTEX_OPTIONS'}) {
    use File::Basename;
    use Cwd;

    # identify the main file
    my $target = $ARGV[-1];
    my $file = basename($target);

    if ($file =~ /\.tex$/) {
	# change directory for a limited scope
	my $orig_dir = cwd();
	my $subdir = dirname($target);
	chdir($subdir);
	# run chktex on main file
	$status = system(
    "/usr/bin/run-chktex.sh",
    $orig_dir,
    $file
  );
	# go back to original directory
	chdir($orig_dir);

	# in VALIDATE mode we always exit after running chktex
	# otherwise we exit if EXIT_ON_ERROR is set

	if ($ENV{'CHKTEX_EXIT_ON_ERROR'} || $ENV{'CHKTEX_VALIDATE'}) {
	    # chktex doesn't let us access the error info via exit status
	    # so look through the output
	    open(my $fh, "<", "output.chktex");
	    my $errors = 0;
	    {
		local $/ = "\n";
		while(<$fh>) {
		    if (/^\S+:\d+:\d+: Error:/) {
			$errors++;
			print;
		    }
		}
	    }
	    close($fh);
	    exit(1) if $errors > 0;
	    exit(0) if $ENV{'CHKTEX_VALIDATE'};
	}
    }
}

==> references-tex.tex <==
%% This BibTeX bibliography file was created using BibDesk.
%% https://bibdesk.sourceforge.io/

%% Created for Rasmus Flaschmann at 2022-03-17 20:44:11 +0100 


%% Saved with string encoding Unicode (UTF-8) 




@article{Abr57,
	title={On the magnetic properties of superconductors of the second group},
	author={Abrikosov, Alexei A},
	journal={Sov. Phys. JETP},
	volume={5},
	pages={1174--1182},
	year={1957}
}

@article{Akh12,
	title={Reduced dark counts in optimized geometries for superconducting nanowire single photon detectors},
	author={Akhlaghi, Mohsen K and Atikian, Haig and Eftekharian, Amin and Loncar, Marko and Majedi, A Hamed},
	journal={Optics express},
	volume={20},
	number={21},
	pages={23610--23616},
	year={2012},
	publisher={Optica Publishing Group}
}

@article{All19,
	title={Intrinsic timing jitter and latency in superconducting nanowire single-photon detectors},
	author={Allmaras, Jason P and Kozorezov, Alexander G and Korzh, Boris A and Berggren, Karl K and Shaw, Matthew D},
	journal={Physical Review Applied},
	volume={11},
	number={3},
	pages={034062},
	year={2019},
	publisher={APS}
}

@article{Bar62,
	title={Critical fields and currents in superconductors},
	author={Bardeen, John},
	journal={Reviews of modern physics},
	volume={34},
	number={4},
	pages={667},
	year={1962},
	publisher={APS}
}

@incollection{Bar16,
	title={Fluctuation mechanisms in superconductors},
	author={Bartolf, Holger},
	booktitle={Fluctuation Mechanisms in Superconductors},
	pages={181--184},
	year={2016},
	publisher={Springer}}

@article{Bec22,
	title={2023 roadmap for materials for quantum technologies},
	author={Becher, Christoph and Gao, Weibo and Kar, Swastik and Marciniak, Christian and Monz, Thomas and Bartholomew, John G and Goldner, Philippe and Loh, Huanqian and Marcellina, Elizabeth and Goh, Kuan Eng Johnson and others},
	journal={Materials for Quantum Technology},
	year={2022}}

@article{Ber71,
	title={Destruction of long-range order in one-dimensional and two-dimensional systems having a continuous symmetry group I. Classical systems},
	author={Berezinskii, VL314399},
	journal={Sov. Phys. JETP},
	volume={32},
	number={3},
	pages={493--500},
	year={1971}
}

@article{Bop22,
	title={Quantum dot molecule devices with optical control of charge status and electronic control of coupling},
	author={Bopp, Frederik and Rojas, Jonathan and Revenga, Natalia and Riedl, Hubert and Sbresny, Friedrich and Boos, Katarina and Simmet, Tobias and Ahmadi, Arash and Gershoni, David and Kasprzak, Jacek and others},
	journal={arXiv preprint arXiv:2205.10001},
	year={2022}
}

@article{Bor12,
	title={Deep-ultraviolet Raman investigation of silicon oxide: thin film on silicon substrate versus bulk material},
	author={Borowicz, Pawe{\l} and Latek, Mariusz and Rzodkiewicz, Witold and {\L}aszcz, Adam and Czerwinski, Andrzej and Ratajczak, Jacek},
	journal={Advances in Natural Sciences: Nanoscience and Nanotechnology},
	volume={3},
	number={4},
	pages={045003},
	year={2012},
	publisher={IOP Publishing}
}

@article{Bre20,
	title={Quantum dot single-photon emission coupled into single-mode fibers with 3D printed micro-objectives},
	author={Bremer, Lucas and Weber, Ksenia and Fischbach, Sarah and Thiele, Simon and Schmidt, Marco and Kaganskiy, Arsenty and Rodt, Sven and Herkommer, Alois and Sartison, Marc and Portalupi, Simone Luca and others},
	journal={APL Photonics},
	volume={5},
	number={10},
	pages={106101},
	year={2020},
	publisher={AIP Publishing LLC}
}

@article{Bul11,
	title={Vortex-induced dissipation in narrow current-biased thin-film superconducting strips},
	author={Bulaevskii, LN and Graf, MJ and Batista, CD and Kogan, VG},
	journal={Physical Review B},
	volume={83},
	number={14},
	pages={144526},
	year={2011},
	publisher={APS}
}

@article{Bur17,
	title = {Fiber-Coupled Diamond Quantum Nanophotonic Interface},
	author = {Burek, Michael J. and Meuwly, Charles and Evans, Ruffin E. and Bhaskar, Mihir K. and Sipahigil, Alp and Meesala, Srujan and Machielse, Bartholomeus and Sukachev, Denis D. and Nguyen, Christian T. and Pacheco, Jose L. and Bielejec, Edward and Lukin, Mikhail D. and Lon\ifmmode \check{c}\else \v{c}\fi{}ar, Marko},
	journal = {Phys. Rev. Applied},
	volume = {8},
	issue = {2},
	pages = {024026},
	numpages = {10},
	year = {2017},
	month = {Aug},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevApplied.8.024026},
	url = {https://link.aps.org/doi/10.1103/PhysRevApplied.8.024026}
}

@article{Cat22,
	title={Using materials for quasiparticle engineering},
	author={Catelani, Gianluigi and Pekola, Jukka P},
	journal={Materials for Quantum Technology},
	volume={2},
	number={1},
	pages={013001},
	year={2022},
	publisher={IOP Publishing}
}

@article{Cha75,
	title={Proximity effect in electron-beam lithography},
	author={Chang, THP},
	journal={Journal of vacuum science and technology},
	volume={12},
	number={6},
	pages={1271--1275},
	year={1975},
	publisher={American Vacuum Society}
}

@article{Cha91,
	title={Topography and microstructure of Al films formed under various deposition conditions},
	author={Chang, CY and Vook, RW},
	journal={Journal of Vacuum Science \& Technology A: Vacuum, Surfaces, and Films},
	volume={9},
	number={3},
	pages={559--562},
	year={1991},
	publisher={American Vacuum Society}
}

@book{Cha18,
	title={Improving the Spectral Bandwidth of Superconducting Nanowire Single-Photon Detectors (SNSPDs)},
	author={Charaev, Ilya},
	volume={20},
	year={2018},
	publisher={KIT Scientific Publishing}
}

@article{Cha19,
	title={Multimode-fiber-coupled superconducting nanowire single-photon detectors with high detection efficiency and time resolution},
	author={Chang, Jin and Zadeh, Iman Esmaeil and Los, Johannes WN and Zichi, Julien and Fognini, Andreas and Gevers, Monique and Dorenbos, Sander and Pereira, Silvania F and Urbach, Paul and Zwiller, Val},
	journal={Applied optics},
	volume={58},
	number={36},
	pages={9803--9807},
	year={2019},
	publisher={Optica Publishing Group}
}

@article{Che22,
	title={Unveiling photon statistics with a 100-pixel photon-number-resolving detector},
	author={Cheng, Risheng and Zhou, Yiyu and Wang, Sihao and Shen, Mohan and Taher, Towsif and Tang, Hong X},
	journal={arXiv preprint arXiv:2206.13753},
	year={2022}
}

@article{Chi18,
	author = {Xiaoming Chi and Kai Zou and Chao Gu and Julien Zichi and Yuhao Cheng and Nan Hu and Xiaojian Lan and Shufan Chen and Zuzeng Lin and Val Zwiller and Xiaolong Hu},
	journal = {Opt. Lett.},
	keywords = {Photon counting; Detectors; Quantum optics; Amorphous materials; Electron beam lithography; Multimode fibers; Single photon detectors; Thin films; Wire grid polarizers},
	number = {20},
	pages = {5017--5020},
	publisher = {Optica Publishing Group},
	title = {Fractal superconducting nanowire single-photon detectors with reduced polarization sensitivity},
	volume = {43},
	month = {Oct},
	year = {2018},
	url = {http://opg.optica.org/ol/abstract.cfm?URI=ol-43-20-5017},
	doi = {10.1364/OL.43.005017},
}

@article{Chi21,
	title={First constraints on dark photon dark matter with superconducting nanowire detectors in an optical haloscope},
	author={Chiles, Jeff and Charaev, Ilya and Lasenby, Robert and Baryakhtar, Masha and Huang, Junwu and Roshko, Alexana and Burton, George and Colangelo, Marco and Van Tilburg, Ken and Arvanitaki, Asimina and others},
	journal={arXiv preprint arXiv:2110.01582},
	year={2021}
}

@inproceedings{Chu12,
	title={Automated grain sizing using mark-based watershed algorithm},
	author={Chuang, Han-Sheng and Lin, Chao-Hung},
	booktitle={2012 IEEE International Geoscience and Remote Sensing Symposium},
	pages={2332--2335},
	year={2012},
	organization={IEEE}
}

@article{Cle11,
	title={Geometry-dependent critical currents in superconducting nanocircuits},
	author={Clem, John R and Berggren, Karl K},
	journal={Physical Review B},
	volume={84},
	number={17},
	pages={174510},
	year={2011},
	publisher={APS}
}

@article{Dau14,
	title={Review of superconducting nanowire single-photon detector system design options and demonstrated performance},
	author={Dauler, Eric A and Grein, Matthew E and Kerman, Andrew J and Marsili, Francesco and Miki, Shigehito and Nam, Sae Woo and Shaw, Matthew D and Terai, Hirotaka and Verma, Varun B and Yamashita, Taro},
	journal={Optical Engineering},
	volume={53},
	number={8},
	pages={081907},
	year={2014},
	publisher={SPIE}
}

@article{Dix09,
	title={Ultrashort dead time of photon-counting InGaAs avalanche photodiodes},
	author={Dixon, AR and Dynes, JF and Yuan, ZL and Sharpe, AW and Bennett, AJ and Shields, AJ},
	journal={Applied Physics Letters},
	volume={94},
	number={23},
	pages={231113},
	year={2009},
	publisher={American Institute of Physics}
}

@article{Dor08,
	title={Superconducting single photon detectors with minimized polarization dependence},
	author={Dorenbos, SN and Reiger, EM and Akopian, N and Perinetti, U and Zwiller, V and Zijlstra, T and Klapwijk, TM},
	journal={Applied Physics Letters},
	volume={93},
	number={16},
	pages={161102},
	year={2008},
	publisher={American Institute of Physics}
}

@article{Dub07,
	title={Nature of the superconductor--insulator transition in disordered superconductors},
	author={Dubi, Yonatan and Meir, Yigal and Avishai, Yshai},
	journal={Nature},
	volume={449},
	number={7164},
	pages={876--880},
	year={2007},
	publisher={Nature Publishing Group}
}

@article{Ein06,
	title={Zur theorie der brownschen bewegung},
	author={Einstein, Albert},
	journal={Annalen der physik},
	volume={324},
	number={2},
	pages={371--381},
	year={1906},
	publisher={WILEY-VCH Verlag Leipzig}
}

@article{Eng13,
	title={Temperature-dependence of detection efficiency in NbN and TaN SNSPD},
	author={Engel, Andreas and Inderbitzin, Kevin and Schilling, Andreas and Lusche, Robert and Semenov, Alexei and H{\"u}bers, Heinz-Wilhelm and Henrich, Dagmar and Hofherr, Matthias and Il'in, Konstantin and Siegel, Michael},
	journal={IEEE transactions on applied superconductivity},
	volume={23},
	number={3},
	pages={2300505--2300505},
	year={2013},
	publisher={IEEE}
}

@article{Eng14,
	title={Detection mechanism in SNSPD: numerical results of a conceptually simple, yet powerful detection model},
	author={Engel, Andreas and Lonsky, Julia and Zhang, Xiaofu and Schilling, Andreas},
	journal={IEEE Transactions on Applied Superconductivity},
	volume={25},
	number={3},
	pages={1--7},
	year={2014},
	publisher={IEEE}
}

@article{Eng15,
	title={Detection mechanism of superconducting nanowire single-photon detectors},
	author={Engel, Andreas and Renema, JJ and Il’in, Konstantin and Semenov, Alexander},
	journal={Superconductor Science and Technology},
	volume={28},
	number={11},
	pages={114003},
	year={2015},
	publisher={IOP Publishing}
}

@MastersThesis {Ern22,
	title={Optimization of the Structure and Current Flow of Superconducting Nanowire Single-Photon Detectors},
	author={Ernst, Sven Torsten},
	school={Technical University of Munich},
	year={2022}
}

@article{Ero18,
	title={Nano-optical photoresponse mapping of superconducting nanowires with enhanced near infrared absorption},
	author={Erotokritou, Kleanthis and Heath, Robert M and Taylor, Gregor G and Tian, Cheng and Banerjee, Archan and Casaburi, Alessandro and Natarajan, Chandra M and Miki, Shigehito and Terai, Hirotaka and Hadfield, Robert H},
	journal={Superconductor Science and Technology},
	volume={31},
	number={12},
	pages={125012},
	year={2018},
	publisher={IOP Publishing}
}

@article{Fer18,
	title={Waveguide-integrated superconducting nanowire single-photon detectors},
	author={Ferrari, Simone and Schuck, Carsten and Pernice, Wolfram},
	journal={Nanophotonics},
	volume={7},
	number={11},
	pages={1725--1758},
	year={2018},
	publisher={De Gruyter}
}

@MastersThesis {Fla18,
	title={Multi-Photon Interaction in Superconducting Nanowires: Two Approaches Towards Photon Number Resolution},
	author={Flaschmann, Rasmus},
	school={Technical University of Munich},
	year={2018}
}

@inproceedings{Fla22a,
	title={Automated, deep reactive ion etching free fiber coupling to nanophotonic devices},
	author={Flassig, Fabian and Flaschmann, Rasmus and Kainz, Thomas and Ernst, Sven and Strohauer, Stefan and Schmid, Christian and Zugliani, Lucio and M{\"u}ller, Kai and Finley, Jonathan J},
	booktitle={Quantum Sensing and Nano Electronics and Photonics XVIII},
	volume={12009},
	pages={102--110},
	year={2022},
	organization={SPIE}
}

@Article{Fla23a,
	title  ={The dependence of timing jitter of superconducting nanowire single-photon detectors on the multi-layer sample design and slew rate},
	author ={Flaschmann, Rasmus and Zugliani, Lucio and Schmid, Christian and Spedicato, Simone and Strohauer, Stefan and Wietschorke, Fabian and Flassig, Fabian and Finley, Jonathan J. and Müller, Kai},
	journal  ={Nanoscale},
	issue  ={3},
	volume  ={15},
	pages  ={1086--1091},
	year  ={2023},
	publisher  ={The Royal Society of Chemistry},
	doi  ={10.1039/D2NR04494C},
	url  ="{http://dx.doi.org/10.1039/D2NR04494C},
	abstract  ={We investigated the timing jitter of superconducting nanowire single-photon detectors (SNSPDs) and found a strong dependence on the detector response. By varying the multi-layer structure, we observed changes in pulse shape which are attributed to capacitive behaviour affecting the pulse heights, rise times and consequently timing jitter. Moreover, we developed a technique to predict the timing jitter of a single device within certain limits by capturing only a single detector pulse, eliminating the need for detailed jitter measurement using a pulsed laser when a rough estimate of the timing jitter is sufficient.}}

% once was Fla22c
@article{Fla23b,
	title={Optimizing the growth conditions of Al mirrors for superconducting nanowire single-photon detectors},
	author={Flaschmann, R and Schmid, C and Zugliani, L and Strohauer, and Finley, J and Müller, K},
	journal={Materials for Quantum Technologies},
	volume={123},
	number={123},
	pages={123},
	year={2023},
	publisher={IOP Publishing}
}

@misc{Fla23c,
	title={Oxydization barrier and improved detector design},
	author={Flaschmann, Rasmus, and Ernst, Sven and Zugliani, Lucio and Schmid, Christian and Strohauer, Stefan and Müller, Kai and Finley, Jonathan},
	year={2023},
	publisher={Google Patents},
	note={EPA Patent application 22 183 535.8},
	keywords={Oxydization barrier}
}

@article{Fra19,
	title={Determining the depairing current in superconducting nanowire single-photon detectors},
	author={Frasca, S and Korzh, B and Colangelo, M and Zhu, D and Lita, AE and Allmaras, JP and Wollman, EE and Verma, VB and Dane, AE and Ramirez, E and others},
	journal={Physical Review B},
	volume={100},
	number={5},
	pages={054520},
	year={2019},
	publisher={APS}
}


@article{Fuk11,
	author = {Fukuda, Daiji and Fujii, Go and Numata, Takayuki and Amemiya, Kuniaki and Yoshizawa, Akio and Tsuchida, Hidemi and Fujino, Hidetoshi and Ishii, Hiroyuki and Itatani, Taro and Inoue, Shuichiro and Zama, Tatsuya},
	year = {2011},
	title = {Titanium Superconducting Photon-Number-Resolving Detector},
	pages = {241--245},
	volume = {21},
	number = {3},
	issn = {1051-8223},
	journal = {IEEE Transactions on Applied Superconductivity},
	doi = {10.1109/TASC.2010.2089953}
}

@incollection{Gro18,
	title={Festk{\"o}rperphysik},
	author={Gross, Rudolf and Marx, Achim and Einzel, Dietrich and Gepr{\"a}gs, Stephan},
	booktitle={Festk{\"o}rperphysik},
	year={2018},
	publisher={de Gruyter}
}

@article{Gor59,
	title={Microscopic derivation of the Ginzburg-Landau equations in the theory of superconductivity},
	author={Gor’kov, Lev Petrovich},
	journal={Sov. Phys. JETP},
	volume={9},
	number={6},
	pages={1364--1367},
	year={1959}
}

@article{Gho01,
	title={Inhomogeneous pairing in highly disordered s-wave superconductors},
	author={Ghosal, Amit and Randeria, Mohit and Trivedi, Nandini},
	journal={Physical Review B},
	volume={65},
	number={1},
	pages={014501},
	year={2001},
	publisher={APS}
}

@article{Gin50,
	title={J. Exp. Theor. Phys.},
	author={Ginzburg, VL and Landau, LD and Leontovich, MA and Fok, VA},
	journal={JETP},
	volume={20},
	pages={1064},
	year={1950}
}

@article{Gol01,
	title={Fabrication and properties of an ultrafast NbN hot-electron single-photon detector},
	author={Gol'tsman, G and Okunev, O and Chulkova, G and Lipatov, A and Dzardanov, A and Smirnov, K and Semenov, A and Voronov, B and Williams, C and Sobolewski, Roman},
	journal={IEEE Transactions on applied superconductivity},
	volume={11},
	number={1},
	pages={574--577},
	year={2001},
	publisher={IEEE}
}

@article{Gol01b,
	title={Picosecond superconducting single-photon optical detector},
	author={Gol’Tsman, GN and Okunev, O and Chulkova, G and Lipatov, A and Semenov, A and Smirnov, K and Voronov, B and Dzardanov, A and Williams, C and Sobolewski, Roman},
	journal={Applied physics letters},
	volume={79},
	number={6},
	pages={705--707},
	year={2001},
	publisher={American Institute of Physics}
}

@book{Gra09,
	title={Analysis and design of analog integrated circuits},
	author={Gray, Paul R and Hurst, Paul J and Lewis, Stephen H and Meyer, Robert G},
	year={2009},
	publisher={John Wiley \& Sons},
	pages={40}
}

@MastersThesis {Gro22,
	title={Development of Amorphous Superconducting Thin Films for Near-Infrared Single-Photon Detection},
	author={Grotowski, Stefanie},
	school={Technical University of Munich},
	year={2022}
}

@article{Guo15,
	title={Single photon detector with high polarization sensitivity},
	author={Guo, Qi and Li, Hao and You, LiXing and Zhang, WeiJun and Zhang, Lu and Wang, Zhen and Xie, XiaoMing and Qi, Ming},
	journal={Scientific reports},
	volume={5},
	number={1},
	pages={1--5},
	year={2015},
	publisher={Nature Publishing Group}
}

@article{Guo16,
	title={Impact of trapezoidal cross section on polarization sensitivity of SNSPD with ultranarrow nanowire},
	author={Guo, Qi and You, Lixing and Li, Hao and Zhang, Weijun and Zhang, Lu and Liu, Xiaoyu and Yang, Xiaoyan and Chen, Sijing and Wang, Zhen and Xie, Xiaoming},
	journal={IEEE Transactions on Applied Superconductivity},
	volume={27},
	number={4},
	pages={1--4},
	year={2016},
	publisher={IEEE}
}

@misc{Gri05,
	title={Introduction to electrodynamics},
	author={Griffiths, David J},
	year={2005},
	publisher={American Association of Physics Teachers}
}

@article{Had05,
	title={Single photon source characterization with a superconducting single photon detector},
	author={Hadfield, Robert H and Stevens, Martin J and Gruber, Steven S and Miller, Aaron J and Schwall, Robert E and Mirin, Richard P and Nam, Sae Woo},
	journal={Optics Express},
	volume={13},
	number={26},
	pages={10846--10853},
	year={2005},
	publisher={Optical Society of America}
}

@article{Hag63,
	title={Right-angle bends in thin strip conductors},
	author={Hagedorn, Fred B and Hall, PM},
	journal={Journal of Applied Physics},
	volume={34},
	number={1},
	pages={128--133},
	year={1963},
	publisher={American Institute of Physics}
}

@article{Hao22,
	title={A superconducting nanowire photon number resolving four-quadrant detector-based Gigabit deep-space laser communication receiver prototype},
	author={Hao, Hao and Zhao, Qing-Yuan and Huang, Yang-Hui and Deng, Jie and Wang, Hui and Guo, Jia-Wei and Chen, Shi and Ru, Sai-Ying and Liu, Zhen and Zhou, Yi-Jin and others},
	journal={arXiv preprint arXiv:2212.04927},
	year={2022}
}

@article{Han18,
	title={Quantum dot single-photon sources with ultra-low multi-photon probability},
	author={Hanschke, Lukas and Fischer, Kevin A and Appel, Stefan and Lukin, Daniil and Wierzbowski, Jakob and Sun, Shuo and Trivedi, Rahul and Vu{\v{c}}kovi{\'c}, Jelena and Finley, Jonathan J and M{\"u}ller, Kai},
	journal={npj Quantum Information},
	volume={4},
	number={1},
	pages={1--6},
	year={2018},
	publisher={Nature Publishing Group}
}

@article{Hel64,
	title={Temperature and purity dependence of the superconducting critical field, Hc2},
	author={Helfand, E and Werthamer, NR},
	journal={Physical Review Letters},
	volume={13},
	number={23},
	pages={686},
	year={1964},
	publisher={APS}
}

@article{Hel66,
	title={Temperature and purity dependence of the superconducting critical field, Hc2. II},
	author={Helfand, E and Werthamer, NR},
	journal={Physical Review},
	volume={147},
	number={1},
	pages={288},
	year={1966},
	publisher={APS}
}

@article{Hen12,
	title={Geometry-induced reduction of the critical current in superconducting nanowires},
	author={Henrich, Dagmar and Reichensperger, P and Hofherr, M and Meckbach, JM and Il'in, Konstantin and Siegel, Michael and Semenov, A and Zotova, Anna and Vodolazov, D Yu},
	journal={Physical Review B},
	volume={86},
	number={14},
	pages={144504},
	year={2012},
	publisher={APS}
}

@article{Hof10a,
	author = {M. Hofherr AND D. Rall AND K. S. Ilin AND A. Semenov AND N. Gippius AND H.-W. Huebers AND M. Siegel},
	date-added = {2018-04-25 08:53:51 +0000},
	date-modified = {2018-05-19 06:20:37 +0000},
	journal = {Journal of Physics: Conference Series (SuST)},
	number = {012017},
	title = {Superconducting nanowire single-photon detectors: Quantum Efficiency vs. thickness of NbN films},
	volume = {234},
	year = {2010}}

@article{Hof10b,
	title={Intrinsic detection efficiency of superconducting nanowire single-photon detectors with different thicknesses},
	author={Hofherr, Mattias and Rall, Dagmar and Ilin, Konstantin and Siegel, Michael and Semenov, Alexej and H{\"u}bers, H-W and Gippius, NA},
	journal={Journal of Applied Physics},
	volume={108},
	number={1},
	pages={014507},
	year={2010},
	publisher={American Institute of Physics}
}

@book{Hor89,
	title={The art of electronics},
	author={Horowitz, Paul and Hill, Winfield},
	year={1989},
	volume={3},
	publisher={Cambridge: Cambridge university press},
	pages={408-410}
}

@article{Hum22,
	title={Nanosecond gating of superconducting nanowire single-photon detectors using cryogenic bias circuitry},
	author={Hummel, Thomas and Widhalm, Alex and H{\"O}pker, Jan Philipp and J{\"O}ns, Klaus D and Chang, Jin and Fognini, Andreas and Steinhauer, Stephan and Zwiller, Val and Zrenner, Artur and Bartley, Tim J},
	journal={arXiv preprint arXiv:2210.14841},
	year={2022}
}

@article{Ind12,
	title={An ultra-fast superconducting Nb nanowire single-photon detector for soft x-rays},
	author={Inderbitzin, Kevin and Engel, Andreas and Schilling, Andreas and Il'in, Konstantin and Siegel, Michael},
	journal={Applied Physics Letters},
	volume={101},
	number={16},
	pages={162601},
	year={2012},
	publisher={American Institute of Physics}
}

@article{Jah20,
	title={Probabilistic vortex crossing criterion for superconducting nanowire single-photon detectors},
	author={Jahani, Saman and Yang, Li-Ping and Buganza Tepole, Adri{\'a}n and Bardin, Joseph C and Tang, Hong X and Jacob, Zubin},
	journal={Journal of Applied Physics},
	volume={127},
	number={14},
	pages={143101},
	year={2020},
	publisher={AIP Publishing LLC}
}

@article{Jon22,
	title={Current crowding in nanoscale superconductors within the Ginzburg-Landau model},
	author={J{\"o}nsson, Mattias and Vedin, Robert and Gyger, Samuel and Sutton, James A and Steinhauer, Stephan and Zwiller, Val and Wallin, Mats and Lidmar, Jack},
	journal={Physical Review Applied},
	volume={17},
	number={6},
	pages={064046},
	year={2022},
	publisher={APS}
}

@article{Kao10,
	title={Nobel Lecture: Sand from centuries past: Send future voices fast},
	author={Kao, Charles K},
	journal={Reviews of Modern Physics},
	volume={82},
	number={3},
	pages={2299},
	year={2010},
	publisher={APS}
}

@inproceedings{Kao66,
	title={Dielectric-fibre surface waveguides for optical frequencies},
	author={Kao, K Charles and Hockham, George A},
	booktitle={Proceedings of the Institution of Electrical Engineers},
	volume={113},
	number={7},
	pages={1151--1158},
	year={1966},
	organization={IET}
}

@article{Khu22,
	title={Dispersive Spectrometry At Terahertz Frequencies for Probing the Quality of NbTiN Superconducting Films},
	author={Khudchenko, A and Lap, BNR and Rudakov, KI and Hesper, R and Koshelets, VP and Dmitriev, PN and Chekushkin, A and Khan, FV and Zhukova, ES and Kadyrov, LS and others},
	journal={IEEE Transactions on Applied Superconductivity},
	volume={32},
	number={4},
	pages={1--6},
	year={2022},
	publisher={IEEE}
}

@techreport{Kon21,
	author = {Konig, Julian and Flaschmann, Rasmus and Jiao, Yuqing and Müller, Kai},
	institution = {Eindhoven University of Technology},
	type= {Internship Report, },
	organization = {Eindhoven University of Technology and Technical University of Munich},
	title = {Detection efficiency optimization for superconducting nanowire single-photon detectors},
	number  = {Institute for Photonic Integration},
	year = {2021}}

@article{Koj99,
	title={XRR and XPS studies of SiO2 thin films formed by rf magnetron sputtering},
	author={Kojima, Isao and Li, Boquan and Fujimoto, Toshiyuki},
	journal={Surface and Interface Analysis: An International Journal devoted to the development and application of techniques for the analysis of surfaces, interfaces and thin films},
	volume={28},
	number={1},
	pages={267--270},
	year={1999},
	publisher={Wiley Online Library}
}

@conference{Kor18a,
	author = {B. Korzh AND Q.-Y. Zhao AND S. Frasca AND D. Zhu AND E. Ramirez AND E. Bersin AND M. Colnangelo AND A. Dane AND A. Beyer AND J. Allmaras AND E. Wollman AND K. Berggren AND M. Shaw},
	booktitle = {Conference on Lasers and Electro-Optics},
	date-added = {2018-06-01 00:29:05 +0000},
	date-modified = {2018-06-01 00:30:52 +0000},
	editor = {Optical Society of America},
	pages = {paper FW3F.3},
	title = {WSi superconducting nanowire single photon detector with a temporal resolution below 5 ps},
	year = {2018}}

@article{Kor18b,
	title={Decoherence-protected memory for a single-photon qubit},
	author={K{\"o}rber, Matthias and Morin, Olivier and Langenfeld, Stefan and Neuzner, Andreas and Ritter, Stephan and Rempe, Gerhard},
	journal={Nature Photonics},
	volume={12},
	number={1},
	pages={18--21},
	year={2018},
	publisher={Nature Publishing Group}
}

@article{Kor18c,
	title={Optical single-photon detection in micrometer-scale NbN bridges},
	author={Korneeva, Yu P and Vodolazov, D Yu and Semenov, AV and Florya, IN and Simonov, N and Baeva, E and Korneev, AA and Goltsman, GN and Klapwijk, TM},
	journal={Physical Review Applied},
	volume={9},
	number={6},
	pages={064037},
	year={2018},
	publisher={APS}
}

@article{Kos73,
	title={Ordering, metastability and phase transitions in two-dimensional systems},
	author={Kosterlitz, John Michael and Thouless, David James},
	journal={Journal of Physics C: Solid State Physics},
	volume={6},
	number={7},
	pages={1181},
	year={1973},
	publisher={IOP Publishing}
}

@article{Koz15,
	title={Quasiparticle recombination in hotspots in superconducting current-carrying nanowires},
	author={Kozorezov, AG and Lambert, Colin and Marsili, Francesco and Stevens, MJ and Verma, VB and Stern, Jeffrey A and Horansky, Rob and Dyer, Shellee and Duff, Shannon and Pappas, David P and others},
	journal={Physical Review B},
	volume={92},
	number={6},
	pages={064504},
	year={2015},
	publisher={APS}
}

@article{Koz17,
	title={Fano fluctuations in superconducting-nanowire single-photon detectors},
	author={Kozorezov, AG and Lambert, C and Marsili, F and Stevens, MJ and Verma, VB and Allmaras, JP and Shaw, MD and Mirin, RP and Nam, Sae Woo},
	journal={Physical Review B},
	volume={96},
	number={5},
	pages={054507},
	year={2017},
	publisher={APS}
}

@article{Kup80,
	title={Temperature dependence of pair-breaking current in superconductors},
	author={Kupryanov, M Yu and Lukichev, VF},
	journal={Sov. J. Low Temp. Phys.(Engl. Transl.);(United States)},
	volume={6},
	number={4},
	year={1980},
	publisher={Moscow Institute of Radio Engineering, Electronics, and Automation}
}

@article{Kup21,
	title={Evaluating a Stand-Alone Quantum-Dot Single-Photon Source for Quantum Key Distribution at Telecom Wavelengths},
	author={Kupko, Timm and Rickert, Lucas and Urban, Felix and Gro{\ss}e, Jan and Srocka, Nicole and Rodt, Sven and Musia{\l}, Anna and {\.Z}o{\l}nacz, Kinga and Mergo, Pawe{\l} and Dybka, Kamil and others},
	journal={arXiv preprint arXiv:2105.03473},
	year={2021}
}

@misc{Lae96,
	title={Method of anisotropically etching silicon},
	author={Laermer, Franz and Schilp, Andrea},
	year={1996},
	month=mar # "~26",
	publisher={Google Patents},
	note={US Patent 5,501,893},
	keywords={Bosch process}
}

@article{Lan80,
	title={Chapter i--the fundamental principles of statistical physics},
	author={Landau, LD and Lifshitz, EM},
	journal={Course of Theoretical Physics},
	pages={1--33},
	year={1980},
	publisher={Elsevier}
}

@article{LiB02,
	title={Surface evolution of ultrahigh vacuum magnetron sputter deposited amorphous SiO 2 thin films},
	author={Li, BQ and Kojima, I and Zuo, Jian-Min},
	journal={Journal of applied physics},
	volume={91},
	number={7},
	pages={4082--4089},
	year={2002},
	publisher={American Institute of Physics}
}

@article{LiH19,
	title={Multispectral superconducting nanowire single photon detector},
	author={Li, Hao and Wang, Heqing and You, Lixing and Hu, Peng and Shen, Weidong and Zhang, Weijun and Yang, Xiaoyan and Zhang, Lu and Zhou, Hui and Wang, Zhen and others},
	journal={Optics express},
	volume={27},
	number={4},
	pages={4727--4733},
	year={2019},
	publisher={Optica Publishing Group}
}

@article{Liz15,
	title={Roughness reduction of large-area high-quality thick Al films for echelle gratings by multi-step deposition method},
	author={Li, Zizheng and Gao, Jinsong and Yang, Haigui and Wang, Tongtong and Wang, Xiaoyi},
	journal={Optics express},
	volume={23},
	number={18},
	pages={23738--23747},
	year={2015},
	publisher={Optica Publishing Group}
}

@article{Lon35,
	title={The electromagnetic equations of the supraconductor},
	author={London, Fritz and London, Heinz},
	journal={Proceedings of the Royal Society of London. Series A-Mathematical and Physical Sciences},
	volume={149},
	number={866},
	pages={71--88},
	year={1935},
	publisher={The Royal Society London}
}

@article{Lop18,
	title={On the trends and application of pattern density dependent isofocal dose of positive resists for 100 keV electron beam lithography},
	author={Lopez, Gerald G and De Villafranca, Glen and Azadi, Mohsen and Metzler, Meredith G and Lister, Kevin and Labella, Michael and Eichfeld, Chad and Belic, Nikola and Hofmann, Ulrich},
	journal={Journal of Vacuum Science \& Technology B, Nanotechnology and Microelectronics: Materials, Processing, Measurement, and Phenomena},
	volume={36},
	number={6},
	pages={06JA05},
	year={2018},
	publisher={American Vacuum Society}
}

@article{Lus23,
	title={Large active-area superconducting microwire detector array with single-photon sensitivity in the near-infrared},
	author={Luskin, Jamie S and Schmidt, Ekkehart and Korzh, Boris and Beyer, Andrew D and Bumble, Bruce and Allmaras, Jason P and Walter, Alexander B and Wollman, Emma E and Narv{\'a}ez, Lautaro and Verma, Varun B and others},
	journal={arXiv preprint arXiv:2303.10739},
	year={2023}
}

@article{Ma22,
	title={Single photon detection performance of highly disordered NbTiN thin films},
	author={Ma, Ruoyan and Shu, Rui and Zhang, Xingyu and Yu, Aobo and Jia, Huang and Xiao, You and Yu, Huiqin and Liu, Xiaoyu and Li, Hao and Eklund, Per and others},
	journal={arXiv preprint arXiv:2210.15215},
	year={2022}
}

@article{Mak10,
	title={Characterization of NbTiN thin films deposited on various substrates},
	author={Makise, Kazumasa and Terai, Hirotaka and Takeda, Masanori and Uzawa, Yoshinori and Wang, Zhen},
	journal={IEEE transactions on applied superconductivity},
	volume={21},
	number={3},
	pages={139--142},
	year={2010},
	publisher={IEEE}
}

@article{Mat03,
	title={Characterization of NbTiN thin films prepared by reactive DC-magnetron sputtering},
	author={Matsunaga, Teruhiko and Maezawa, Hiroyuki and Noguchi, Takashi},
	journal={IEEE transactions on applied superconductivity},
	volume={13},
	number={2},
	pages={3284--3287},
	year={2003},
	publisher={IEEE}
}

@article{Mar09a,
	title={High quality superconducting NbN thin films on GaAs},
	author={Marsili, Francesco and Gaggero, Alessandro and Li, Lianhe H and Surrente, Alessandro and Leoni, Roberto and L{\'e}vy, Francis and Fiore, Andrea},
	journal={Superconductor Science and Technology},
	volume={22},
	number={9},
	pages={095013},
	year={2009},
	publisher={IOP Publishing}
}

@article{Mar09b,
	author = {M. Marksteiner AND A. Divochiy AND M. Sclafani AND P. Haslinger AND H. Ulbricht AND A. Korneev AND A. Semenov AND G. Goltsman AND M. Arndt},
	date-added = {2018-05-16 22:07:07 +0000},
	date-modified = {2018-05-16 22:07:40 +0000},
	journal = {Nanotechnology},
	title = {A superconducting NbN detector for neutral nanoparticles},
	volume = {20},
	year = {2009}}

@book{Mea13,
	title={Electrical resistance of metals},
	author={Meaden, George T},
	year={2013},
	publisher={Springer}
}

@article{Mei21,
	title={Optimization of quantum-dot qubit fabrication via machine learning},
	author={Mei, Antonio B and Milosavljevic, Ivan and Simpson, Amanda L and Smetanka, Valerie A and Feeney, Colin P and Seguin, Shay M and Ha, Sieu D and Ha, Wonill and Reed, Matthew D},
	journal={Applied Physics Letters},
	volume={118},
	number={20},
	pages={204001},
	year={2021},
	publisher={AIP Publishing LLC}
}

@article{Mei33,
	title={Ein neuer effekt bei eintritt der supraleitf{\"a}higkeit},
	author={Meissner, Walther and Ochsenfeld, Robert},
	journal={Naturwissenschaften},
	volume={21},
	number={44},
	pages={787--788},
	year={1933},
	publisher={Springer-Verlag}
}

@article{Men20,
	title={Fractal superconducting nanowires detect infrared single photons with 91\% polarization-independent system efficiency and 19 ps timing resolution},
	author={Meng, Yun and Zou, Kai and Hu, Nan and Xu, Liang and Lan, Xiaojian and Steinhauer, Stephan and Gyger, Samuel and Zwiller, Val and Hu, Xiaolong},
	journal={arXiv preprint arXiv:2012.06730},
	year={2020}
}

@article{Men22,
	title={Fractal superconducting nanowires detect infrared single photons with 84\% system detection efficiency, 1.02 polarization sensitivity, and 20.8 ps timing resolution},
	author={Meng, Yun and Zou, Kai and Hu, Nan and Xu, Liang and Lan, Xiaojian and Steinhauer, Stephan and Gyger, Samuel and Zwiller, Val and Hu, Xiaolong},
	journal={Acs Photonics},
	volume={9},
	number={5},
	pages={1547--1553},
	year={2022},
	publisher={ACS Publications}
}

@article{Mic15,
	title={The 100th anniversary of the four-point probe technique: the role of probe geometries in isotropic and anisotropic systems},
	author={Miccoli, Ilio and Edler, Frederik and Pfn{\"u}r, Herbert and Tegenkamp, Christoph},
	journal={Journal of Physics: Condensed Matter},
	volume={27},
	number={22},
	pages={223201},
	year={2015},
	publisher={IOP Publishing}
}

@article{Mor20,
	title={Precisely determining photon-number in real-time},
	author={Morais, Leonardo Assis and Weinhold, Till and de Almeida, Marcelo Pereira and Combes, Joshua and Lita, Adriana and Gerrits, Thomas and Nam, Sae Woo and White, Andrew G and Gillett, Geoff},
	journal={arXiv preprint arXiv:2012.10158},
	year={2020}
}

@article{Mue23,
	title={Time-walk and jitter correction in SNSPDs at high count rates},
	author={Mueller, Andrew and Wollman, Emma E and Korzh, Boris and Beyer, Andrew D and Narvaez, Lautaro and Rogalin, Ryan and Spiropulu, Maria and Shaw, Matthew D},
	journal={Applied Physics Letters},
	volume={122},
	number={4},
	pages={044001},
	year={2023},
	publisher={AIP Publishing LLC}
}

@article{Muk18,
	author = {Anna Mukhtarova and Luca Redaelli and Dibyendu Hazra and Houssaine Machhadani and St\'{e}phane Lequien and Max Hofheinz and Jean-Luc Thomassin and Frederic Gustavo and Julien Zichi and Val Zwiller and Eva Monroy and Jean-Michel G\'{e}rard},
	journal = {Opt. Express},
	keywords = {Infrared; Photodetectors; Absorption coefficient; Chemical vapor deposition; Quantum cryptography; Scanning electron microscopy; Single photon detectors; Thin films},
	number = {13},
	pages = {17697--17704},
	publisher = {Optica Publishing Group},
	title = {Polarization-insensitive fiber-coupled superconducting-nanowire single photon detector using a high-index dielectric capping layer},
	volume = {26},
	month = {Jun},
	year = {2018},
	url = {http://opg.optica.org/oe/abstract.cfm?URI=oe-26-13-17697},
	doi = {10.1364/OE.26.017697},
	abstract = {Superconducting-nanowire single photon detectors (SNSPDs) are able to reach near-unity detection efficiency in the infrared spectral range. However, due to the intrinsic asymmetry of nanowires, SNSPDs are usually very sensitive to the polarization of the incident radiation, their responsivity being maximum for light polarized parallel to the nanowire length (transverse-electric (TE) polarization). Here, we report on the reduction of the polarization sensitivity obtained by capping NbN-based SNSPDs with a high-index SiNx dielectric layer, which reduces the permittivity mismatch between the NbN wire and the surrounding area. Experimentally, a polarization sensitivity below 0.1 is obtained both at 1.31 and 1.55 \&\#x00B5;m, in excellent agreement with simulations.},
}

@article{Nic19,
	title={Universal model for the turn-on dynamics of superconducting nanowire single-photon detectors},
	author={Nicolich, Kathryn L and Cahall, Clinton and Islam, Nurul T and Lafyatis, Gregory P and Kim, Jungsang and Miller, Aaron J and Gauthier, Daniel J},
	journal={Physical Review Applied},
	volume={12},
	number={3},
	pages={034020},
	year={2019},
	publisher={APS}
}

@article{Nig88,
	title={Electrical resistivity of polycrystalline niobium nitride films},
	author={Nigro, A and Nobile, G and Rubino, MG and Vaglio, R},
	journal={Physical Review B},
	volume={37},
	number={8},
	pages={3970},
	year={1988},
	publisher={APS}
}

@book{Noj15,
	title={Dry etching technology for semiconductors},
	author={Nojiri, Kazuo},
	year={2015},
	publisher={Springer}
}

@article{Onn13,
	title={Investigations into the properties of substances at low temperatures, which have led, amongst other things, to the preparation of liquid helium},
	author={Onnes, Heike Kamerlingh},
	journal={Nobel lecture},
	volume={4},
	pages={306--336},
	year={1913}
}

@article{Per12b,
	title={Plasma etch characteristics of aluminum nitride mask layers grown by low-temperature plasma enhanced atomic layer deposition in SF6 based plasmas},
	author={Perros, Alexander and Bosund, Markus and Sajavaara, Timo and Laitinen, Mikko and Sainiemi, Lauri and Huhtio, Teppo and Lipsanen, Harri},
	journal={Journal of Vacuum Science \& Technology A: Vacuum, Surfaces, and Films},
	volume={30},
	number={1},
	pages={011504},
	year={2012},
	publisher={American Vacuum Society}
}

@article{Pfa14,
	title={Unconditional quantum teleportation between distant solid-state quantum bits},
	author={Pfaff, Wolfgang and Hensen, Bas J and Bernien, Hannes and van Dam, Suzanne B and Blok, Machiel S and Taminiau, Tim H and Tiggelman, Marijn J and Schouten, Raymond N and Markham, Matthew and Twitchen, Daniel J and others},
	journal={Science},
	volume={345},
	number={6196},
	pages={532--535},
	year={2014},
	publisher={American Association for the Advancement of Science}
}

@article{Pli21,
	title={Ultrahigh numerical aperture meta-fibre for flexible optical trapping},
	author={Plidschun, Malte and Ren, Haoran and Kim, Jisoo and F{\"o}rster, Ronny and Maier, Stefan A and Schmidt, Markus A},
	journal={Light: Science \& Applications},
	volume={10},
	number={1},
	pages={1--11},
	year={2021},
	publisher={Nature Publishing Group}
}

@Article{Pig14,
	author={Piggott, Alexander Y. and Lu, Jesse and Babinec, Thomas M. and Lagoudakis, Konstantinos G. and Petykiewicz, Jan and Vučković, Jelena},
	title={Inverse design and implementation of a wavelength demultiplexing grating coupler},
	journal={Scientific Reports},
	year={2014},
	month={Nov},
	day={27},
	volume={4},
	number={7210},
	abstract={Nanophotonics has emerged as a powerful tool for manipulating light on chips. Almost all of today's devices, however, have been designed using slow and ineffective brute-force search methods, leading in many cases to limited device performance. In this article, we provide a complete demonstration of our recently proposed inverse design technique, wherein the user specifies design constraints in the form of target fields rather than a dielectric constant profile and in particular we use this method to demonstrate a new demultiplexing grating. The novel grating, which has not been developed using conventional techniques, accepts a vertical-incident Gaussian beam from a free-space and separates O-band (1300 nm) and C-band (1550 nm) light into separate waveguides. This inverse design concept is simple and extendable to a broad class of highly compact devices including frequency filters, mode converters and spatial mode multiplexers.},
	issn={2045-2322},
	doi={10.1038/srep07210},
	url={https://doi.org/10.1038/srep07210}
}

@article{Qia04,
	title={Modeling electrical properties of gold films at infrared frequency using FDTD method},
	author={Qiang, Rui and Chen, Richard L and Chen, Ji},
	journal={International journal of infrared and millimeter waves},
	volume={25},
	number={8},
	pages={1263--1270},
	year={2004},
	publisher={Springer}
}

@inproceedings{Qui21,
	title={Influence of evaporation rate and chamber pressure on the FUV reflectance and physical characteristics of aluminum films},
	author={Quijada, Manuel A and Del Hoyo, Javier G and Gray, Emrold and Richardson, J Grabriel and Howe, Andrew and de Marcos, Luis Rodriguez and Sheikh, David A},
	booktitle={UV/Optical/IR Space Telescopes and Instruments: Innovative Technologies and Concepts X},
	volume={11819},
	pages={153--162},
	year={2021},
	organization={SPIE}
}

@article{Rec07,
	abstract = {This article reports a complete characterization of single photon avalanche diodes (SPADs) at temperatures down to 120 K. We show that deep cooling of the device by means of a compact liquid-nitrogen Dewar brings several advantages, such as extremely low dark counting rates (down to 1 counts/s), better time resolution, and higher quantum efficiency in the visible range. By using a special current pick-off circuit, we achieved a time resolution of 20 ps full width at half maximum at 120 K for a 50 mum diameter SPAD. Afterpulsing effects are avoided by using a sufficiently long hold-off time (microseconds).},
	author = {Rech, Ivan and Labanca, Ivan and Armellini, Giacomo and Gulinatti, Angelo and Ghioni, Massimo and Cova, Sergio},
	year = {2007},
	title = {Operation of silicon single photon avalanche diodes at cryogenic temperature},
	pages = {063105},
	volume = {78},
	number = {6},
	issn = {0034-6748},
	journal = {The Review of scientific instruments},
	doi = {10.1063/1.2743167},
	file = {Rech, Labanca et al. 2007 - Operation of silicon single photon:C\:\\Users\\christian.schmid\\Documents\\Citavi 6\\Projects\\Thesis\\Citavi Attachments\\Rech, Labanca et al. 2007 - Operation of silicon single photon.pdf:pdf}
}

@article{Red17,
	title={Design of polarization-insensitive superconducting single photon detectors with high-index dielectrics},
	author={Redaelli, Luca and Zwiller, Val and Monroy, E and G{\'e}rard, JM},
	journal={Superconductor Science and Technology},
	volume={30},
	number={3},
	pages={035005},
	year={2017},
	publisher={IOP Publishing}
}

@article{Red22,
	title={Broadband polarization insensitivity and high detection efficiency in high-fill-factor superconducting microwire single-photon detectors},
	author={Reddy, Dileep V and Otrooshi, Negar and Nam, Sae Woo and Mirin, Richard P and Verma, Varun B},
	journal={APL Photonics},
	volume={7},
	number={5},
	pages={051302},
	year={2022},
	publisher={AIP Publishing LLC}
}

@article{Rob86,
	title={The microstructure of aluminium thin films on amorphous SiO2},
	author={Roberts, S and Dobson, PJ},
	journal={Thin solid films},
	volume={135},
	number={1},
	pages={137--148},
	year={1986},
	publisher={Elsevier}
}

@article{Sav64,
	author = {Savitzky, Abraham. and Golay, M. J. E.},
	title = {Smoothing and Differentiation of Data by Simplified Least Squares Procedures.},
	journal = {Analytical Chemistry},
	volume = {36},
	number = {8},
	pages = {1627-1639},
	year = {1964},
	doi = {10.1021/ac60214a047},
	URL = {https://doi.org/10.1021/ac60214a047},
	eprint = {https://doi.org/10.1021/ac60214a047}
}

@article{Sav21,
	title={NV--diamond laser},
	author={Savvin, Alexander and Dormidonov, Alexander and Smetanina, Evgeniya and Mitrokhin, Vladimir and Lipatov, Evgeniy and Genin, Dmitriy and Potanin, Sergey and Yelisseyev, Alexander and Vins, Viktor},
	journal={Nature Communications},
	volume={12},
	number={1},
	pages={1--8},
	year={2021},
	publisher={Nature Publishing Group}
}

@article{Sbr22,
	title={Stimulated generation of indistinguishable single photons from a quantum ladder system},
	author={Sbresny, Friedrich and Hanschke, Lukas and Sch{\"o}ll, Eva and Rauhaus, William and Scaparra, Bianca and Boos, Katarina and Casalengua, Eduardo Zubizarreta and Riedl, Hubert and Del Valle, Elena and Finley, Jonathan J and others},
	journal={Physical Review Letters},
	volume={128},
	number={9},
	pages={093603},
	year={2022},
	publisher={APS}
}

@MastersThesis {Sch21a,
	title={Development of Highly Efficient Superconducting Single-Photon Detectors},
	author={Schmid, Christian},
	school={Technical University of Munich},
	year={2021}
}

@article{Sem01,
	title={Quantum detection by current carrying superconducting film},
	author={Semenov, Alex D and Gol’tsman, Gregory N and Korneev, Alexander A},
	journal={Physica C: Superconductivity},
	volume={351},
	number={4},
	pages={349--356},
	year={2001},
	publisher={Elsevier}
}

@article{Sem05,
	title={Spectral cut-off in the efficiency of the resistive state formation caused by absorption of a single-photon in current-carrying superconducting nano-strips},
	author={Semenov, Alexei and Engel, Andreas and H{\"u}bers, H-W and Il'in, Konstantin and Siegel, Michael},
	journal={The European Physical Journal B-Condensed Matter and Complex Systems},
	volume={47},
	number={4},
	pages={495--501},
	year={2005},
	publisher={Springer}
}

@article{Sen17,
	title={High-performance semiconductor quantum-dot single-photon sources},
	author={Senellart, Pascale and Solomon, Glenn and White, Andrew},
	journal={Nature nanotechnology},
	volume={12},
	number={11},
	pages={1026--1039},
	year={2017},
	publisher={Nature Publishing Group}
}

@article{Shi99,
	title={Differential pulse-position modulation for power-efficient optical communication},
	author={Shiu, Da-shan and Kahn, Joseph M},
	journal={IEEE transactions on communications},
	volume={47},
	number={8},
	pages={1201--1210},
	year={1999},
	publisher={IEEE}
}

@article{Sid21,
	title={Magnetoconductance and photoresponse properties of disordered NbTiN films},
	author={Sidorova, Mariia and Semenov, AD and H{\"u}bers, H-W and Gyger, Samuel and Steinhauer, Stephan and Zhang, X and Schilling, A},
	journal={Physical Review B},
	volume={104},
	number={18},
	pages={184514},
	year={2021},
	publisher={APS}
}

@inproceedings{Sin16,
	title={Evolution in quantum computing},
	author={Singh, Jasmeet and Singh, Mohit},
	booktitle={2016 International Conference System Modeling \& Advancement in Research Trends (SMART)},
	pages={267--270},
	year={2016},
	organization={IEEE}
}

@article{Smi16,
	title={Rise time of voltage pulses in NbN superconducting single photon detectors},
	author={Smirnov, KV and Divochiy, AV and Vakhtomin, Yu B and Sidorova, MV and Karpova, UV and Morozov, PV and Seleznev, VA and Zotova, AN and Vodolazov, D Yu},
	journal={Applied Physics Letters},
	volume={109},
	number={5},
	pages={052601},
	year={2016},
	publisher={AIP Publishing LLC}
}

@article{Smi58,
	title={Measurement of sheet resistivities with the four-point probe},
	author={Smits, FM},
	journal={Bell System Technical Journal},
	volume={37},
	number={3},
	pages={711--718},
	year={1958},
	publisher={Wiley Online Library}
}
@article{Smo06,
	title={Zur kinetischen theorie der brownschen molekularbewegung und der suspensionen},
	author={Von Smoluchowski, Marian},
	journal={Annalen der physik},
	volume={326},
	number={14},
	pages={756--780},
	year={1906},
	publisher={Wiley Online Library}
}

@MastersThesis {Spe22,
	title={Optimization of Superconducting Thin Films for Quantum Light Detection},
	author={Spedicato, Simone},
	school={Technical University of Munich},
	year={2022}
}

@article{Str23,
	title={Site-Selective Enhancement of Superconducting Nanowire Single-Photon Detectorsvia Local Helium Ion Irradiation},
	author={Strohauer, Stefan and Wietschorke, Fabian and Zugliani, Lucio and Flaschmann, Rasmus and Althammer, Matthias and Schmid, Christian and Grotowski, Stefanie and Gross, Rudolf and Müller, Kai and Finley Jonathan},
	journal={arXiv preprint arXiv:230x.xxxxx},
	year={2023}
}

@article{Ter22,
	title={Ultrafast quantum key distribution using fully parallelized quantum channels},
	author={Terhaar, Robin and R{\"o}diger, Jasper and H{\"a}u{\ss}ler, Matthias and Wahl, Michael and Gehring, Helge and Wolff, Martin A and Beutel, Fabian and Hartmann, Wladick and Walter, Nicolai and Hanke, Jonas and others},
	journal={arXiv preprint arXiv:2207.07345},
	year={2022}
}

@book{Val48,
	title={Vacuum tube amplifiers},
	author={Valley, George Edward and Wallman, Henry},
	year={1948},
	publisher={McGraw-Hill New York},
	pages={77-78}
}

@article{vdP58,
	title={A method of measuring specific resistivity and Hall effect of discs of arbitrary shape},
	author={Philips’Gloeilampenfabrieken, O},
	journal={Philips Res. Rep},
	volume={13},
	number={1},
	pages={1--9},
	year={1958}
}

@article{Ver86,
	title={Effects of water on the growth of aluminium films deposited by vacuum evaporation},
	author={Verkerk, MJ and Brankaert, WAMC},
	journal={Thin Solid Films},
	volume={139},
	number={1},
	pages={77--88},
	year={1986},
	publisher={Elsevier}
}

@article{Vig22,
	title={Probing quantum devices with radio-frequency reflectometry},
	author={Vigneau, Florian and Fedele, Federico and Chatterjee, Anasua and Reilly, David and Kuemmeth, Ferdinand and Gonzalez-Zalba, Fernando and Laird, Edward and Ares, Natalia},
	journal={arXiv preprint arXiv:2202.10516},
	year={2022}
}

@article{Vod17,
	title={Single-photon detection by a dirty current-carrying superconducting strip based on the kinetic-equation approach},
	author={Vodolazov, D Yu},
	journal={Physical Review Applied},
	volume={7},
	number={3},
	pages={034014},
	year={2017},
	publisher={APS}
}

@article{Vod19,
	title={Minimal timing jitter in superconducting nanowire single-photon detectors},
	author={Vodolazov, D Yu},
	journal={Physical Review Applied},
	volume={11},
	number={1},
	pages={014016},
	year={2019},
	publisher={APS}
}

@ARTICLE{Wan11,
	author={Wang, Qian and Loh, Ter-Hoe and Ng, Doris Keh Ting and Ho, Seng-Tiong},
	journal={IEEE Journal of Selected Topics in Quantum Electronics}, 
	title={Design and Analysis of Optical Coupling Between Silicon Nanophotonic Waveguide and Standard Single-Mode Fiber Using an Integrated Asymmetric Super-GRIN Lens}, 
	year={2011},
	volume={17},
	number={3},
	pages={581-589},
	doi={10.1109/JSTQE.2010.2075917}}

@article{Wan19,
	title={Wavelength dependence of intrinsic detection efficiency of NbN superconducting nanowire single-photon detector},
	author={Wang, Yong and Li, Hao and You, Li-Xing and Lv, Chao-Lin and Wang, He-Qing and Zhang, Xing-Yu and Zhang, Wei-Jun and Zhou, Hui and Zhang, Lu and Yang, Xiao-Yan and others},
	journal={Chinese Physics B},
	volume={28},
	number={7},
	pages={078502},
	year={2019},
	publisher={IOP Publishing}
}

@MastersThesis{Wie22,
	title={Controlling transport properties and detection efficiency of SSPDs via helium ion irradiation},
	author={Wietschorke, Fabian},
	school={Technical University of Munich},
	year={2022}
}

@article{Wol17,
	title={UV superconducting nanowire single-photon detectors with high efficiency, low noise, and 4 K operating temperature},
	author={Wollman, Emma E and Verma, Varun B and Beyer, Andrew D and Briggs, Ryan M and Korzh, B and Allmaras, Jason P and Marsili, F and Lita, Adriana E and Mirin, RP and Nam, SW and others},
	journal={Optics express},
	volume={25},
	number={22},
	pages={26792--26801},
	year={2017},
	publisher={Optica Publishing Group}
}

@article{Wol20,
	title={Superconducting nanowire single-photon detectors integrated with tantalum pentoxide waveguides},
	author={Wolff, Martin A and Vogel, Simon and Splitthoff, Lukas and Schuck, Carsten},
	journal={Scientific Reports},
	volume={10},
	number={1},
	pages={1--9},
	year={2020},
	publisher={Nature Publishing Group}
}

@article{Xia21,
	title={Short-wave infrared confocal fluorescence imaging of deep mouse brain with a superconducting nanowire single-photon detector},
	author={Xia, Fei and Gevers, Monique and Fognini, Andreas and Mok, Aaron T and Li, Bo and Akbari, Najva and Zadeh, Iman Esmaeil and Qin-Dregely, Jessie and Xu, Chris},
	journal={ACS Photonics},
	volume={8},
	number={9},
	pages={2800--2810},
	year={2021},
	publisher={ACS Publications}
}

@article{Xie21,
	title={The Applications of Ultra-Thin Nanofilm for Aerospace Advanced Manufacturing Technology},
	author={Xie, Guibai and Bai, Hongwu and Miao, Guanghui and Feng, Guobao and Yang, Jing and He, Yun and Li, Xiaojun and Li, Yun},
	journal={Nanomaterials},
	volume={11},
	number={12},
	pages={3282},
	year={2021},
	publisher={MDPI}
}

@article{Xin10,
	doi = {10.1088/1674-1056/19/8/086802},
	url = {https://doi.org/10.1088/1674-1056/19/8/086802},
	year = 2010,
	month = {aug},
	publisher = {{IOP} Publishing},
	volume = {19},
	number = {8},
	pages = {086802},
	author = {Zhang Xin and Song Xiao-Hui and Zhang Dian-Lin},
	title = {Thickness dependence of grain size and surface roughness for dc magnetron sputtered Au films},
	journal = {Chinese Physics B},
	abstract = {The grain size and surface morphology of sputtered Au films are studied by x-ray diffraction and atomic force microscope. For as-deposited samples the grain growth mechanism is consistent with the two-dimensional (2D) theory, which gives relatively low diffusion coefficient during deposition. The annealing process demonstrates the secondary grain growth mechanism in which the thickness dependence of grain boundary energy plays a key role. The surface roughness increases with the increase of grain size.}
}

@article{Xio22,
	title={Reducing current crowding in meander superconducting strip single-photon detectors by thickening bends},
	author={Xiong, Jia-Min and Zhang, Wei-Jun and Xu, Guang-Zhao and You, Li-Xing and Zhang, Xing-Yu and Zhang, Lu and Zhang, Cheng-Jun and Fan, Dong-Hui and Wang, Yu-Ze and Li, Hao and others},
	journal={Superconductor Science and Technology},
	volume={35},
	number={5},
	pages={055015},
	year={2022},
	publisher={IOP Publishing}
}

@article{XuY21,
	author = {Yilin Xu and Artem Kuzmin and Emanuel Knehr and Matthias Blaicher and Konstantin Ilin and Philipp-Immanuel Dietrich and Wolfgang Freude and Michael Siegel and Christian Koos},
	journal = {Optics Express},
	keywords = {Freeform lenses; Laser ranging; Quantum efficiency; Quantum key distribution; Total internal reflection; Variable optical attenuators},
	number = {17},
	pages = {27708--27731},
	publisher = {Optica Publishing Group},
	title = {Superconducting nanowire single-photon detector with 3D-printed free-form microlenses},
	volume = {29},
	month = {Aug},
	year = {2021},
	url = {http://opg.optica.org/oe/abstract.cfm?URI=oe-29-17-27708},
	doi = {10.1364/OE.427639},
	keywords = {Fiber coupling, 3D couplers},
	abstract = {We present an approach to increase the effective light-receiving area of superconducting nanowire single-photon detectors (SNSPD) by free-form microlenses. These lenses are printed in situ on top of the sensitive detector areas using high-resolution multi-photon lithography. We demonstrate a detector based on niobium-nitride (NbN) nanowires with a 4.5\&\#x2005;\&\#x00B5;m\&\#x2009;\&\#x00D7;\&\#x2009;4.5\&\#x2005;\&\#x00B5;m sensitive area, supplemented with a lens of 60-\&\#x00B5;m-diameter. For a plane-wave-like free-space illumination at a wavelength of 1550\&\#x2005;nm, the lensed sensor has a 100-fold increased effective collection area, which leads to a strongly enhanced system detection efficiency without the need for long nanowires. Our approach can be readily applied to a wide range of sensor types. It effectively overcomes the inherent design conflict between high count rate, high timing accuracy, and high fabrication yield on the one hand and high collection efficiency through a large effective detection area on the other hand.},
}

@article{XuG21,
	title={Superconducting microstrip single-photon detector with system detection efficiency over 90\% at 1550 nm},
	author={Xu, Guang-Zhao and Zhang, Wei-Jun and You, Li-Xing and Xiong, Jia-Min and Sun, Xing-Qu and Huang, Hao and Ou, Xin and Pan, Yi-Ming and Lv, Chao-Lin and Li, Hao and others},
	journal={Photonics Research},
	volume={9},
	number={6},
	pages={958--967},
	year={2021},
	publisher={Optica Publishing Group}
}


@article{Yu05,
	title={Fabrication of niobium titanium nitride thin films with high superconducting transition temperatures and short penetration lengths},
	author={Yu, Lei and Singh, RK and Liu, Hongxue and Wu, Stephen Y and Hu, Roger and Durand, D and Bulman, John and Rowell, John M and Newman, Nate},
	journal={IEEE transactions on applied superconductivity},
	volume={15},
	number={1},
	pages={44--48},
	year={2005},
	publisher={IEEE}
}

@article{Zha19,
	title={Saturating intrinsic detection efficiency of superconducting nanowire single-photon detectors via defect engineering},
	author={Zhang, Weijun and Jia, Qi and You, Lixing and Ou, Xin and Huang, Hao and Zhang, Lu and Li, Hao and Wang, Zhen and Xie, Xiaoming},
	journal={Physical Review Applied},
	volume={12},
	number={4},
	pages={044040},
	year={2019},
	publisher={APS}
}

@article{Zha22,
	title={Geometric origin of intrinsic dark counts in superconducting nanowire single-photon detectors},
	author={Zhang, Xingyu and Zhang, Xiaofu and Huang, Jia and Yang, Can and You, Lixing and Liu, Xiaoyu and Hu, Peng and Xiao, You and Zhang, Wenying and Wang, Yongliang and others},
	journal={Superconductivity},
	volume={1},
	pages={100006},
	year={2022},
	publisher={Elsevier}
}

@article{Zhu19,
	title={Superconducting nanowire single-photon detector with integrated impedance-matching taper},
	author={Zhu, Di and Colangelo, Marco and Korzh, Boris A and Zhao, Qing-Yuan and Frasca, Simone and Dane, Andrew E and Velasco, Angel E and Beyer, Andrew D and Allmaras, Jason P and Ramirez, Edward and others},
	journal={Applied Physics Letters},
	volume={114},
	number={4},
	pages={042601},
	year={2019},
	publisher={AIP Publishing LLC}
}

@article{Zol23,
	title={High-resistivity niobium nitride films for unity-efficiency SMSPDs at telecom wavelengths and beyond},
	author={Zolotov, Philipp and Svyatodukh, Sergey and Divochiy, Alexander and Seleznev, Vitaliy and Goltsman, Gregory},
	journal={arXiv preprint arXiv:2301.00400},
	year={2023}
}

@article{Zot14,
	title={Intrinsic detection efficiency of superconducting nanowire single photon detector in the modified hot spot model},
	author={Zotova, AN and Vodolazov, D Yu},
	journal={Superconductor Science and Technology},
	volume={27},
	number={12},
	pages={125001},
	year={2014},
	publisher={IOP Publishing}
}

@MastersThesis {Zug20,
	title={Superconducting Single Photon Detectors: Interplay between Geometry and Performance},
	author={Zugliani, Lucio},
	school={Technical University of Munich},
	year={2020}
}

@article{Ann10,
	title={Reset dynamics and latching in niobium superconducting nanowire single-photon detectors},
	author={Annunziata, Anthony J and Quaranta, Orlando and Santavicca, Daniel F and Casaburi, Alessandro and Frunzio, Luigi and Ejrnaes, Mikkel and Rooks, Michael J and Cristiano, Roberto and Pagano, Sergio and Frydman, Aviad and others},
	journal={Journal of Applied Physics},
	volume={108},
	number={8},
	pages={084507},
	year={2010},
	publisher={American Institute of Physics}
}

@article{Che17,
	title={Inhomogeneity-induced timing jitter of superconducting nanowire single-photon detectors},
	author={Cheng, Yuhao and Gu, Chao and Hu, Xiaolong},
	journal={Applied Physics Letters},
	volume={111},
	number={6},
	pages={062604},
	year={2017},
	publisher={AIP Publishing LLC}
}

@article{Bar10,
	title={Current-assisted thermally activated flux liberation in ultrathin nanopatterned NbN superconducting meander structures},
	author={Bartolf, Holger and Engel, Andreas and Schilling, Andreas and Il’in, Konstantin and Siegel, Michael and H{\"u}bers, H-W and Semenov, A},
	journal={Physical Review B},
	volume={81},
	number={2},
	pages={024502},
	year={2010},
	publisher={APS}
}

@article{Heo21,
	title={Procedure via cross-Kerr nonlinearities for encoding single logical qubit information onto four-photon decoherence-free states},
	author={Heo, Jino and Choi, Seong-Gon},
	journal={Scientific Reports},
	volume={11},
	number={1},
	pages={1--14},
	year={2021},
	publisher={Nature Publishing Group}
}


@article{Cha21b,
	title={Mid-infrared Single-photon Detection Using Superconducting NbTiN Nanowires with Sub-15 ps Time Resolution in a Gifford-McMahon Cryocooler},
	author={Chang, Jin and Los, Johannes WN and Gourgues, Ronan and Steinhauer, Stephan and Dorenbos, SN and Pereira, Silvania F and Urbach, H Paul and Zwiller, Val and Zadeh, Iman Esmaeil},
	journal={arXiv preprint arXiv:2107.06354},
	year={2021}
}

@article{San19,
	title={Jitter characterization of a dual-readout SNSPD},
	author={Santavicca, Daniel F and Noble, Brian and Kilgore, Cameron and Wurtz, Gregory A and Colangelo, Marco and Zhu, Di and Berggren, Karl K},
	journal={IEEE Transactions on Applied Superconductivity},
	volume={29},
	number={5},
	pages={1--4},
	year={2019},
	publisher={IEEE}
}


@article{Shi13,
	title={Superconducting nanowire single-photon detector with ultralow dark count rate using cold optical filters},
	author={Shibata, Hiroyuki and Shimizu, Kaoru and Takesue, Hiroki and Tokura, Yasuhiro},
	journal={Applied Physics Express},
	volume={6},
	number={7},
	pages={072801},
	year={2013},
	publisher={IOP Publishing}
}

@article{Vet16,
	title={Cavity-enhanced and ultrafast superconducting single-photon detectors},
	author={Vetter, Andreas and Ferrari, Simone and Rath, Patrik and Alaee, Rasoul and Kahl, Oliver and Kovalyuk, Vadim and Diewald, Silvia and Goltsman, Gregory N and Korneev, Alexander and Rockstuhl, Carsten and others},
	journal={Nano letters},
	volume={16},
	number={11},
	pages={7085--7092},
	year={2016},
	keywords={Dead time},
	publisher={ACS Publications}
}

@article{Cal16,
	title={Superconducting nanowire detector jitter limited by detector geometry},
	author={Calandri, Niccol{\`o} and Zhao, Qing-Yuan and Zhu, Di and Dane, Andrew and Berggren, Karl K},
	journal={Applied Physics Letters},
	volume={109},
	number={15},
	pages={152601},
	year={2016},
	keywords={Timing jitter},
	publisher={AIP Publishing LLC}
}

@article{Ste21,
	title={Progress on large-scale superconducting nanowire single-photon detectors},
	author={Steinhauer, Stephan and Gyger, Samuel and Zwiller, Val},
	journal={Applied Physics Letters},
	volume={118},
	number={10},
	pages={100501},
	year={2021},
	keywords={Large area SSPD},
	publisher={AIP Publishing LLC}
}

@article{You09,
	title={Shaping the response pulse of superconducting nanowire single photon detection with a snubber},
	author={You, LX and Shen, XF},
	journal={Applied Physics Letters},
	volume={95},
	number={15},
	pages={152514},
	year={2009},
	keywords={Dead time, snubber},
	publisher={American Institute of Physics}
}

@article{Sch13,
	title={Waveguide integrated low noise NbTiN nanowire single-photon detectors with milli-Hz dark count rate},
	author={Schuck, Carsten and Pernice, Wolfram HP and Tang, Hong X},
	journal={Scientific reports},
	volume={3},
	number={1},
	pages={1--6},
	year={2013},
	keywords={DCR, Waveguide integration},
	publisher={Nature Publishing Group}
}

@article{Zad20,
	title={A platform for high performance photon correlation measurements},
	author={Zadeh, Iman Esmaeil and Los, Johannes WN and Gourgues, Ronan and Chang, Jin and Elshaari, Ali W and Zichi, Julien and van Staaden, Yuri J and Swens, Jeroen and Kalhor, Nima and Guardiani, Antonio and others},
	journal={arXiv preprint arXiv:2003.09916},
	keywords={Timing jitter},
	year={2020}
}

@article{Kor20,
	title={Demonstration of sub-3 ps temporal resolution with a superconducting nanowire single-photon detector},
	author={Korzh, Boris and Zhao, Qing-Yuan and Allmaras, Jason P and Frasca, Simone and Autry, Travis M and Bersin, Eric A and Beyer, Andrew D and Briggs, Ryan M and Bumble, Bruce and Colangelo, Marco and others},
	journal={Nature Photonics},
	volume={14},
	number={4},
	pages={250--255},
	year={2020},
	keywords={Timing jitter},
	publisher={Nature Publishing Group}
}

@article{Yin20,
	title={Entanglement-based secure quantum cryptography over 1,120 kilometres},
	author={Yin, Juan and Li, Yu-Huai and Liao, Sheng-Kai and Yang, Meng and Cao, Yuan and Zhang, Liang and Ren, Ji-Gang and Cai, Wen-Qi and Liu, Wei-Yue and Li, Shuang-Lin and others},
	journal={Nature},
	volume={582},
	number={7813},
	pages={501--505},
	year={2020},
	keywords = {QKD},
	publisher={Nature Publishing Group}
}

@article{Kup20,
	title={Tools for the performance optimization of single-photon quantum key distribution},
	author={Kupko, Timm and von Helversen, Martin and Rickert, Lucas and Schulze, Jan-Hindrik and Strittmatter, Andr{\'e} and Gschrey, Manuel and Rodt, Sven and Reitzenstein, Stephan and Heindel, Tobias},
	journal={npj Quantum Information},
	volume={6},
	number={1},
	pages={1--8},
	year={2020},
	keywords = {QKD},
	publisher={Nature Publishing Group}
}

@article{Lee19,
	title={A fiber-integrated nanobeam single photon source emitting at telecom wavelengths},
	author={Lee, Chang-Min and Buyukkaya, Mustafa Atabey and Aghaeimeibodi, Shahriar and Karasahin, Aziz and Richardson, Christopher JK and Waks, Edo},
	journal={Applied Physics Letters},
	volume={114},
	number={17},
	pages={171101},
	year={2019},
	keywords = {Quantum dots},
	publisher={AIP Publishing LLC}
}

@article{Str10,
	title={Towards efficient quantum sources},
	author={Strauf, Stefan},
	journal={Nature Photonics},
	volume={4},
	number={3},
	pages={132--134},
	year={2010},
	keywords = {Quantum dots},
	publisher={Nature Publishing Group}
}

@article{Man19,
	title={Single-photon sources with quantum dots in III--V nanowires},
	author={M{\"a}ntynen, Henrik and Anttu, Nicklas and Sun, Zhipei and Lipsanen, Harri},
	journal={Nanophotonics},
	volume={8},
	number={5},
	pages={747--769},
	year={2019},
	keywords = {Quantum dots},
	publisher={De Gruyter}
}

@article{Rei15,
	author = {Reithmaier, G and Kaniber, M and Flassig, F and Lichtmannecker, S and M{\"u}ller, K and Andrejew, A and Vuckovic, J and Gross, R and Finley, JJ},
	journal = {Nano letters},
	keywords = {Team SSPD},
	number = {8},
	pages = {5208--5213},
	publisher = {ACS Publications},
	title = {On-chip generation, routing, and detection of resonance fluorescence},
	volume = {15},
	year = {2015}}

@article{Rei13a,
	author = {Reithmaier, G{\"u}nther and Lichtmannecker, Stefan and Reichert, Thorsten and Hasch, Peter and M{\"u}ller, Kai and Bichler, Max and Gross, Rudolf and Finley, Jonathan J},
	journal = {Scientific reports},
	keywords = {Team SSPD},
	number = {1},
	pages = {1--6},
	publisher = {Nature Publishing Group},
	title = {On-chip time resolved detection of quantum dot emission using integrated superconducting single photon detectors},
	volume = {3},
	year = {2013}}

@article{Cha21a,
	author = {Chang, J and Los, JWN and Tenorio-Pearl, JO and Noordzij, N and Gourgues, R and Guardiani, A and , JR and Pereira, SF and Urbach, HP and Zwiller, Val and others},
	journal = {APL Photonics},
	keywords = {NbTiN},
	number = {3},
	pages = {036114},
	publisher = {AIP Publishing LLC},
	title = {Detecting telecom single photons with 99.5- 2.07+ 0.5\% system detection efficiency and high time resolution},
	volume = {6},
	year = {2021}}

@article{Hu20,
	author = {Hu, Peng and Li, Hao and You, Lixing and Wang, Heqing and Xiao, You and Huang, Jia and Yang, Xiaoyan and Zhang, Weijun and Wang, Zhen and Xie, Xiaoming},
	journal = {Optics Express},
	keywords = {NbN},
	number = {24},
	pages = {36884--36891},
	publisher = {Optical Society of America},
	title = {Detecting single infrared photons toward optimal system detection efficiency},
	volume = {28},
	year = {2020}}

@article{Zha17,
	title={NbN superconducting nanowire single photon detector with efficiency over 90\% at 1550 nm wavelength operational at compact cryocooler temperature},
	author={Zhang, WeiJun and You, LiXing and Li, Hao and Huang, Jia and Lv, ChaoLin and Zhang, Lu and Liu, XiaoYu and Wu, JunJie and Wang, Zhen and Xie, XiaoMing},
	journal={Science China Physics, Mechanics \& Astronomy},
	volume={60},
	number={12},
	pages={1--10},
	year={2017},
	keywords = {NbN},
	publisher={Springer}
}

@article{Red20,
	author = {Reddy, Dileep V and Nerem, Robert R and Nam, Sae Woo and Mirin, Richard P and Verma, Varun B},
	journal = {Optica},
	keywords = {MoSi},
	number = {12},
	pages = {1649--1653},
	publisher = {Optical Society of America},
	title = {Superconducting nanowire single-photon detectors with 98\% system detection efficiency at 1550 nm},
	volume = {7},
	year = {2020}}

@article{Mik13,
	title={High performance fiber-coupled NbTiN superconducting nanowire single photon detectors with Gifford-McMahon cryocooler},
	author={Miki, Shigehito and Yamashita, Taro and Terai, Hirotaka and Wang, Zhen},
	journal={Optics express},
	volume={21},
	number={8},
	pages={10208--10214},
	year={2013},
	keywords = {SSPD, Fiber coupling},
	publisher={Optical Society of America}
}

@article{Zad21,
	author = {Zadeh, Esmaeil and Chang, J and Los, Johannes WN and Gyger, Samuel and Elshaari, Ali W and Steinhauer, Stephan and Dorenbos, Sander N and Zwiller, Val},
	journal = {Applied Physics Letters},
	keywords = {SSPD},
	number = {19},
	pages = {190502},
	publisher = {AIP Publishing LLC},
	title = {Superconducting nanowire single-photon detectors: A perspective on evolution, state-of-the-art, future developments, and applications},
	volume = {118},
	year = {2021}}

@article{Hol19,
	author = {Holzman, Itamar and Ivry, Yachin},
	journal = {Advanced Quantum Technologies},
	keywords = {SSPD},
	number = {3-4},
	pages = {1800058},
	publisher = {Wiley Online Library},
	title = {Superconducting nanowires for single-photon detection: progress, challenges, and opportunities},
	volume = {2},
	year = {2019}}

@article{Red16,
	author = {Redaelli, Luca and Bulgarini, Gabriele and Dobrovolskiy, Sergiy and Dorenbos, Sander N and Zwiller, Vall and Monroy, Eva and G{\'e}rard, Jean-Michel},
	journal = {Superconductor Science and Technology},
	keywords = {SSPD},
	number = {6},
	pages = {065016},
	publisher = {IOP Publishing},
	title = {Design of broadband high-efficiency superconducting-nanowire single photon detectors},
	volume = {29},
	year = {2016}}

@article{Mil11,
	author = {Miller, Aaron J and Lita, Adriana E and Calkins, Brice and Vayshenker, Igor and Gruber, Steven M and Nam, Sae Woo},
	journal = {Optics express},
	keywords = {SSPD},
	number = {10},
	pages = {9102--9110},
	publisher = {Optical Society of America},
	title = {Compact cryogenic self-aligning fiber-to-detector coupling with losses below one percent},
	volume = {19},
	year = {2011}
}

@article{Sch21,
	title={Bright Electrically Controllable Quantum-Dot-Molecule Devices Fabricated by In Situ Electron-Beam Lithography},
	author={Schall, Johannes and Deconinck, Marielle and Bart, Nikolai and Florian, Matthias and von Helversen, Martin and Dangel, Christian and Schmidt, Ronny and Bremer, Lucas and Bopp, Frederik and H{\"u}llen, Isabell and others},
	journal={Advanced Quantum Technologies},
	volume={4},
	number={6},
	pages={2100002},
	year={2021},
	keywords = {Quantum dot molecules},
	publisher={Wiley Online Library}
}

@article{Mik10,
	title={Multichannel SNSPD system with high detection efficiency at telecommunication wavelength},
	author={Miki, Shigehito and Yamashita, Taro and Fujiwara, Mikio and Sasaki, Masahide and Wang, Zhen},
	journal={Optics letters},
	volume={35},
	number={13},
	pages={2133--2135},
	year={2010},
	keywords = {Fiber coupling, SSPD, GRIN},
	publisher={Optical Society of America}
}

@article{Wan10,
	title={Design and analysis of optical coupling between silicon nanophotonic waveguide and standard single-mode fiber using an integrated asymmetric super-GRIN lens},
	author={Wang, Qian and Loh, Ter-Hoe and Ng, Doris Keh Ting and Ho, Seng-Tiong},
	journal={IEEE Journal of Selected Topics in Quantum Electronics},
	volume={17},
	number={3},
	pages={581--589},
	year={2010},
	keywords = {Fiber coupling, SSPD, GRIN},
	publisher={IEEE}
}

@article{Bar15,
	title={Review of devices, packaging, and materials for cryogenic optoelectronics},
	author={Bardalen, Eivind and Akram, Muhammad Nadeem and Malmbekk, Helge and Ohlckers, Per},
	journal={Journal of Microelectronics and Electronic Packaging},
	volume={12},
	number={4},
	pages={189--204},
	year={2015},
	keywords = {Fiber coupling},
	publisher={International Microelectronics Assembly and Packaging Society Collection}
}

@article{Tie15,
	title={Efficient fiber-optical interface for nanophotonic devices},
	author={Tiecke, TG and Nayak, KP and Thompson, Jeffrey Douglas and Peyronel, T and de Leon, Nathalie P and Vuleti{\'c}, V and Lukin, MD},
	journal={Optica},
	volume={2},
	number={2},
	pages={70--75},
	year={2015},
		keywords = {Fiber coupling},
	publisher={Optical Society of America}
}

@article{And42,
	title={Attenuated superconductors I. For measuring infra-red radiation},
	author={Andrews, Donald H and Brucksch Jr, WF and Ziegler, WT and Blanchard, ER},
	journal={Review of Scientific Instruments},
	volume={13},
	number={7},
	pages={281--292},
	year={1942},
	keywords = {TES},
	publisher={American Institute of Physics}}

@article{Lit08,
	title={Counting near-infrared single-photons with 95\% efficiency},
	author={Lita, Adriana E and Miller, Aaron J and Nam, Sae Woo},
	journal={Optics express},
	volume={16},
	number={5},
	pages={3032--3040},
	year={2008},
	keywords = {TES},
	publisher={Optical Society of America}
}

@article{Ull15,
	author = {Ullom, Joel N and Bennett, Douglas A},
	journal = {Superconductor Science and Technology},
	keywords = {TES},
	number = {8},
	pages = {084003},
	publisher = {IOP Publishing},
	title = {Review of superconducting transition-edge sensors for x-ray and gamma-ray spectroscopy},
	volume = {28},
	year = {2015}}

@article{Tra16,
	author = {Tran, Toan Trong and Elbadawi, Christopher and Totonjian, Daniel and Lobo, Charlene J and Grosso, Gabriele and Moon, Hyowon and Englund, Dirk R and Ford, Michael J and Aharonovich, Igor and Toth, Milos},
	journal = {ACS nano},
	keywords = {2D materials},
	number = {8},
	pages = {7331--7338},
	publisher = {ACS Publications},
	title = {Robust multicolor single photon emission from point defects in hexagonal boron nitride},
	volume = {10},
	year = {2016}}

@article{Lie14,
	title={Tapered fiber coupling of single photons emitted by a deterministically positioned single nitrogen vacancy center},
	author={Liebermeister, Lars and Petersen, Fabian and M{\"u}nchow, Asmus v and Burchardt, Daniel and Hermelbracht, Juliane and Tashima, Toshiyuki and Schell, Andreas W and Benson, Oliver and Meinhardt, Thomas and Krueger, Anke and others},
	journal={Applied Physics Letters},
	volume={104},
	number={3},
	pages={031101},
	year={2014},
	keywords = {NV-centers},
	publisher={American Institute of Physics}
}

@article{Kur00,
	author = {Kurtsiefer, Christian and Mayer, Sonja and Zarda, Patrick and Weinfurter, Harald},
	journal = {Physical review letters},
	keywords = {NV-centers},
	number = {2},
	pages = {290},
	publisher = {APS},
	title = {Stable solid-state source of single photons},
	volume = {85},
	year = {2000}}

@article{Fry00,
	author = {Fry, PW and Finley, JJ and Wilson, LR and Lemaitre, A and Mowbray, DJ and Skolnick, MS and Hopkinson, M and Hill, G and Clark, JC},
	journal = {Applied Physics Letters},
	keywords = {Quantum dot},
	number = {26},
	pages = {4344--4346},
	publisher = {American Institute of Physics},
	title = {Electric-field-dependent carrier capture and escape in self-assembled InAs/GaAs quantum dots},
	volume = {77},
	year = {2000}}

@article{Bru19a,
	author = {Bruschini, Claudio and Homulle, Harald and Antolovic, Ivan Michel and Burri, Samuel and Charbon, Edoardo},
	journal = {Light: Science \& Applications},
	keywords = {SPAD},
	number = {1},
	pages = {1--28},
	publisher = {Nature Publishing Group},
	title = {Single-photon avalanche diode imagers in biophotonics: review and outlook},
	volume = {8},
	year = {2019}}

@article{His00,
	title={Performance and design of InGaAs/InP photodiodes for single-photon counting at 1.55 $\mu$m},
	author={Hiskett, Philip A and Buller, Gerald S and Loudon, Alison Y and Smith, Jason M and Gontijo, Ivair and Walker, Andrew C and Townsend, Paul D and Robertson, Michael J},
	journal={Applied Optics},
	volume={39},
	number={36},
	pages={6818--6829},
	year={2000},
	keywords = {SPAD},
	publisher={Optical Society of America}
}

@article{Ghi07,
	author = {Ghioni, Massimo and Gulinatti, Angelo and Rech, Ivan and Zappa, Franco and Cova, Sergio},
	journal = {IEEE Journal of selected topics in quantum electronics},
	keywords = {SPAD},
	number = {4},
	pages = {852--862},
	publisher = {IEEE},
	title = {Progress in silicon single-photon avalanche diodes},
	volume = {13},
	year = {2007}}

@article{Zap07,
	author = {Zappa, Franco and Tisa, Simone and Tosi, Alberto and Cova, Sergio},
	journal = {Sensors and Actuators A: Physical},
	keywords = {SPAD},
	number = {1},
	pages = {103--112},
	publisher = {Elsevier},
	title = {Principles and features of single-photon avalanche diode arrays},
	volume = {140},
	year = {2007}}

@article{Nix32,
	author = {Nix, Foster C},
	journal = {Reviews of Modern Physics},
	keywords = {SPAD},
	number = {4},
	pages = {723},
	publisher = {APS},
	title = {Photo-conductivity},
	volume = {4},
	year = {1932}}

@article{Aru19,
	title={Quantum supremacy using a programmable superconducting processor},
	author={Arute, Frank and Arya, Kunal and Babbush, Ryan and Bacon, Dave and Bardin, Joseph C and Barends, Rami and Biswas, Rupak and Boixo, Sergio and Brandao, Fernando GSL and Buell, David A and others},
	journal={Nature},
	volume={574},
	number={7779},
	pages={505--510},
	year={2019},
	keywords = {Quantum computation},
	publisher={Nature Publishing Group}
}

@article{Rud17,
	author = {Rudolph, Terry},
	journal = {APL Photonics},
	keywords = {Quantum computation},
	number = {3},
	pages = {030901},
	publisher = {AIP Publishing LLC AIP Publishing},
	title = {Why I am optimistic about the silicon-photonic route to quantum computing},
	volume = {2},
	year = {2017}}

@article{Fey86,
	title={Quantum mechanical computers},
	author={Feynman, Richard P},
	journal={Foundations of physics},
	volume={16},
	number={6},
	pages={507--531},
	year={1986},
	keywords = {Quantum computation},
	publisher={Kluwer Academic Publishers-Plenum Publishers}
}

@article{Pir19,
	author = {Pirandola, Stefano},
	journal = {Communications Physics},
	keywords = {Quantum communication},
	number = {1},
	pages = {1--10},
	publisher = {Nature Publishing Group},
	title = {End-to-end capacities of a quantum communication network},
	volume = {2},
	year = {2019}}

@article{Coz19,
	author = {Cozzolino, Daniele and Da Lio, Beatrice and Bacco, Davide and Oxenl{\o}we, Leif Katsuo},
	journal = {Advanced Quantum Technologies},
	keywords = {Quantum communication},
	number = {12},
	pages = {1900038},
	publisher = {Wiley Online Library},
	title = {High-dimensional quantum communication: benefits, progress, and future challenges},
	volume = {2},
	year = {2019}}

@article{Che21,
	author = {Chen, Yu-Ao and Zhang, Qiang and Chen, Teng-Yun and Cai, Wen-Qi and Liao, Sheng-Kai and Zhang, Jun and Chen, Kai and Yin, Juan and Ren, Ji-Gang and Chen, Zhu and others},
	journal = {Nature},
	keywords = {Quantum communication},
	number = {7841},
	pages = {214--219},
	publisher = {Nature Publishing Group},
	title = {An integrated space-to-ground quantum communication network over 4,600 kilometres},
	volume = {589},
	year = {2021}}

@article{Tak07,
	title={Quantum key distribution over a 40-dB channel loss using superconducting single-photon detectors},
	author={Takesue, Hiroki and Nam, Sae Woo and Zhang, Qiang and Hadfield, Robert H and Honjo, Toshimori and Tamaki, Kiyoshi and Yamamoto, Yoshihisa},
	journal={Nature photonics},
	volume={1},
	number={6},
	pages={343--348},
	year={2007},
	keywords = {DSOC},
	publisher={Nature Publishing Group}
}

@article{Gre15,
	title={A superconducting photon-counting receiver for optical communication from the Moon},
	author={Grein, Matthew and Dauler, Eric and Kerman, Andrew and Willis, Matthew and Romkey, Barry and Robinson, Bryan and Murphy, Daniel and Boroson, Don},
	journal={SPIE Newsroom},
	volume={9},
	keywords = {DSOC},
	year={2015}
}

@inproceedings{Iva20,
	author = {Ivanov, Hristo and Leitgeb, Erich},
	booktitle = {2020 22nd International Conference on Transparent Optical Networks (ICTON)},
	keywords = {DSOC},
	organization = {IEEE},
	pages = {1--4},
	title = {Characteristics of Ultra-Long Deep Space FSO Downlinks Using Special Detector Technologies Like SNSPD},
	year = {2020}}

@article{Shi14,
	author = {Shibata, Hiroyuki and Honjo, Toshimori and Shimizu, Kaoru},
	journal = {Optics letters},
	keywords = {QKD, SSPD},
	number = {17},
	pages = {5078--5081},
	publisher = {Optical Society of America},
	title = {Quantum key distribution over a 72 dB channel loss using ultralow dark count superconducting single-photon detectors},
	volume = {39},
	year = {2014}}

@misc{BB84,
	author = {Bennett, Charles H and Brassard, Gilles},
	date-modified = {2022-03-17 13:00:27 +0100},
	journal = {Proceed- ings of IEEE International Conference on Computers, Systems and Signal Processing, Bangalore},
	keywords = {BB84},
	publisher = {IEEE New York},
	title = {Proceedings of the ieee international conference on computers, systems and signal processing},
	year = {1984}}

@article{Cac19,
	author = {Cacciapuoti, Angela Sara and Caleffi, Marcello and Tafuri, Francesco and Cataliotti, Francesco Saverio and Gherardini, Stefano and Bianchi, Giuseppe},
	date-modified = {2022-03-17 13:02:09 +0100},
	journal = {IEEE Network},
	keywords = {Quantum internet},
	number = {1},
	pages = {137--143},
	publisher = {IEEE},
	title = {Quantum internet: networking challenges in distributed quantum computing},
	volume = {34},
	year = {2019}}

@article{Cac20,
	author = {Cacciapuoti, Angela Sara and Caleffi, Marcello and Van Meter, Rodney and Hanzo, Lajos},
	date-modified = {2022-03-17 13:02:24 +0100},
	journal = {IEEE Transactions on Communications},
	keywords = {Quantum encryption},
	number = {6},
	pages = {3808--3833},
	publisher = {IEEE},
	title = {When entanglement meets classical communications: Quantum teleportation for the quantum internet},
	volume = {68},
	year = {2020}}

@article{Cal19,
	title={Intrinsically-limited timing jitter in molybdenum silicide superconducting nanowire single-photon detectors},
	author={Caloz, Misael and Korzh, Boris and Ramirez, Edward and Sch{\"o}nenberger, Christian and Warburton, Richard J and Zbinden, Hugo and Shaw, Matthew D and Bussi{\`e}res, F{\'e}lix},
	journal={Journal of Applied Physics},
	volume={126},
	number={16},
	pages={164501},
	year={2019},
	publisher={AIP Publishing LLC}
}

@inproceedings{Cal19b,
	author = {Calvo, Ramon Mata and Poliak, Juraj and Surof, Janis and Reeves, Andrew and Richerzhagen, Mathias and Kelemu, Helawae Friew and Barrios, Ricardo and Carrizo, Carlos and Wolf, Raphael and Rein, Fabian and others},
	booktitle = {Free-Space Laser Communications XXXI},
	keywords = {DSOC},
	organization = {SPIE},
	pages = {189--204},
	title = {Optical technologies for very high throughput satellite communications},
	volume = {10910},
	year = {2019}}

@article{Weh18,
	author = {Wehner, Stephanie and Elkouss, David and Hanson, Ronald},
	journal = {Science},
	number = {6412},
	pages = {eaam9288},
	publisher = {American Association for the Advancement of Science},
	title = {Quantum internet: A vision for the road ahead},
	volume = {362},
	year = {2018}}

@article{Ghe19,
	author = {Gheorghiu, Alexandru and Kapourniotis, Theodoros and Kashefi, Elham},
	journal = {Theory of computing systems},
	number = {4},
	pages = {715--808},
	publisher = {Springer},
	title = {Verification of quantum computation: An overview of existing approaches},
	volume = {63},
	year = {2019}}

@article{Div95,
	author = {DiVincenzo, David P},
	date-modified = {2022-03-17 13:12:17 +0100},
	journal = {Science},
	keywords = {Quantum computation},
	number = {5234},
	pages = {255--261},
	publisher = {American Association for the Advancement of Science},
	title = {Quantum computation},
	volume = {270},
	year = {1995}}

@article{Los98,
	author = {Loss, Daniel and DiVincenzo, David P},
	journal = {Physical Review A},
	number = {1},
	pages = {120},
	publisher = {APS},
	title = {Quantum computation with quantum dots},
	volume = {57},
	year = {1998}}

@article{Zha01,
	author = {Zhang, Yong-Sheng and Li, Chuan-Feng and Guo, Guang-Can},
	date-modified = {2022-03-17 12:12:04 +0100},
	journal = {Physical Review A},
	keywords = {Quantum encryption},
	number = {2},
	pages = {024302},
	publisher = {APS},
	title = {Quantum key distribution via quantum encryption},
	volume = {64},
	year = {2001}}

@article{Rem20,
	author = {Rembold, Phila and Oshnik, Nimba and M{\"u}ller, Matthias M and Montangero, Simone and Calarco, Tommaso and Neu, Elke},
	date-modified = {2022-03-17 12:14:01 +0100},
	journal = {AVS Quantum Science},
	keywords = {Quantum sensing},
	number = {2},
	pages = {024701},
	publisher = {American Vacuum Society},
	title = {Introduction to quantum optimal control for quantum sensing with nitrogen-vacancy centers in diamond},
	volume = {2},
	year = {2020}}

@article{Pir18,
	author = {Pirandola, Stefano and Bardhan, B Roy and Gehring, Tobias and Weedbrook, Christian and Lloyd, Seth},
	date-modified = {2022-03-17 12:13:44 +0100},
	journal = {Nature Photonics},
	keywords = {Quantum sensing},
	number = {12},
	pages = {724--733},
	publisher = {Nature Publishing Group},
	title = {Advances in photonic quantum sensing},
	volume = {12},
	year = {2018}}

@article{Deg17,
	author = {Degen, Christian L and Reinhard, F and Cappellaro, Paola},
	date-modified = {2022-03-17 12:13:31 +0100},
	journal = {Reviews of modern physics},
	keywords = {Quantum sensing},
	number = {3},
	pages = {035002},
	publisher = {APS},
	title = {Quantum sensing},
	volume = {89},
	year = {2017}}

@article{Ber20,
	author = {Bergeron, L and Chartrand, C and Kurkjian, ATK and Morse, KJ and Riemann, H and Abrosimov, NV and Becker, P and Pohl, H-J and Thewalt, MLW and Simmons, S},
	date-modified = {2022-03-17 13:01:28 +0100},
	journal = {PRX Quantum},
	keywords = {Spin-photon interface},
	number = {2},
	pages = {020301},
	publisher = {APS},
	title = {Silicon-integrated telecommunications photon-spin interface},
	volume = {1},
	year = {2020}}

@article{Ata18,
	author = {Atat{\"u}re, Mete and Englund, Dirk and Vamivakas, Nick and Lee, Sang-Yun and Wrachtrup, Joerg},
	date-modified = {2022-03-17 12:09:12 +0100},
	journal = {Nature Reviews Materials},
	keywords = {Spin-photon interface},
	number = {5},
	pages = {38--51},
	publisher = {Nature Publishing Group},
	title = {Material platforms for spin-based photonic quantum technologies},
	volume = {3},
	year = {2018}}

@article{MiX18,
	author = {Mi, Xiao and Benito, M{\'o}nica and Putz, Stefan and Zajac, David M and Taylor, Jacob M and Burkard, Guido and Petta, Jason R},
	journal = {Nature},
	number = {7698},
	pages = {599--603},
	publisher = {Nature Publishing Group},
	title = {A coherent spin--photon interface in silicon},
	volume = {555},
	year = {2018}}

@article{Jav18,
	author = {Javadi, Alisa and Ding, Dapeng and Appel, Martin Hayhurst and Mahmoodian, Sahand and L{\"o}bl, Matthias Christian and S{\"o}llner, Immo and Schott, R{\"u}diger and Papon, Camille and Pregnolato, Tommaso and Stobbe, S{\o}ren and others},
	journal = {Nature nanotechnology},
	number = {5},
	pages = {398--403},
	publisher = {Nature Publishing Group},
	title = {Spin--photon interface and spin-controlled photon switching in a nanobeam waveguide},
	volume = {13},
	year = {2018}}

@article{Hua20,
	author = {Huang, He-Liang and Wu, Dachao and Fan, Daojin and Zhu, Xiaobo},
	date-modified = {2022-03-17 12:10:41 +0100},
	journal = {Science China Information Sciences},
	keywords = {Superconducting qubits},
	number = {8},
	pages = {1--32},
	publisher = {Springer},
	title = {Superconducting quantum computing: a review},
	volume = {63},
	year = {2020}}

@article{Goo20,
	author = {Google-AI-Quantum and Arute, Frank and Arya, Kunal and Babbush, Ryan and Bacon, Dave and Bardin, Joseph C and Barends, Rami and Boixo, Sergio and Broughton, Michael and Buckley, Bob B and others},
	date-modified = {2022-03-17 12:10:51 +0100},
	journal = {Science},
	keywords = {Superconducting qubits},
	number = {6507},
	pages = {1084--1089},
	publisher = {American Association for the Advancement of Science},
	title = {Hartree-Fock on a superconducting qubit quantum computer},
	volume = {369},
	year = {2020}}

@article{Kie02,
	author = {Kielpinski, David and Monroe, Chris and Wineland, David J},
	date-modified = {2022-03-17 12:19:32 +0100},
	journal = {Nature},
	keywords = {Trapped ions},
	number = {6890},
	pages = {709--711},
	publisher = {Nature Publishing Group},
	title = {Architecture for a large-scale ion-trap quantum computer},
	volume = {417},
	year = {2002}}

@article{Lek17,
	author = {Lekitsch, Bjoern and Weidt, Sebastian and Fowler, Austin G and M{\o}lmer, Klaus and Devitt, Simon J and Wunderlich, Christof and Hensinger, Winfried K},
	date-modified = {2022-03-17 12:19:47 +0100},
	journal = {Science Advances},
	keywords = {Trapped ions},
	number = {2},
	pages = {e1601540},
	publisher = {American Association for the Advancement of Science},
	title = {Blueprint for a microwave trapped ion quantum computer},
	volume = {3},
	year = {2017}}

@article{Bru19b,
	author = {Bruzewicz, Colin D and Chiaverini, John and McConnell, Robert and Sage, Jeremy M},
	date-modified = {2022-03-17 12:20:03 +0100},
	journal = {Applied Physics Reviews},
	keywords = {Trapped ions},
	number = {2},
	pages = {021314},
	publisher = {AIP Publishing LLC},
	title = {Trapped-ion quantum computing: Progress and challenges},
	volume = {6},
	year = {2019}}

@article{Maz19,
	author = {Mazhandu, Farai and Mathieson, Kayleigh and Coleman, Christopher and Bhattacharyya, Somnath},
	date-modified = {2022-03-17 12:17:58 +0100},
	journal = {Applied Physics Letters},
	keywords = {NV-centers},
	number = {23},
	pages = {233501},
	publisher = {AIP Publishing LLC},
	title = {Experimental simulation of hybrid quantum systems and entanglement on a quantum computer},
	volume = {115},
	year = {2019}}

@article{Chi13,
	author = {Childress, Lilian and Hanson, Ronald},
	date-modified = {2022-03-17 12:17:41 +0100},
	journal = {MRS bulletin},
	keywords = {NV-centers},
	number = {2},
	pages = {134--138},
	publisher = {Cambridge University Press},
	title = {Diamond NV centers for quantum computing and quantum networks},
	volume = {38},
	year = {2013}}

@article{Pez21,
	author = {Pezzagna, S{\'e}bastien and Meijer, Jan},
	date-modified = {2022-03-17 12:18:16 +0100},
	journal = {Applied Physics Reviews},
	keywords = {NV-centers},
	number = {1},
	pages = {011308},
	publisher = {AIP Publishing LLC},
	title = {Quantum computer based on color centers in diamond},
	volume = {8},
	year = {2021}}

@article{Wan20,
	abstract = {Quantum technologies comprise an emerging class of devices capable of controlling superposition and entanglement of quantum states of light or matter, to realize fundamental performance advantages over ordinary classical machines. The technology of integrated quantum photonics has enabled the generation, processing and detection of quantum states of light at a steadily increasing scale and level of complexity, progressing from few-component circuitry occupying centimetre-scale footprints and operating on two photons, to programmable devices approaching 1,000 components occupying millimetre-scale footprints with integrated generation of multiphoton states. This Review summarizes the advances in integrated photonic quantum technologies and its demonstrated applications, including quantum communications, simulations of quantum chemical and physical systems, sampling algorithms, and linear-optic quantum information processing.},
	author = {Wang, Jianwei and Sciarrino, Fabio and Laing, Anthony and Thompson, Mark G.},
	da = {2020/05/01},
	date-added = {2022-03-17 11:11:51 +0100},
	date-modified = {2022-03-17 11:12:00 +0100},
	doi = {10.1038/s41566-019-0532-1},
	id = {Wang2020},
	isbn = {1749-4893},
	journal = {Nature Photonics},
	number = {5},
	pages = {273--284},
	title = {Integrated photonic quantum technologies},
	ty = {JOUR},
	url = {https://doi.org/10.1038/s41566-019-0532-1},
	volume = {14},
	year = {2020},
	Bdsk-Url-1 = {https://doi.org/10.1038/s41566-019-0532-1}}

@article{Cir00,
	abstract = {Quantum computers require the storage of quantum information in a set of two-level systems (called qubits), the processing of this information using quantum gates and a means of final readout1. So far, only a few systems have been identified as potentially viable quantum computer models---accurate quantum control of the coherent evolution is required in order to realize gate operations, while at the same time decoherence must be avoided. Examples include quantum optical systems (such as those utilizing trapped ions2,3,4,5,6,7,8,9 or neutral atoms10,11,12, cavity quantum electrodynamics13,14,15 and nuclear magnetic resonance16,17) and solid state systems (using nuclear spins1,18, quantum dots19 and Josephson junctions20). The most advanced candidates are the quantum optical and nuclear magnetic resonance systems, and we expect that they will allow quantum computing with about ten qubits within the next few years. This is still far from the numbers required for useful applications: for example, the factorization of a 200-digit number requires about 3,500 qubits21, rising to 100,000 if error correction22 is implemented. Scalability of proposed quantum computer architectures to many qubits is thus of central importance. Here we propose a model for an ion trap quantum computer that combines scalability (a feature usually associated with solid state proposals) with the advantages of quantum optical systems (in particular, quantum control and long decoherence times).},
	author = {Cirac, J. I. and Zoller, P.},
	da = {2000/04/01},
	date-added = {2022-03-17 10:57:46 +0100},
	date-modified = {2022-03-17 12:19:12 +0100},
	doi = {10.1038/35007021},
	id = {Cirac2000},
	isbn = {1476-4687},
	journal = {Nature},
	keywords = {Trapped ions, Quantum computation},
	number = {6778},
	pages = {579--581},
	title = {A scalable quantum computer with ions in an array of microtraps},
	ty = {JOUR},
	url = {https://doi.org/10.1038/35007021},
	volume = {404},
	year = {2000},
	Bdsk-Url-1 = {https://doi.org/10.1038/35007021}}

@article{Cla08,
	abstract = {Superconducting circuits are macroscopic in size but have generic quantum properties such as quantized energy levels, superposition of states, and entanglement, all of which are more commonly associated with atoms. Superconducting quantum bits (qubits) form the key component of these circuits. Their quantum state is manipulated by using electromagnetic pulses to control the magnetic flux, the electric charge or the phase difference across a Josephson junction (a device with nonlinear inductance and no energy dissipation). As such, superconducting qubits are not only of considerable fundamental interest but also might ultimately form the primitive building blocks of quantum computers.},
	author = {Clarke, John and Wilhelm, Frank K.},
	da = {2008/06/01},
	date-added = {2022-03-17 10:55:27 +0100},
	date-modified = {2022-03-17 12:09:53 +0100},
	doi = {10.1038/nature07128},
	id = {Clarke2008},
	isbn = {1476-4687},
	journal = {Nature},
	keywords = {Superconducting qubits},
	number = {7198},
	pages = {1031--1042},
	title = {Superconducting quantum bits},
	ty = {JOUR},
	url = {https://doi.org/10.1038/nature07128},
	volume = {453},
	year = {2008},
	Bdsk-Url-1 = {https://doi.org/10.1038/nature07128}}

@article{Han20,
	annote = {doi: 10.1126/science.abe8770},
	author = {Zhong HanSen and Wang Hui and Deng Yu-Hao and Chen Ming-Cheng and Peng Li-Chao and Luo Yi-Han and Qin Jian and Wu Dian and Ding Xing and Hu Yi and Hu Peng and Yang Xiao-Yan and Zhang Wei-Jun and Li Hao and Li Yuxuan and Jiang Xiao and Gan Lin and Yang Guangwen and You Lixing and Wang Zhen and Li Li and Liu Nai-Le and Lu Chao-Yang and Pan Jian-Wei},
	booktitle = {Science},
	da = {2020/12/18},
	date = {2020/12/18},
	date-added = {2022-03-17 10:41:46 +0100},
	date-modified = {2022-03-17 12:20:37 +0100},
	doi = {10.1126/science.abe8770},
	journal = {Science},
	journal1 = {Science},
	keywords = {Photonic quantum computer, Quantum computation, Photons},
	m3 = {doi: 10.1126/science.abe8770},
	month = {2022/03/17},
	number = {6523},
	pages = {1460--1463},
	publisher = {American Association for the Advancement of Science},
	title = {Quantum computational advantage using photons},
	ty = {JOUR},
	url = {https://doi.org/10.1126/science.abe8770},
	volume = {370},
	year = {2020},
	year1 = {2020},
	Bdsk-Url-1 = {https://doi.org/10.1126/science.abe8770}}

@article{Smi20,
	abstract = {Technology hype is an important concept in business, marketing, and science and technology studies, but it is rarely related to security studies. What is technology hype? How does it relate to nati...},
	author = {Smith, Frank L.},
	date-added = {2022-03-17 10:12:07 +0100},
	date-modified = {2022-03-17 10:12:16 +0100},
	doi = {10.1177/0967010620904922},
	file = {Smith 2020 - Quantum technology hype and national:C\:\\Users\\christian.schmid\\Documents\\Citavi 6\\Projects\\Thesis\\Citavi Attachments\\Smith 2020 - Quantum technology hype and national.pdf:pdf},
	journal = {Security Dialogue},
	number = {5},
	pages = {499--516},
	title = {Quantum technology hype and national security},
	volume = {51},
	year = {2020},
	Bdsk-Url-1 = {https://doi.org/10.1177/0967010620904922}}

@article{Hos16,
	abstract = {Quantum metrology uses quantum entanglement--correlations in the properties of microscopic systems--to improve the statistical precision of physical measurements. When measuring a signal, such as the phase shift of a light beam or an atomic state, a prominent limitation to achievable precision arises from the noise associated with the counting of uncorrelated probe particles. This noise, commonly referred to as shot noise or projection noise, gives rise to the standard quantum limit (SQL) to phase resolution. However, it can be mitigated down to the fundamental Heisenberg limit by entangling the probe particles. Despite considerable experimental progress in a variety of physical systems, a question that persists is whether these methods can achieve performance levels that compare favourably with optimized conventional (non-entangled) systems. Here we demonstrate an approach that achieves unprecedented levels of metrological improvement using half a million (87)Rb atoms in their 'clock' states. The ensemble is 20.1 $\pm$ 0.3 decibels (100-fold) spin-squeezed via an optical-cavity-based measurement. We directly resolve small microwave-induced rotations 18.5 $\pm$ 0.3 decibels (70-fold) beyond the SQL. The single-shot phase resolution of 147 microradians achieved by the apparatus is better than that achieved by the best engineered cold atom sensors despite lower atom numbers. We infer entanglement of more than 680 $\pm$ 35 particles in the atomic ensemble. Applications include atomic clocks, inertial sensors, and fundamental physics experiments such as tests of general relativity or searches for electron electric dipole moment. To this end, we demonstrate an atomic clock measurement with a quantum enhancement of 10.5 $\pm$ 0.3 decibels (11-fold), limited by the phase noise of our microwave source.},
	address = {Department of Physics, Stanford University, Stanford, California 94305, USA.; Department of Physics, Stanford University, Stanford, California 94305, USA.; Department of Physics, Stanford University, Stanford, California 94305, USA.; Department of Physics, Stanford University, Stanford, California 94305, USA.},
	author = {Hosten, Onur and Engelsen, Nils J and Krishnakumar, Rajiv and Kasevich, Mark A},
	crdt = {2016/01/12 06:00},
	date = {2016 Jan 28},
	date-added = {2022-03-17 09:49:38 +0100},
	date-modified = {2022-03-17 12:13:11 +0100},
	dcom = {20160211},
	dep = {20160111},
	doi = {10.1038/nature16176},
	edat = {2016/01/12 06:00},
	issn = {1476-4687 (Electronic); 0028-0836 (Linking)},
	jid = {0410462},
	journal = {Nature},
	jt = {Nature},
	keywords = {Metrology},
	language = {eng},
	lid = {10.1038/nature16176 {$[$}doi{$]$}},
	lr = {20160128},
	mhda = {2016/01/12 06:01},
	month = {Jan},
	number = {7587},
	own = {NLM},
	pages = {505--508},
	phst = {2015/06/30 00:00 {$[$}received{$]$}; 2015/10/22 00:00 {$[$}accepted{$]$}; 2016/01/12 06:00 {$[$}entrez{$]$}; 2016/01/12 06:00 {$[$}pubmed{$]$}; 2016/01/12 06:01 {$[$}medline{$]$}},
	pii = {nature16176},
	pl = {England},
	pmid = {26751056},
	pst = {ppublish},
	pt = {Journal Article; Research Support, Non-U.S. Gov't; Research Support, U.S. Gov't, Non-P.H.S.},
	status = {PubMed-not-MEDLINE},
	title = {Measurement noise 100 times lower than the quantum-projection limit using entangled atoms.},
	volume = {529},
	year = {2016},
	Bdsk-Url-1 = {https://doi.org/10.1038/nature16176}}

@article{Aci18,
	abstract = {Within the last two decades, quantum technologies (QT) have made tremendous progress, moving from Nobel Prize award-winning experiments on quantum physics (1997: Chu, Cohen-Tanoudji, Phillips; 2001: Cornell, Ketterle, Wieman; 2005: Hall, H{\"a}nsch-, Glauber; 2012: Haroche, Wineland) into a cross-disciplinary field of applied research. Technologies are being developed now that explicitly address individual quantum states and make use of the `strange'quantum properties, such as superposition and entanglement. The field comprises four domains: quantum communication, where individual or entangled photons are used to transmit data in a provably secure way; quantum simulation, where well-controlled quantum systems are used to reproduce the behaviour of other, less accessible quantum systems; quantum computation, which employs quantum effects to dramatically speed up certain calculations, such as number factoring; and quantum sensing and metrology, where the high sensitivity of coherent quantum systems to external perturbations is exploited to enhance the performance of measurements of physical quantities. In Europe, the QT community has profited from several EC funded coordination projects, which, among other things, have coordinated the creation of a 150-page QT Roadmap (http://qurope.eu/h2020/qtflagship/roadmap2016). This article presents an updated summary of this roadmap.},
	author = {Ac{\'\i}n, Antonio and Bloch, Immanuel and Buhrman, Harry and Calarco, Tommaso and Eichler, Christopher and Eisert, Jens and Esteve, Daniel and Gisin, Nicolas and Glaser, Steffen J and Jelezko, Fedor and Kuhr, Stefan and Lewenstein, Maciej and Riedel, Max F and Schmidt, Piet O and Thew, Rob and Wallraff, Andreas and Walmsley, Ian and Wilhelm, Frank K},
	booktitle = {New Journal of Physics},
	da = {2018/08/15},
	date-added = {2022-03-17 09:39:50 +0100},
	date-modified = {2022-03-17 12:21:40 +0100},
	doi = {10.1088/1367-2630/aad1ea},
	isbn = {1367-2630},
	journal = {New Journal of Physics},
	keywords = {Review},
	number = {8},
	pages = {080201},
	publisher = {IOP Publishing},
	title = {The quantum technologies roadmap: a European community view},
	ty = {JOUR},
	url = {http://dx.doi.org/10.1088/1367-2630/aad1ea},
	volume = {20},
	year = {2018},
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/1367-2630/aad1ea}}

@article{Cir17,
	abstract = {Quantum optics is a well-established field that spans from fundamental physics to quantum information science. In the coming decade, areas including computation, communication and metrology are all likely to experience scientific and technological advances supported by this far-reaching research field.},
	author = {Cirac, J. Ignacio and Kimble, H. Jeff},
	da = {2017/01/01},
	date-added = {2022-03-17 09:26:53 +0100},
	date-modified = {2022-03-17 12:09:41 +0100},
	doi = {10.1038/nphoton.2016.259},
	id = {Cirac2017},
	isbn = {1749-4893},
	journal = {Nature Photonics},
	keywords = {Review},
	number = {1},
	pages = {18--20},
	title = {Quantum optics, what next?},
	ty = {JOUR},
	url = {https://doi.org/10.1038/nphoton.2016.259},
	volume = {11},
	year = {2017},
	Bdsk-Url-1 = {https://doi.org/10.1038/nphoton.2016.259}}

@techreport{Bro14,
	address = {TINA memo 2003-003},
	author = {P. Bromiley},
	date-added = {2018-06-01 00:26:39 +0000},
	date-modified = {2018-06-01 00:29:02 +0000},
	institution = {University of Manchester},
	number = {maging Sciences Research Group},
	organization = {University of Manchester},
	title = {Prducts and Convolutions of Gaussian Probability Density Functions},
	type = {Institute of Population Health},
	year = {2014}}

@article{Per12,
	author = {W. Pernice AND C. Schuck AND O. Minaeva AND M. Li AND G. Goltsman AND A. Sergienko AND H. Tang},
	date-added = {2018-06-01 00:24:59 +0000},
	date-modified = {2018-06-01 00:26:35 +0000},
	journal = {Nature Communications},
	number = {1325},
	title = {High-speed and high-efficiency travelling wave single-photon detectors embedded in nanophotonic circuits},
	volume = {3},
	year = {2012}}

@article{Gis02,
	author = {N. Gisin AND G. Ribordy AND W. Tittel AND H. Zbinden},
	date-added = {2018-05-22 07:15:07 +0000},
	date-modified = {2018-05-22 07:15:56 +0000},
	journal = {Reviews of Modern Physics},
	pages = {145-195},
	title = {Quantum cryptography},
	volume = {74},
	year = {2002}}

@article{Dua01,
	author = {L.-M. Duan AND M. Lukin AND J. cirac AND P. Zoller},
	date-added = {2018-05-22 07:13:53 +0000},
	date-modified = {2018-05-22 07:15:03 +0000},
	journal = {Nature},
	pages = {413-418},
	title = {Long-distance quantum communication with atomic ensembles and linear optics},
	volume = {414},
	year = {2001}}

@article{Kim08,
	author = {H. Kimble},
	date-added = {2018-05-22 07:13:24 +0000},
	date-modified = {2022-03-17 12:11:47 +0100},
	journal = {Nature},
	keywords = {Quantum internet},
	pages = {1023-1030},
	title = {The quantum internet},
	volume = {453},
	year = {2008}}

@article{Var08,
	author = {M. Varnava AND D. Browne AND T. Rudolph},
	date-added = {2018-05-22 07:10:26 +0000},
	date-modified = {2018-05-22 07:11:24 +0000},
	journal = {Physical Review Letters},
	number = {060502},
	title = {How Good Must SIngle Photon Sources and Detectors Be for Efficient Linear Optical Quantum Computation?},
	volume = {100},
	year = {2008}}

@article{Had09,
	author = {R. Hadfield},
	date-added = {2018-05-22 07:09:47 +0000},
	date-modified = {2018-05-22 07:10:23 +0000},
	journal = {Nature Photonics},
	pages = {696-795},
	title = {Single-photon detectors for optical quantum information applications},
	volume = {3},
	keywords={Review},
	year = {2009}}

@article{DiV00,
	author = {D. DiVicenzo},
	date-added = {2018-05-22 07:09:03 +0000},
	date-modified = {2022-03-17 13:12:25 +0100},
	journal = {Fortschritte der Physik},
	keywords = {Quantum computation},
	pages = {771-783},
	title = {The Physical Implementation of Quantum Computation},
	volume = {48},
	year = {2000}}

@article{Fic18,
	author = {Q. Ficheux AND S. Jezouin AND Z. Leghtas AND B. Huard},
	date-added = {2018-05-22 07:08:18 +0000},
	date-modified = {2018-05-22 07:08:52 +0000},
	journal = {Nature Communications},
	number = {1926},
	title = {Dynamics of a qubit while simultaneously monitoring its relaxation and dephasing},
	volume = {9},
	year = {2018}}

@article{Iku18,
	author = {R. Ikuta AND T. Kobayashi AND T. Kawakami AND S. Miki AND M. Yabuno AND T. Yamashita AND H. Terai AND M. Koashi AND T. Mukai AND T. Yamamoto AND N. Imoto},
	date-added = {2018-05-22 07:07:36 +0000},
	date-modified = {2018-05-22 07:08:15 +0000},
	journal = {Nature Communications},
	number = {1997},
	title = {Polarization insensitive frequency conversion for an atom-photon entanglement distribution via a telecom network},
	volume = {9},
	year = {2018}}

@article{Zen17,
	author = {W. Zeng AND B. Johnson AND R. Smith AND N. Rubin AND M. Reagor AND C. Ryan AND C. Rigetti},
	date-added = {2018-05-22 07:06:30 +0000},
	date-modified = {2018-05-22 07:07:33 +0000},
	journal = {Nature},
	number = {7671},
	title = {First quantum computers need smart software},
	volume = {549},
	year = {2017}}

@article{Fey82,
	author = {R. Feynman},
	date-added = {2018-05-22 07:05:21 +0000},
	date-modified = {2022-03-17 13:12:54 +0100},
	journal = {International Journal of Theoretical Physics},
	keywords = {Quantum simulation},
	number = {6},
	pages = {467-488},
	title = {Simulating physics with computers},
	volume = {21},
	year = {1982}}

@article{Pla13,
	author = {J. Pla AND K. Tan AND J. Dehollain AND W. Lim AND J. Morton AND F. Zwanenburg AND D. Jamieson AND A. Dzurak AND A. Morello},
	date-added = {2018-05-22 07:03:42 +0000},
	date-modified = {2018-05-22 07:05:18 +0000},
	journal = {Nature},
	number = {7445},
	title = {High-fidelity readout and control of a nuclear spin qubit in silicon},
	volume = {496},
	year = {2013}}

@article{Lei05,
	author = {D. Leibfried AND E. Knill AND S. Seidelin AND J. Britton AND R. Blakestad AND J. Chiaverini AND D. Hume AND W. Itano AND J. Jost AND C. Lagner AND R. Ozeri AND R. Reichle AND D. Wineland},
	date-added = {2018-05-22 07:01:38 +0000},
	date-modified = {2018-05-22 07:03:18 +0000},
	journal = {Nature},
	pages = {639-642},
	title = {Creation of a six-atom Schrodinger cat state},
	volume = {438},
	year = {2005}}

@article{Deu85,
	author = {D. Deutsch},
	date-added = {2018-05-22 07:00:03 +0000},
	date-modified = {2018-05-22 07:01:36 +0000},
	journal = {Proceedings of the Royal Society of London},
	number = {1818},
	pages = {97-117},
	title = {Quantum Theory, the Church-Turing Principle and the Universal Quantum Computer},
	volume = {400},
	year = {1985},
	Bdsk-File-1 = {YnBsaXN0MDDSAQIDBFxyZWxhdGl2ZVBhdGhZYWxpYXNEYXRhXxAhLi4vLi4vRG93bmxvYWRzL0lPUEVYUE9SVF9SSVMucmlzTxEBVAAAAAABVAACAAAMTWFjaW50b3NoIEhEAAAAAAAAAAAAAAAAAAAAAAAAAEJEAAH/////EUlPUEVYUE9SVF9SSVMucmlzAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAP////8AAAAAAAAAAAAAAAAAAgACAAAKIGN1AAAAAAAAAAAAAAAAAAlEb3dubG9hZHMAAAIAKi86VXNlcnM6cmFzbXVzOkRvd25sb2FkczpJT1BFWFBPUlRfUklTLnJpcwAOACQAEQBJAE8AUABFAFgAUABPAFIAVABfAFIASQBTAC4AcgBpAHMADwAaAAwATQBhAGMAaQBuAHQAbwBzAGgAIABIAEQAEgAoVXNlcnMvcmFzbXVzL0Rvd25sb2Fkcy9JT1BFWFBPUlRfUklTLnJpcwATAAEvAAAVAAIADf//AAAACAANABoAJABIAAAAAAAAAgEAAAAAAAAABQAAAAAAAAAAAAAAAAAAAaA=}}

@article{Geo14,
	author = {I. Georgescu AND S. Ashhab AND F. Nori},
	date-added = {2018-05-22 06:58:52 +0000},
	date-modified = {2018-05-22 06:59:56 +0000},
	journal = {Reviews of Modern Physics},
	number = {153},
	title = {Quantum simulation},
	volume = {86},
	year = {2014}}

@article{Kit04,
	author = {D. Kitchen AND D. Decornez AND J. Furr AND J. Bajorath},
	date-added = {2018-05-22 06:57:46 +0000},
	date-modified = {2018-05-22 06:58:49 +0000},
	journal = {Nature Reviews Drug Discovery},
	pages = {935-949},
	title = {Docking and scoring in virtual screening for drug discovery: methods and applications},
	volume = {3},
	year = {2004}}

@article{Cox00,
	author = {P. Cox AND R. Betts AND C. Jones AND S. Spall AND I. Totterdell},
	date-added = {2018-05-22 06:56:20 +0000},
	date-modified = {2018-05-22 06:57:35 +0000},
	journal = {Nature},
	pages = {184-187},
	title = {Acceleration of global warming due to carbon-cycle feedbacks in a coupled climate model},
	volume = {408},
	year = {2000}}

@article{Des16,
	author = {S. Desai AND S. Madhvapathy AND A. Sachid AND J. Llinas AND Q. Wang AND G. Ahn AND G. Pitner AND M. Kim AND J. Bokor AND C. Hu AND H.-S. Wong AND A. Javey},
	date-added = {2018-05-22 06:55:10 +0000},
	date-modified = {2018-05-22 06:56:16 +0000},
	journal = {Science},
	number = {6308},
	pages = {99-102},
	title = {MoS2 transistors with 1-nanometer gate lengths},
	volume = {354},
	year = {2016}}

@article{Moo65,
	author = {G. Moore},
	date-added = {2018-05-22 06:54:32 +0000},
	date-modified = {2018-05-22 06:55:07 +0000},
	journal = {Electronics},
	number = {8},
	title = {Cramming more components onto integrated circuits},
	volume = {38},
	year = {1965}}

@article{Mat72,
	author = {M. Mathur AND D. Deis AND J. Gavaler},
	date-added = {2018-05-22 06:51:43 +0000},
	date-modified = {2018-05-22 06:52:35 +0000},
	journal = {Journal of Applied Physics},
	number = {3158},
	title = {Lower Critical Field Measurements in NbN Bulk and Thin Films},
	volume = {43},
	year = {1972}}

@article{Doc11,
	author = {D. Dochev AND V. Desmaris AND A. Pavolotky AND D. Meledin AND Z. Lai AND E. Janzen AND E. Pippel AND J. Woltersdorf AND V. Belitsky},
	date-added = {2018-05-22 06:50:34 +0000},
	date-modified = {2018-05-22 06:51:40 +0000},
	journal = {Superconductor Science and Technology},
	number = {3},
	title = {Growth and characterization of epitaxial ultra-thin NbN films on 3C-Sic/Si substrate for terahertz applications},
	volume = {24},
	year = {2011}}

@conference{Lee06,
	author = {H. Lee AND L.Heun Yu AND S.-W. Ryu AND J.-W. Han AND K. Jeon AND D.-Y. Jang AND K.-H. Kim AND J. Lee AND J.-H. Kim AND J. Cheol AND G. Lee AND O. Sub AND P. Chang AND W. Bae AND L. Mok AND J. Yang AND J. Yoo AND S. Kim AND C. Yang-Kyu},
	date-added = {2018-05-22 06:47:38 +0000},
	date-modified = {2018-05-22 06:50:10 +0000},
	journal = {VLSI Technology},
	pages = {58-59},
	title = {Sub-5nm All-Around Gate FinFET for Ultimate Scaling},
	volume = {12},
	year = {2006}}

@conference{Yan04,
	author = {F.-L. Yang AND D.-H. Lee AND H.-Y. Chen AND C.-Y. Chang AND S.-D. Liu AND C.-C. Huang AND T.-X. Chung AND H.-W. Chen AND C.-C. Huang AND Y.-H. Liu AND C.-C. Wu AND C.-C. Chen AND S.-C. Chen AND Y.-T. Chen AND Y.-H. Chen AND C.-J. Chen AND B.-W. Chan AND P.-F. Hsu AND J.-H. Shieh AND H.-J. Tao AND Y.-C. Yeo AND Y. Li, J.-W. Lee AND P. Chen AND M.-S. Liang AND C. Hu},
	date-added = {2018-05-22 06:43:46 +0000},
	date-modified = {2018-05-22 06:50:30 +0000},
	journal = {VLSI Technology},
	pages = {196-197},
	title = {5nm-gate nanowire FinFET},
	year = {2004}}

@article{Obr09,
	author = {J. O'Brien AND A. Furusawa AND J. Vuckovic},
	date-added = {2018-05-22 06:42:55 +0000},
	date-modified = {2018-05-22 06:43:42 +0000},
	journal = {Nature Photonics},
	pages = {687-695},
	title = {Photonic quantum technologies},
	volume = {3},
	year = {2009}}

@article{Kni01,
	author = {E. Knill AND R. Lamme AND G. Milburng},
	date-added = {2018-05-22 06:41:41 +0000},
	date-modified = {2018-05-22 06:42:24 +0000},
	journal = {Nature},
	pages = {46-52},
	title = {Scheme for efficient quantum computation with linear optics},
	volume = {409},
	year = {2001}}

@article{Obr03,
	author = {J. O'Brien AND G. Pryde AND A. White AND T. Ralph AND D. Branning},
	date-added = {2018-05-22 06:40:37 +0000},
	date-modified = {2018-05-22 06:41:38 +0000},
	journal = {Nature},
	pages = {264-267},
	title = {Demonstration of an all-optical quantum controlled NOT gate},
	volume = {426},
	year = {2003}}

@article{Obr07,
	author = {J. O'Brien},
	date-added = {2018-05-22 06:39:38 +0000},
	date-modified = {2018-05-22 06:40:28 +0000},
	journal = {Science},
	pages = {156-1570},
	title = {Optical Qantum Computing},
	volume = {318},
	year = {2007}}

@article{Pol09,
	author = {A. Politi AND J. Matthews AND M. Thompson AND J. O'Brien},
	date-added = {2018-05-22 06:38:51 +0000},
	date-modified = {2018-05-22 06:39:26 +0000},
	journal = {IEEE Transactions on Applied Superconductivity},
	number = {6},
	title = {Integrated Quantum Photonics},
	volume = {15},
	year = {2009}}

@article{Ren14,
	author = {J. Renema AND R. Gaudio AND Q. Wang AND Z. Zhou AND A. Gaggero AND F. Mattioli AND R. Leoni AND D. Sahin AND M. de Dood AND A. Fiore AND M. van Exter},
	date-added = {2018-05-21 06:42:59 +0000},
	date-modified = {2018-05-21 06:43:38 +0000},
	journal = {Physical Review Letters},
	number = {117604},
	title = {Experimental Test of Theories of the Detection Mechanism in a Nanowire Superconducting Single Photon Detector},
	volume = {112},
	year = {2014}}

@article{Zho13,
	author = {Z. Zhou AND G. Frucci AND F. Mattioli AND A. Gaggero AND R. Leoni AND S. Jahanmirinejad AND T. Hoang AND A. Fiore},
	date-added = {2018-05-21 06:42:09 +0000},
	date-modified = {2018-05-21 06:42:53 +0000},
	journal = {Physical Review Letters},
	number = {113605},
	title = {Ultrasensitive N-Photon Interferometric Autocorrelator},
	volume = {110},
	year = {2013}}

@article{Gau16,
	author = {R. Gaudio AND J. Renema AND Z. Zhou AND V. Verma AND A. Lita AND J. Shainline AND M. Stevens AND R. Mirin AND S. Nam AND M. van Exter AND M. de Dood AND A. Fiore},
	date-added = {2018-05-21 06:41:26 +0000},
	date-modified = {2018-05-22 06:42:40 +0000},
	journal = {Applied Physics Letters},
	number = {031101},
	title = {Experimental investigation of the detection mech- anism in WSi nanowire superconducting single photon detectors},
	volume = {109},
	year = {2016}}

@article{Mat15,
	author = {F. Mattioli AND Z. Zhou AND A. Gaggero AND R. Gaudio AND S. Jahanmirinejad AND D. Sahin AND F. Marsili AND R. Leoni AND A. Fiore},
	date-added = {2018-05-21 06:40:42 +0000},
	date-modified = {2018-05-21 06:41:22 +0000},
	journal = {Superconductor Science and Technology},
	number = {104001},
	title = {Photon-number-resolving superconducting nanowire detectors},
	volume = {28},
	year = {2015}}

@article{Zho14,
	author = {Z. Zhou AND S. Jahanmirinejad AND F. Mattioli AND D. Sahin AND G. Frucci AND A. Gaggero AND R. Leoni AND A. Fiore},
	date-added = {2018-05-21 06:39:16 +0000},
	date-modified = {2018-05-21 06:40:38 +0000},
	journal = {Optics Express},
	number = {3},
	pages = {3475-3489},
	title = {Superconducting series nanowire detector counting up to twelve photons},
	volume = {22},
	year = {2014}}

@article{Mar16,
	author = {F. Marsili AND M. Stevens AND A. Kozorezov AND V. Verma AND C. Lambert AND J. Stern AND R. Horansky AND S. Dyer AND S. Duff AND D. Pappas AND A. Lita AND M. Shaw AND R. Mirin AND S. Nam},
	date-added = {2018-05-21 06:37:13 +0000},
	date-modified = {2018-05-21 06:39:13 +0000},
	journal = {Physical Review B},
	number = {094518},
	title = {Hotspot relaxation dynamics in a current-carrying superconductor},
	volume = {03},
	year = {2016}}

@article{Hee12,
	author = {R. Heeres AND V. Zwiller},
	date-added = {2018-05-21 06:36:32 +0000},
	date-modified = {2018-05-21 06:37:09 +0000},
	journal = {Applied Physics Letters},
	number = {112603},
	title = {Superconducting detector dynamics studied by quantum pump-probe spec- troscopy},
	volume = {101},
	year = {2012}}

@article{Jah12,
	author = {S. Jahanmirinejad AND G. Frucci AND F. Matiioli AND D. Sahin AND A. Gaggero AND R. Leoni AND A. Fiore},
	date-added = {2018-05-19 06:44:25 +0000},
	date-modified = {2018-05-19 06:45:55 +0000},
	journal = {Applied Physics Letters},
	number = {072602},
	title = {Photon-number resolving detector based on a series array of superconducting nanowires},
	volume = {101},
	year = {2012}}

@article{Sah13,
	author = {D. Sahin AND A. Gaggero AND Z. Zhou AND S. Jahanmirinejad AND F. Mattioli AND R. Leoni AND J. Beetz AND M. Lermer AND M. Kamp AND S. Hoefling AND A. Fiore},
	date-added = {2018-05-19 06:43:14 +0000},
	date-modified = {2018-05-19 06:44:22 +0000},
	journal = {Applied Physics Letters},
	number = {111116},
	title = {Waveguide photon-number-resolving detectors for quantum photonic integrated circuits},
	volume = {103},
	year = {2013}}

@article{Gag10,
	author = {A. Gaggero AND S. Nejad AND F. Marisli AND F. Mattioli AND R. Leoni AND D. Bitauld AND D. Sahin AND G. Hamhuis AND R. Noetzel AND R. Sanjines AND A. Fiore},
	date-added = {2018-05-19 06:32:06 +0000},
	date-modified = {2018-05-19 06:42:26 +0000},
	journal = {Applied Physics Letters},
	number = {151108},
	title = {Nanowire superconducting single-photon detectors on GaAs for integrated quantum photonic applications},
	volume = {97},
	year = {2010}}

@article{Dor11,
	author = {S. Dorenbos AND P. Forn-Diaz AND T. Fuse AND A. Verbruggen AND T. Zijlstra AND T. Klapwijk AND V. Zwiller},
	date-added = {2018-05-19 06:30:22 +0000},
	date-modified = {2018-05-19 06:32:00 +0000},
	journal = {Applied Physics Letters},
	number = {251102},
	title = {Low gap superconducting single photon detectors for infrared sensitivity},
	volume = {98},
	year = {2011}}

@conference{Lit15,
	author = {A. Lita AND V. Verma AND R. Horansky AND J. Schainline AND R. Mirin AND S. Nam},
	booktitle = {Symposium VV - Science and Technology of Superconducting Materials},
	date-added = {2018-05-19 06:27:17 +0000},
	date-modified = {2018-05-19 06:30:01 +0000},
	pages = {1-6},
	series = {Material Research Series Proceedings},
	title = {Materials Development for High Efficiency Superconducting Nanowire Single-Photon Detectors},
	volume = {1807},
	year = {2015}}

@article{Eng12,
	author = {A. Engel AND A. Aeschenbacher AND K. Inderbitzin AND A. Schilling AND K. Ilin and M. Hofherr AND M. Siegel AND A. Semenov AND H.-W. Huebers},
	date-added = {2018-05-19 06:22:23 +0000},
	date-modified = {2018-05-19 06:23:56 +0000},
	journal = {Applied Physics Letters},
	number = {062601},
	title = {Tantalum nitride superconducting single-photon detectors with low cut-off energy},
	volume = {11},
	year = {2012}}

@article{Ren15,
	author = {J. Renema AND Q. Wang AND R. Gaudio AND I. Komen AND K. OptHoog AND D. Sahin AND A. Schilling AND M. van Exter AND A. Fiore AND A. Engel AND M. de Dood},
	date-added = {2018-05-19 06:15:38 +0000},
	date-modified = {2018-05-19 06:17:07 +0000},
	journal = {Nano Letters},
	number = {7},
	pages = {4541-4545},
	title = {Position-Dependent Local Detection Efficiency in a Nanowire Superconducting Single-Photon Detector},
	volume = {15},
	year = {2015}}

@article{Mar13,
	author = {F. Marsili AND V. Verma AND J. Stern AND S. Harrington AND A. Lita AND T. Gerrits AND I. Vayshenker AND B. Baek AND M. Shaw AND R. Mirin AND S. Nam},
	date-added = {2018-05-19 06:09:22 +0000},
	date-modified = {2018-05-19 06:11:30 +0000},
	journal = {Nature Photonics},
	keywords = {WSi},
	number = {201},
	title = {Detetecting single infrared photons with 93 percent system efficiency},
	volume = {7},
	year = {2013}}

@article{Geh19a,
	title={Low-loss fiber-to-chip couplers with ultrawide optical bandwidth},
	author={Gehring, H and Blaicher, M and Hartmann, W and Varytis, P and Busch, K and Wegener, M and Pernice, WHP},
	journal={APL Photonics},
	volume={4},
	number={1},
	pages={010801},
	year={2019},
	keywords = {Fiber coupling, 3D couplers},
	publisher={AIP Publishing LLC}
}

@article{Geh19b,
	title={Broadband out-of-plane coupling at visible wavelengths},
	author={Gehring, Helge and Eich, Alexander and Schuck, Carsten and Pernice, Wolfram HP},
	journal={Optics letters},
	volume={44},
	number={20},
	pages={5089--5092},
	year={2019},
	publisher={Optical Society of America},
	keywords = {Fiber coupling, 3D couplers}
}

@article{You17,
	author = {L. You AND H. Li AND W. Zhang AND X. Yang AND L. Zhang AND S. Chen AND H. Zhou AND Z. Wang AND X. Xie},
	date-added = {2018-05-18 06:30:46 +0000},
	date-modified = {2018-05-18 06:31:56 +0000},
	journal = {Superconductor Science and Technology},
	number = {8},
	title = {Superconducting nanowire single-photon detector on dielectric optical films for visible and near infrared wavelengths},
	volume = {30},
	year = {2017}}

@article{Cal17,
	author = {M. Caloz AND B. Korzh AND N. Timoney AND M. Weiss AND S. Gariglio AND R. Warburton AND C. Schoenenberger AND J. Renema AND H. Zbinden AND F. Bussieres},
	date-added = {2018-05-18 06:20:35 +0000},
	date-modified = {2018-05-18 06:22:15 +0000},
	journal = {Applied Physics Letters},
	number = {083106},
	title = {Optically probing the detection mechanism in a molybdenum silicide superconducting nanowire single-photon detector},
	volume = {110},
	year = {2017}
}

@article{Ver15,
	author = {V. Verma AND B. Korzh AND F. Bussieres, R. Horansky AND S. Dyer AND A. Lita AND I. Vayshenker AND F. Marsili AND M. Shaw AND H. Zbinden AND R. Mirin AND S. Nam},
	date-added = {2018-05-18 06:17:40 +0000},
	date-modified = {2018-05-18 06:20:31 +0000},
	journal = {Optics Express},
	number = {26},
	pages = {33792-33801},
	title = {High-efficiency superconducting nanowire single-photon detectors fabricated from MoSi thin-films},
	volume = {23},
	year = {2015}}

@article{Kor14,
	author = {Y. Korneeva AND M. Mikhailov AND Y. Pershin AND N. Manova AND A. Divochiy AND Y. Vakhtomin AND A. Korneev AND K. Smirnov AND A. Sivakov AND A. Devizenko AND G. Goltsman},
	date-added = {2018-05-18 06:16:24 +0000},
	date-modified = {2018-05-18 06:17:32 +0000},
	journal = {Superconductor Science and Technology},
	number = {095012},
	title = {Superconducting single-photon detector made of MoSi film},
	volume = {27},
	year = {2014}}

@article{Ver14,
	author = {V. Verma AND A. Lita AND M. Vissers AND F. Marsili AND D. Pappas AND R. Mirin AND S. Nam},
	date-added = {2018-05-18 06:12:58 +0000},
	date-modified = {2018-05-18 06:14:57 +0000},
	journal = {Applied Physics Letters},
	keywords = {MoGe},
	number = {022602},
	title = {Superconducting nanowire single photon detectors fabricated from an amorphous Mo0.75Ge0.25 thin film},
	volume = {105},
	year = {2014}}

@article{Cal18,
	author = {M. Caloz AND M. Perrenoud AND C. Autebert AND B. Korzh AND C. Schoenenberger AND R. Warburton AND H. Zbinden AND F. Bussieres},
	date-added = {2018-05-18 06:11:39 +0000},
	date-modified = {2018-05-18 06:35:18 +0000},
	journal = {Applied Physics Letters},
	keywords = {MoSi},
	number = {061103},
	title = {High-detection efficiency and low-timing jitter with amorphous superconducting nanowire single-photon detectors},
	volume = {112},
	year = {2018}}

@article{Che13,
	author = {R. Cheng AND H. Yin AND J. Liu AND T. Li AND H. Cai AND Z. Xu AND W, Chen},
	date-added = {2018-05-18 06:09:10 +0000},
	date-modified = {2018-05-18 06:10:52 +0000},
	journal = {IEEE Transactions on Applied Superconductivity},
	keywords = {Theory},
	number = {1},
	title = {Photon-Number-Resolving Detector Based on Superconducting Serial Nanowires},
	volume = {23},
	year = {2013}}

@article{Hee10,
	author = {R. Heeres AND S. Dorenbos AND B. Koene AND G. Solomon AND L. Kouwenhoven AND V. Zwiller},
	date-added = {2018-05-16 22:06:17 +0000},
	date-modified = {2018-05-16 22:07:04 +0000},
	journal = {Nano Letters},
	pages = {661-664},
	title = {On-Chip Single Plasmon Detection},
	volume = {10},
	year = {2010}}

@article{Ros10,
	author = {M. Rosticher AND F. Ladan AND J. Maneval AND S. Dorenbos AND T. Zijlstra AND T. Klapwijk AND V. Zwiller AND A. Lupacu AND G. Nogues},
	date-added = {2018-05-16 22:05:40 +0000},
	date-modified = {2018-05-16 22:06:13 +0000},
	journal = {Applied Physics Letters},
	title = {A high efficiency superconducting nanowire single electron detector},
	volume = {97},
	year = {2010}}

@article{Hec67,
	author = {K. Hechler AND E. Saur AND H. Wizgall},
	date-added = {2018-05-16 22:04:50 +0000},
	date-modified = {2018-05-16 22:05:37 +0000},
	journal = {Zeitschrift f{\"u}r Physik},
	pages = {400-408},
	title = {Critical Data of Niobium Nitride in Transverse Magnetic Fields},
	volume = {205},
	year = {1967}}

@article{Yam72,
	author = {T. Yamashita AND S. Kitahara AND Y. Onodera},
	date-added = {2018-05-16 22:04:13 +0000},
	date-modified = {2018-05-16 22:04:46 +0000},
	journal = {Journal of Applied Physics},
	number = {11},
	title = {Upper critical field of superconducting NbN films},
	volume = {43},
	year = {1972}}

@article{Suz87,
	author = {M. Suzuki AND M. Baba AND T. Anayama},
	date-added = {2018-05-16 22:03:25 +0000},
	date-modified = {2018-05-16 22:04:05 +0000},
	journal = {Japanase Journal of Applied Physics},
	title = {Critical Magnetic Field of Superconducting NbN Films Prepared by Reactive Sputtering},
	volume = {26},
	year = {1987}}

@article{Ros08,
	author = {E. Rosa},
	date-added = {2018-05-16 22:02:34 +0000},
	date-modified = {2018-05-16 22:03:18 +0000},
	journal = {Bulletin of the Bureau of Standards},
	number = {2},
	pages = {301ff},
	title = {The Self and Mutual Inductances of Linear Conductors},
	volume = {4},
	year = {1908}}

@article{Fin10,
	author = {C. Finlay AND S. Maus AND C. Beggan AND T. Bondar AND A. Chambodut AND T. Chernova AND A. Chulliat AND V. Golovkov AND B. Hamilton AND M. Hamoudi AND R. HolmeAND G. Hulot AND W. Kuang AND B. Langlais AND V. Lesur AND F. Lowes AND H. L{\"u}hr AND S. Macmillan AND M. Mandea AND S. McLean AND C. Manoj AND M. Menvielle AND I. Michaelis AND N. Olsen AND J. Rauberg AND M. Rother AND T. Sabaka AND A. Tangborn AND L. Toeffner-Clausen AND E. Thebault AND A. Thomson AND I. Wardinski AND Z. Wei AND T. Zvereva},
	date-added = {2018-05-16 22:01:23 +0000},
	date-modified = {2018-05-16 22:02:30 +0000},
	journal = {Geophysical Journal International},
	month = {Dezember},
	number = {3},
	pages = {1216-1230},
	title = {International Geomagnetic Reference Field: the eleventh generation},
	volume = {183},
	year = {2010}}

@article{Hor12,
	author = {H. Hortensius AND E. Driessen AND T. Klapwijk AND K. Berggreen},
	date-added = {2018-05-13 17:31:25 +0000},
	date-modified = {2018-05-13 17:33:12 +0000},
	journal = {Applied Physics Letters},
	number = {182602},
	title = {Critical-Current Reduction in Thin Superconducting Wires Due to Current Crowding},
	volume = {100},
	year = {2012}}

@article{Yan09,
	author = {Z. Yan AND A. Majedi},
	date-added = {2018-05-13 09:16:09 +0000},
	date-modified = {2018-05-13 09:16:49 +0000},
	journal = {IEEE Transactions on Applied Superconductivity},
	month = {Oktober},
	number = {5},
	title = {Experimental Investigations on Nonlinear Properties of Superconducting Nanowire Meanderline in RF and Microwave Frequencies},
	volume = {19},
	year = {2009}}

@article{Won93,
	author = {M. Wong AND W. Sproul AND X. Chu AND S. Barnett},
	date-added = {2018-05-13 09:15:10 +0000},
	date-modified = {2018-05-13 09:16:07 +0000},
	journal = {Journal of Vacuum Science Tech- nology A: Vacuum, Surfaces, and Films},
	number = {1528-1533},
	title = {Reactive magnetron sputter depositionof niobium nitride films},
	volume = {11},
	year = {1993}}

@book{Jou16,
	author = {K. Jousten},
	date-added = {2018-05-13 09:14:31 +0000},
	date-modified = {2018-05-13 09:15:05 +0000},
	publisher = {Wiley-VCH},
	title = {Handbook of Vacuum Technology},
	year = {2016}}

@article{Ili05,
	author = {K. Ilin AND M. Siegel AND A. Semenov AND A. Engel AND H.-W. H{\"u}bers},
	date-added = {2018-05-10 17:42:30 +0000},
	date-modified = {2018-05-10 17:43:36 +0000},
	journal = {Physica Status Solidi (c)},
	number = {5},
	pages = {1680-1687},
	title = {Critical current of Nb and NbN thin film structures: The cross-section dependence},
	volume = {2},
	year = {2005}}

@article{Kam10,
	author = {A. Kamlapure AND M. Mondal AND M. Chand AND A. Mishra AND J. Jesudasan AND V. Bagwe AND L. Befatto AND V. Tripathi AND P. Raychaudhuri},
	date-added = {2018-05-09 22:28:04 +0000},
	date-modified = {2018-05-09 22:29:48 +0000},
	journal = {Applied Physics Letters},
	number = {072509},
	title = {Measurement of magnetic penetration depth and superconducting energy gap in very thin NbN films},
	volume = {96},
	year = {2010}}

@article{Ros13,
	author = {D. Rosenberg AND A. Kerman AND R. Molnar AND E. Dauler},
	date-added = {2018-05-09 14:30:56 +0000},
	date-modified = {2018-05-09 14:31:37 +0000},
	journal = {Optics express},
	number = {2},
	pages = {1440-1447},
	title = {High-speed and high-efficiency superconducting nanowire single photon detector array},
	volume = {21},
	year = {2013}}

@article{Yan17,
	title={Comparison of superconducting nanowire single-photon detectors made of NbTiN and NbN thin films},
	author={Yang, Xiaoyan and You, Lixing and Zhang, Lu and Lv, Chaolin and Li, Hao and Liu, Xiaoyu and Zhou, Hui and Wang, Zhen},
	journal={IEEE Transactions on Applied Superconductivity},
	volume={28},
	number={1},
	pages={1--6},
	year={2017},
	publisher={IEEE}
}

@article{You13,
	author = {L. You AND X. Yang AND Y. He AND W. Zhang AND D. Liu AND W. Zhang AND L. Zhang AND L. Zhang AND X. Liu AND S. Chen AND Z. Wang AND X. Xie},
	date-added = {2018-05-09 14:10:30 +0000},
	date-modified = {2018-05-09 14:13:43 +0000},
	journal = {AIP Advances},
	number = {072135},
	title = {Jitter analysis of a superconducting nanowire single photon detector},
	volume = {3},
	pages={072135},
	year = {2013}}

@article{Ker06,
	title={Kinetic-inductance-limited reset time of superconducting nanowire photon counters},
	author={Kerman, Andrew J and Dauler, Eric A and Keicher, William E and Yang, Joel KW and Berggren, Karl K and Gol’Tsman, G and Voronov, B},
	journal={Applied physics letters},
	volume={88},
	number={11},
	pages={111116},
	year={2006},
	publisher={American Institute of Physics}
}

@article{Ker07,
	title={Constriction-limited detection efficiency of superconducting nanowire single-photon detectors},
	author={Kerman, Andrew J and Dauler, Eric A and Yang, Joel KW and Rosfjord, Kristine M and Anant, Vikas and Berggren, Karl K and Gol’tsman, Gregory N and Voronov, Boris M},
	journal={Applied Physics Letters},
	volume={90},
	number={10},
	pages={101110},
	year={2007},
	publisher={American Institute of Physics}
}

@phdthesis{Kit08,
	author = {J. Kitaygorsky},
	date-added = {2018-05-07 15:25:20 +0000},
	date-modified = {2018-05-07 15:26:25 +0000},
	school = {University of Rochester},
	title = {Photon and Dark Counts in NbN Superconducting Single-Photon Detectors and Nanostripes},
	year = {2008}}

@article{Wan17,
	author = {Q. Wang AND J. Renema AND A. Engel AND M. de Dood},
	date-added = {2018-05-06 15:33:33 +0000},
	date-modified = {2018-05-06 15:34:49 +0000},
	journal = {Physical Review Applied},
	keywords = {Width},
	month = {September},
	number = {034004},
	title = {Design of NbN Superconducting Nanowire Single-Photon Detectors with Enhanced Infrared Detection Efficiency},
	volume = {8},
	year = {2017}}

@article{Ren17,
	author = {J.J. Renema AND Q. Wang AND M.P. van Exter AND M.J.A. de Dood},
	date-added = {2018-04-30 15:10:39 +0000},
	date-modified = {2018-04-30 15:12:11 +0000},
	journal = {Applied Physics Letters},
	number = {233103},
	title = {Probing the Hotspot Interaction Length in NbN Nanowire Superconducting Single Photon Detectors},
	volume = {110},
	year = {2017}}

@article{Zha18,
	author = {L. Zhang AND L. You AND X. Yang AND J. Wu AND C. Lv AND Q. Guo AND W. Zhang AND H. Li AND W. Peng AND Z. Wang AND X. Xie},
	date-added = {2018-04-30 15:05:20 +0000},
	date-modified = {2018-04-30 15:08:59 +0000},
	journal = {Scientific Reports},
	keywords = {Hotspot Relaxation},
	month = {Januar},
	number = {1486},
	title = {Hotspot relaxation time of NbN superconducting nanowire single-photon detectors on various substrates},
	volume = {8},
	year = {2018}}

@article{Ana08,
	author = {V. Anant AND A. J. Kerman AND E. A. Dauler AND J. K. W. Yang AND K. M. Rosfjord AND K. K. Berggren},
	date-added = {2017-01-01 00:20:54 +0000},
	date-modified = {2017-01-01 00:23:25 +0000},
	journal = {Optics express},
	keywords = {Cavity},
	number = {14},
	pages = {10750-10761},
	title = {Optical properties of superconducting nanowire single-photon detectors},
	volume = {16},
	year = {2008}}

@article{Rei13,
	title={Optimisation of NbN thin films on GaAs substrates for in-situ single photon detection in structured photonic devices},
	author={Reithmaier, G{\"u}nther and Senf, J{\"o}rg and Lichtmannecker, Stefan and Reichert, Thorsten and Flassig, Fabian and Voss, Andrej and Gross, Rudolf and Finley, JJ},
	journal={Journal of Applied Physics},
	volume={113},
	number={14},
	pages={143507},
	year={2013},
	publisher={American Institute of Physics}
}

@article{Sun15,
	author = {K. A. Sunter AND A. E. Dane AND C. I. Lang AND K. K. Berggren},
	date-added = {2018-04-25 08:57:54 +0000},
	date-modified = {2018-04-25 08:58:36 +0000},
	journal = {Applied Optics},
	number = {18},
	pages = {5743-5749},
	title = {Infrared transmissometer to measure the thickness of NbN thin films},
	volume = {54},
	year = {2015}}

@article{Yam10,
	author = {T. Yamashita AND S. Miki AND W. Qiu AND M. Fujiwara AND M. Sasaki AND Z. Wang},
	date-added = {2018-04-25 08:52:06 +0000},
	date-modified = {2018-04-25 08:53:22 +0000},
	journal = {Applied Physics Express},
	number = {102502},
	title = {Temperature Dependent Performances of Superconducting Nanowire Single-Photon Detectors in an Ultralow-Temperature Region},
	volume = {3},
	year = {2010}}

@article{Mai10,
	author = {L. Maingault AND M. Tarkhov AND I. Florya AND A. Semenov AND R. E. de Lamaestre AND P. Cavalier AND G. Goltsman AND J.-P. Poizat AND J.-C. Villegier},
	date-added = {2018-04-23 11:56:09 +0000},
	date-modified = {2018-04-23 11:58:34 +0000},
	journal = {Journal of Applied Physics},
	title = {Spectral dependency of superconducting single photon detectors},
	volume = {116103},
	year = {2010}}

@article{Kad96,
	author = {A. M. Kadin AND M. W. Johnson},
	date-added = {2018-04-23 11:54:53 +0000},
	date-modified = {2018-04-23 11:55:32 +0000},
	journal = {Applied Physics Letters},
	title = {Nonequilibrium photon-induced hotspot: A new mechanism for photodetection in ultrathin metallic films},
	volume = {3938-3940},
	year = {1996}}

@article{Bar57a,
	title={Microscopic theory of superconductivity},
	author = {J. Bardeen AND L. Cooper AND J. Schrieffer},
	journal={Physical Review},
	volume={106},
	number={1},
	pages={162},
	year={1957},
	publisher={APS}
}

@article{Bar57b,
	author = {J. Bardeen AND L. Cooper AND J. Schrieffer},
	date-added = {2018-04-23 11:52:32 +0000},
	date-modified = {2022-03-17 13:00:41 +0100},
	journal = {Physical Review},
	keywords = {Superconductivity},
	number = {1175},
	title = {Theory of superconductivity},
	volume = {108},
	year = {1957}}

@article{Tes71,
	author = {L. R. Testardi},
	date-added = {2018-04-23 11:50:29 +0000},
	date-modified = {2018-04-23 11:51:12 +0000},
	journal = {Physical Review B},
	number = {2189-96},
	title = {Destruction of superconductivity by laser light},
	volume = {4},
	year = {1971}}

@article{Ili08,
	author = {K. Ilin AND R. Schneider AND D. Gerthsen AND A. Engel AND H. Bartolf AND A. Schilling AND A. Semenov AND H.-W. Huebers and B. Freitag},
	date-added = {2018-04-19 13:39:42 +0000},
	date-modified = {2022-03-17 09:38:18 +0100},
	title = {Ultra-thin NbN films on Si: Crystalline and superconducting properties},
	year = {2008}}

@article{Sem09,
	author = {A. Semenov AND B. G{\"u}nther AND U. B{\"o}ttger AND H.-W. H{\"u}bers AND H. Bartolf AND A. Engel AND A. Schilling AND K. Ilin AND M. Siegel AND R. Schneider AND D. Gerthsen AND N. A. Gippius},
	date-added = {2018-04-19 13:34:25 +0000},
	date-modified = {2018-04-19 13:36:39 +0000},
	journal = {Physical Review B},
	keywords = {NbN},
	number = {054510},
	title = {Optical and transport porperties of ultrathin NbN films and nanostructures},
	volume = {80},
	pages={054510},
	year = {2009}}

@article{Vya02,
	author = {Vladimir L. Vyazovkin AND Valery V. Korolev AND Vladimir M. Syutkin AND Vladimir A. Tolkatchev},
	date-added = {2018-04-19 11:04:59 +0000},
	date-modified = {2018-04-19 11:06:43 +0000},
	journal = {React.Kinet.Catal.Lett.},
	keywords = {PMMA Oxygen DiffusionS},
	month = {July},
	number = {2},
	pages = {293-299},
	title = {On oxygen diffusion in poly(methyl methacrylate) films},
	volume = {77},
	year = {2002}}

@article{Cha17,
	author = {L.S. Sharath Chandra AND R. Mondal AND A. Thamizhavel AND S.K. Dhar AND S.B. Roy},
	date-added = {2018-04-16 15:36:22 +0000},
	date-modified = {2018-04-16 15:37:56 +0000},
	journal = {Physica B},
	number = {175-177},
	title = {A revisit to the temperature dependence of electrical resistivity of Titanium at low temperatures},
	volume = {521},
	year = {2017}}

@article{Rei86,
	author = {G. Reiss AND J. Vancea AND H. Hoffmann},
	date-added = {2018-04-16 14:09:26 +0000},
	date-modified = {2018-04-16 14:28:12 +0000},
	journal = {Physical Review Letters},
	keywords = {Theory},
	number = {2100-2103},
	title = {Grain-Boundary Resistance in Polycrystalline Metals},
	volume = {56},
	year = {1986}}

@article{Kai02,
	author = {N. Kaiser},
	date-added = {2018-04-16 13:26:43 +0000},
	date-modified = {2018-04-16 13:28:42 +0000},
	journal = {Applied Optics},
	number = {3053-3060},
	title = {Review of the fundamentals of thinfilm growth},
	volume = {41},
	year = {2002}}

@article{Bur86,
	author = {Michael C. Burrel AND Neal R. Armstrong},
	date-added = {2018-04-13 13:43:47 +0000},
	date-modified = {2018-04-13 13:45:37 +0000},
	journal = {Langmuir},
	pages = {30-36},
	title = {Formed on Polycrystalline Titanium Thin-Film Formed at Low and High O2 Partial Pressures Surfaces: Rates of Formation and Composition of Oxides},
	volume = {2},
	year = {1986}}

@article{Wei52,
	author = {Lazarus Weiner AND Premo Chiotti AND H.A. Wilhelm},
	date-added = {2018-04-13 13:31:51 +0000},
	date-modified = {2018-04-13 13:33:25 +0000},
	journal = {Ames Laboratory ISC Technical Reports},
	title = {Temperature Dependence of Electrical Resistivity of Metals},
	volume = {58},
	year = {1952}}

@book{Sch98,
	author = {Dieter K. Schroder},
	date-added = {2018-04-13 13:17:57 +0000},
	date-modified = {2018-04-13 13:29:57 +0000},
	number = {pp. 1-55},
	publisher = {New York: J Wiley \& Sons},
	title = {Semiconductor Material and Device Characterization},
	year = {1998}}

@article{Yan07,
	author = {J. Yang AND A. Kerman AND E. Dauler AND V. Anant AND K. Rosfjord AND K. Berggren},
	date-added = {2018-03-01 13:56:59 +0000},
	date-modified = {2018-03-01 13:58:41 +0000},
	journal = {IEEE Transactions on Applied Superconductivity},
	pages = {581-585},
	title = {Modeling the Electrical and Thermal Response of Superconducting Nanowire Single-Photon Detectors},
	volume = {17},
	year = {2007}}

@article{Gol05,
	author = {G. N. Gol'tsman AND A. Korneev AND I. Rubstova AND I. Milostnaya AND G. Chulkova AND O. Minaeva AND K. Smirnov AND B. Voronov AND W. Sysz AND A. Pearlman AND A. Verevkin AND R. Sobolewski},
	date-added = {2018-03-01 11:51:34 +0000},
	date-modified = {2018-03-01 11:58:56 +0000},
	journal = {Physica Status Solidi (c)},
	number = {1480-1488},
	title = {Ultrafast superconducting single-photon detectors for near-infrared-wavelength quantum communications},
	volume = {2},
	year = {2005},
	Bdsk-File-1 = {YnBsaXN0MDDSAQIDBFxyZWxhdGl2ZVBhdGhZYWxpYXNEYXRhXxAfLi4vLi4vRG93bmxvYWRzL3lhbmctMS0yMDA3LnBkZk8RAXAAAAAAAXAAAgAABk1hY05ldQAAAAAAAAAAAAAAAAAAAAAAAAAAANU90x5IKwAAAAT5XQ95YW5nLTEtMjAwNy5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAH+Dx1r2x4AAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAJRG93bmxvYWRzAAAQAAgAANU9tv4AAAARAAgAANa9o9AAAAABAAwABPldAAT5WgACEnoAAgAwTWFjTmV1OlVzZXJzOgBSYXNtdXM6AERvd25sb2FkczoAeWFuZy0xLTIwMDcucGRmAA4AIAAPAHkAYQBuAGcALQAxAC0AMgAwADAANwAuAHAAZABmAA8ADgAGAE0AYQBjAE4AZQB1ABIAJlVzZXJzL1Jhc211cy9Eb3dubG9hZHMveWFuZy0xLTIwMDcucGRmABMAAS8AABUAAgAN//8AAAAIAA0AGgAkAEYAAAAAAAACAQAAAAAAAAAFAAAAAAAAAAAAAAAAAAABug==}}

@article{Ili98,
	author = {K. S. Ilis AND I. I. Milostnaya AND A. A. Verevkin AND G. N. Gol'tsman AND E. M. Gershenzon AND R. Sobolewski},
	date-added = {2018-03-01 11:43:32 +0000},
	date-modified = {2018-03-01 11:51:21 +0000},
	journal = {Applied Physics Letters},
	pages = {3938-3940},
	title = {Ultimate quantum efficiency of a superconducting hot-electron photodetector},
	volume = {73},
	year = {1998}}

@book{Fli10,
	author = {Torsten Flie{\ss}bach},
	date-added = {2018-02-15 16:13:38 +0000},
	date-modified = {2018-02-15 16:26:04 +0000},
	publisher = {Spektrum Akademischer Verlag},
	read = {0},
	title = {Statistische Physik Lehrbuch zur Theoretischen Physik IV},
	year = {2010}}

@article{Jou52,
	author = {J.P. Joule and W. Thomson},
	date-added = {2018-01-04 20:10:58 +0000},
	date-modified = {2018-01-04 20:16:22 +0000},
	journal = {Philosophical Magazine},
	number = {4},
	pages = {481-492},
	title = {On the thermal effects experienced by air in rushing through small apertures},
	volume = {4},
	year = {1852}}

@article{Hen72,
	author = {Robert C. Hendricks and Ildiko C. Peller and Anne K. Baron},
	date-added = {2018-01-04 19:52:26 +0000},
	date-modified = {2018-01-04 19:59:23 +0000},
	journal = {Nasa Technical note},
	keywords = {THERMODYNAMICS AND COMBUSTION},
	month = {July},
	pages = {60},
	title = {Joule-Thomson inversion curves and related coefficients for several simple fluids},
	volume = {D-6807},
	year = {1972},
	Bdsk-File-1 = {YnBsaXN0MDDSAQIDBFxyZWxhdGl2ZVBhdGhZYWxpYXNEYXRhXxAfLi4vLi4vRG93bmxvYWRzLzE5NzIwMDIwMzE1LnBkZk8RAXAAAAAAAXAAAgAABk1hY05ldQAAAAAAAAAAAAAAAAAAAAAAAAAAANU90x5IKwAAAAT5XQ8xOTcyMDAyMDMxNS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAG25u1nQ/JQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAJRG93bmxvYWRzAAAQAAgAANU9tv4AAAARAAgAANZ0MRUAAAABAAwABPldAAT5WgACEnoAAgAwTWFjTmV1OlVzZXJzOgBSYXNtdXM6AERvd25sb2FkczoAMTk3MjAwMjAzMTUucGRmAA4AIAAPADEAOQA3ADIAMAAwADIAMAAzADEANQAuAHAAZABmAA8ADgAGAE0AYQBjAE4AZQB1ABIAJlVzZXJzL1Jhc211cy9Eb3dubG9hZHMvMTk3MjAwMjAzMTUucGRmABMAAS8AABUAAgAN//8AAAAIAA0AGgAkAEYAAAAAAAACAQAAAAAAAAAFAAAAAAAAAAAAAAAAAAABug==}}

@article{Nat12,
	author = {Chandra M. Natarjan and Michael G. Tanner and Robert H. Hadfield},
	date-added = {2017-09-17 14:05:22 +0000},
	date-modified = {2017-09-17 14:31:13 +0000},
	doi = {10.1088/0953-2048/25/6/063001},
	journal = {Superconductor Science and Technology},
	pages = {063001},
	read = {0},
	title = {Superconducting nanowire single-photon detectors: physics and apllications},
	url = {https://arxiv.org/abs/1204.5560},
	volume = {25},
	year = {2012},
	Bdsk-Url-1 = {https://arxiv.org/abs/1204.5560},
	Bdsk-Url-2 = {http://dx.doi.org/10.1088/0953-2048/25/6/063001}}

@article{Biagioni2012,
	abstract = {Nanoantennas for visible and infrared radiation can strongly enhance the interaction of light with nanoscale matter by their ability to efficiently link propagating and spatially localized optical fields. This ability unlocks an enormous potential for applications ranging from nanoscale optical microscopy and spectroscopy over solar energy conversion, integrated optical nanocircuitry, opto-electronics and density-of-states engineering to ultra-sensing as well as enhancement of optical nonlinearities. Here we review the current understanding of metallic optical antennas based on the background of both well-developed radiowave antenna engineering and plasmonics. In particular, we discuss the role of plasmonic resonances on the performance of nanoantennas and address the influence of geometrical parameters imposed by nanofabrication. Finally, we give a brief account of the current status of the field and the major established and emerging lines of investigation in this vivid area of research.},
	author = {Biagioni, Paolo and Huang, Jer-Shing and Hecht, Bert},
	doi = {10.1088/0034-4885/75/2/024402},
	file = {:C$\backslash$:/Users/sebastian.hammer/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Biagioni, Huang, Hecht - 2012 - Nanoantennas for visible and infrared radiation.pdf:pdf},
	issn = {1361-6633},
	journal = {Reports on progress in physics. Physical Society (Great Britain)},
	month = feb,
	number = {2},
	pages = {024402},
	title = {{Nanoantennas for visible and infrared radiation.}},
	url = {http://www.ncbi.nlm.nih.gov/pubmed/22790344},
	volume = {75},
	year = {2012},
	Bdsk-Url-1 = {http://www.ncbi.nlm.nih.gov/pubmed/22790344},
	Bdsk-Url-2 = {http://dx.doi.org/10.1088/0034-4885/75/2/024402}}

@article{Bracher2011,
	author = {Bracher, G. and Schraml, K. and Jakubeit, C. and Kaniber, M. and Finley, J. J.},
	doi = {10.1063/1.3671641},
	file = {:C$\backslash$:/Users/sebastian.hammer/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Bracher et al. - 2011 - Direct measurement of plasmon propagation lengths on lithographically defined metallic waveguides on GaAs.pdf:pdf},
	issn = {00218979},
	journal = {Journal of Applied Physics},
	number = {12},
	pages = {123106},
	title = {{Direct measurement of plasmon propagation lengths on lithographically defined metallic waveguides on GaAs}},
	url = {http://link.aip.org/link/JAPIAU/v110/i12/p123106/s1\&Agg=doi},
	volume = {110},
	year = {2011},
	Bdsk-Url-1 = {http://link.aip.org/link/JAPIAU/v110/i12/p123106/s1%5C&Agg=doi},
	Bdsk-Url-2 = {http://dx.doi.org/10.1063/1.3671641}}

@article{Chen2003,
	author = {Chen, G. and Hui, P. and Pita, K. and Hing, P. and Kong, L.},
	doi = {10.1007/s00339-003-2321-3},
	file = {:C$\backslash$:/Users/sebastian.hammer/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Chen et al. - 2003 - Conductivity drop and crystallites redistribution in gold film.pdf:pdf},
	issn = {0947-8396},
	journal = {Applied Physics A},
	month = sep,
	number = {3},
	pages = {659--665},
	title = {{Conductivity drop and crystallites redistribution in gold film}},
	url = {http://link.springer.com/10.1007/s00339-003-2321-3},
	volume = {80},
	year = {2003},
	Bdsk-Url-1 = {http://link.springer.com/10.1007/s00339-003-2321-3},
	Bdsk-Url-2 = {http://dx.doi.org/10.1007/s00339-003-2321-3}}

@article{Chen1999,
	author = {Chen, George and Hui, Ping},
	doi = {10.1063/1.123973},
	file = {:C$\backslash$:/Users/sebastian.hammer/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Chen, Hui - 1999 - Thermal conductivities of evaporated gold films on silicon and glass.pdf:pdf},
	issn = {00036951},
	journal = {Applied Physics Letters},
	number = {20},
	pages = {2942},
	title = {{Thermal conductivities of evaporated gold films on silicon and glass}},
	url = {http://scitation.aip.org/content/aip/journal/apl/74/20/10.1063/1.123973},
	volume = {74},
	year = {1999},
	Bdsk-Url-1 = {http://scitation.aip.org/content/aip/journal/apl/74/20/10.1063/1.123973},
	Bdsk-Url-2 = {http://dx.doi.org/10.1063/1.123973}}

@article{Chen2010,
	abstract = {The effect of grain boundaries on the electron relaxation rate is significant even for large area noble metal films and more so for plasmonic nanostructures. Optical spectroscopy and X-ray diffraction show a substantial improvement in plasmon resonance quality for square-particle nanoantennas after annealing due to an enlarged grain size from 22 to 40 nm and improved grain boundaries described by the electron reflection coefficient. The electron relaxation rate due to the grains is shown to decrease by a factor of 3.2.},
	author = {Chen, Kuo-Ping and Drachev, Vladimir P and Borneman, Joshua D and Kildishev, Alexander V and Shalaev, Vladimir M},
	doi = {10.1021/nl9037246},
	file = {:C$\backslash$:/Users/sebastian.hammer/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Chen et al. - 2010 - Drude relaxation rate in grained gold nanoantennas.pdf:pdf},
	issn = {1530-6992},
	journal = {Nano letters},
	keywords = {Crystallization,Crystallization: methods,Gold,Gold: chemistry,Materials Testing,Nanostructures,Nanostructures: chemistry,Nanostructures: ultrastructure,Nanotechnology,Nanotechnology: methods,Particle Size,Surface Plasmon Resonance,Surface Plasmon Resonance: methods},
	month = mar,
	number = {3},
	pages = {916--22},
	pmid = {20128610},
	title = {{Drude relaxation rate in grained gold nanoantennas.}},
	url = {http://www.ncbi.nlm.nih.gov/pubmed/20128610},
	volume = {10},
	year = {2010},
	Bdsk-Url-1 = {http://www.ncbi.nlm.nih.gov/pubmed/20128610},
	Bdsk-Url-2 = {http://dx.doi.org/10.1021/nl9037246}}

@article{Ditlbacher2005,
	author = {Ditlbacher, Harald and Hohenau, Andreas and Wagner, Dieter and Kreibig, Uwe and Rogers, Michael and Hofer, Ferdinand and Aussenegg, Franz and Krenn, Joachim},
	doi = {10.1103/PhysRevLett.95.257403},
	file = {:C$\backslash$:/Users/sebastian.hammer/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Ditlbacher et al. - 2005 - Silver Nanowires as Surface Plasmon Resonators.pdf:pdf},
	issn = {0031-9007},
	journal = {Physical Review Letters},
	month = dec,
	number = {25},
	pages = {257403},
	title = {{Silver Nanowires as Surface Plasmon Resonators}},
	url = {http://link.aps.org/doi/10.1103/PhysRevLett.95.257403},
	volume = {95},
	year = {2005},
	Bdsk-Url-1 = {http://link.aps.org/doi/10.1103/PhysRevLett.95.257403},
	Bdsk-Url-2 = {http://dx.doi.org/10.1103/PhysRevLett.95.257403}}

@article{Gramotnev2013,
	author = {Gramotnev, Dmitri K. and Bozhevolnyi, Sergey I.},
	doi = {10.1038/nphoton.2013.232},
	file = {:C$\backslash$:/Users/sebastian.hammer/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Gramotnev, Bozhevolnyi - 2013 - Nanofocusing of electromagnetic radiation.pdf:pdf},
	issn = {1749-4885},
	journal = {Nature Photonics},
	month = dec,
	number = {1},
	pages = {13--22},
	publisher = {Nature Publishing Group},
	title = {{Nanofocusing of electromagnetic radiation}},
	url = {http://www.nature.com/doifinder/10.1038/nphoton.2013.232},
	volume = {8},
	year = {2013},
	Bdsk-Url-1 = {http://www.nature.com/doifinder/10.1038/nphoton.2013.232},
	Bdsk-Url-2 = {http://dx.doi.org/10.1038/nphoton.2013.232}}

@article{Gramotnev2010,
	author = {Gramotnev, Dmitri K. and Bozhevolnyi, Sergey I.},
	doi = {10.1038/nphoton.2009.282},
	file = {:C$\backslash$:/Users/sebastian.hammer/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Gramotnev, Bozhevolnyi - 2010 - Plasmonics beyond the diffraction limit.pdf:pdf},
	issn = {1749-4885},
	journal = {Nature Photonics},
	month = jan,
	number = {2},
	pages = {83--91},
	publisher = {Nature Publishing Group},
	title = {{Plasmonics beyond the diffraction limit}},
	url = {http://www.nature.com/doifinder/10.1038/nphoton.2009.282},
	volume = {4},
	year = {2010},
	Bdsk-Url-1 = {http://www.nature.com/doifinder/10.1038/nphoton.2009.282},
	Bdsk-Url-2 = {http://dx.doi.org/10.1038/nphoton.2009.282}}

@article{Gruber2013,
	author = {Gruber, Christian and Tr\"{u}gler, Andreas and Hohenau, Andreas and Hohenester, Ulrich and Krenn, Joachim R.},
	file = {:C$\backslash$:/Users/sebastian.hammer/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Gruber et al. - 2013 - Spectral Modifications and Polarization Dependent Coupling in Tailored Assemblies of Quantum Dots and Plasmonic N.pdf:pdf},
	keywords = {coupling,critically on the understanding,electron beam lithography,emitters to their environment,he ability to control,local density of states,matter structured on the,nanowire,of the coupling of,plasmonics,quantum dots,single photon emission depends,the},
	pages = {4257--4262},
	title = {{Spectral Modifications and Polarization Dependent Coupling in Tailored Assemblies of Quantum Dots and Plasmonic Nanowires}},
	volume = {13},
	year = {2013}}

@article{Hill2007,
	author = {Hill, Martin T. and Oei, Yok-Siang and Smalbrugge, Barry and Zhu, Youcai and de Vries, Tjibbe and van Veldhoven, Peter J. and van Otten, Frank W. M. and Eijkemans, Tom J. and Turkiewicz, Jaros{\l}aw P. and de Waardt, Huug and Geluk, Erik Jan and Kwon, Soon-Hong and Lee, Yong-Hee and N\"{o}tzel, Richard and Smit, Meint K.},
	doi = {10.1038/nphoton.2007.171},
	file = {:C$\backslash$:/Users/sebastian.hammer/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Hill et al. - 2007 - Lasing in metallic-coated nanocavities.pdf:pdf},
	issn = {1749-4885},
	journal = {Nature Photonics},
	month = sep,
	number = {10},
	pages = {589--594},
	title = {{Lasing in metallic-coated nanocavities}},
	url = {http://www.nature.com/doifinder/10.1038/nphoton.2007.171},
	volume = {1},
	year = {2007},
	Bdsk-Url-1 = {http://www.nature.com/doifinder/10.1038/nphoton.2007.171},
	Bdsk-Url-2 = {http://dx.doi.org/10.1038/nphoton.2007.171}}

@article{Hua10,
	abstract = {Deep subwavelength integration of high-definition plasmonic nanostructures is of key importance in the development of future optical nanocircuitry for high-speed communication, quantum computation and lab-on-a-chip applications. To date, the experimental realization of proposed extended plasmonic networks consisting of multiple functional elements remains challenging, mainly because of the multi-crystallinity of commonly used thermally evaporated gold layers. This can produce structural imperfections in individual circuit elements that drastically reduce the yield of functional integrated nanocircuits. In this paper we demonstrate the use of large (>100 $\mu$m(2)) but thin (<80 nm) chemically grown single-crystalline gold flakes that, after immobilization, serve as an ideal basis for focused ion beam milling and other top-down nanofabrication techniques on any desired substrate. Using this methodology we obtain high-definition ultrasmooth gold nanostructures with superior optical properties and reproducible nano-sized features over micrometre-length scales. Our approach provides a possible solution to overcome the current fabrication bottleneck and realize high-definition plasmonic nanocircuitry.},
	author = {Huang, Jer-Shing and Callegari, Victor and Geisler, Peter and Br\"{u}ning, Christoph and Kern, Johannes and Prangsma, Jord C and Wu, Xiaofei and Feichtner, Thorsten and Ziegler, Johannes and Weinmann, Pia and Kamp, Martin and Forchel, Alfred and Biagioni, Paolo and Sennhauser, Urs and Hecht, Bert},
	date-modified = {2022-03-17 09:50:00 +0100},
	doi = {10.1038/ncomms1143},
	file = {:C$\backslash$:/Users/sebastian.hammer/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Huang et al. - 2010 - Atomically flat single-crystalline gold nanostructures for plasmonic nanocircuitry.pdf:pdf},
	issn = {2041-1723},
	journal = {Nature communications},
	keywords = {Gold,Gold: chemistry,Microscopy, Electron, Scanning,Nanostructures,Nanostructures: chemistry,Nanostructures: ultrastructure,Nanotechnology,Nanotechnology: methods,Surface Plasmon Resonance},
	month = jan,
	pages = {150},
	pmid = {21267000},
	title = {{Atomically flat single-crystalline gold nanostructures for plasmonic nanocircuitry.}},
	url = {http://www.ncbi.nlm.nih.gov/pubmed/21267000},
	volume = {1},
	year = {2010},
	Bdsk-Url-1 = {http://www.ncbi.nlm.nih.gov/pubmed/21267000},
	Bdsk-Url-2 = {http://dx.doi.org/10.1038/ncomms1143}}

@article{Jankowski2005,
	author = {Jankowski, A F and Saw, C K and Harper, J F and Ferreira, J L and Hayes, J P},
	file = {:C$\backslash$:/Users/sebastian.hammer/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Jankowski et al. - 2005 - NANOCRYSTALLINE GROWTH AND GRAIN-SIZE EFFECTS IN AU-CU ELECTRODEPOSITS.pdf:pdf},
	title = {{NANOCRYSTALLINE GROWTH AND GRAIN-SIZE EFFECTS IN AU-CU ELECTRODEPOSITS}},
	year = {2005}}

@article{Kumar2013,
	archiveprefix = {arXiv},
	arxivid = {arXiv:1310.2421v1},
	author = {Kumar, Shailesh and Huck, Alexander and Lu, Ying-wei and Andersen, Ulrik L},
	eprint = {arXiv:1310.2421v1},
	file = {:C$\backslash$:/Users/sebastian.hammer/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Kumar et al. - 2013 - Coupling of single quantum emitters to plasmons propagating on mechanically etched wires.pdf:pdf},
	title = {{Coupling of single quantum emitters to plasmons propagating on mechanically etched wires}},
	year = {2013}}

@article{Kumar2012,
	abstract = {We demonstrate propagation of plasmons in single crystalline silver nanostructures fabricated using a combination of a bottom-up and a top-down approach. Silver nanoplates of thickness around 65 nm and a surface area of about 100 $\mu$m(2) are made using a wet chemical method. Silver nanotips and nanowires are then sculptured by focused ion beam milling. The plasmons are excited by using the fluorescence from the redeposited silver clusters during the milling process. Propagation of plasmons in the nanowires is observed in the visible spectral region. We also observe a cavity effect by measuring the emission spectrum from the distal wire end.},
	author = {Kumar, Shailesh and Lu, Ying-Wei and Huck, Alexander and Andersen, Ulrik L},
	file = {:C$\backslash$:/Users/sebastian.hammer/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Kumar et al. - 2012 - Propagation of plasmons in designed single crystalline silver nanostructures.pdf:pdf},
	issn = {1094-4087},
	journal = {Optics express},
	month = oct,
	number = {22},
	pages = {24614--22},
	pmid = {23187224},
	title = {{Propagation of plasmons in designed single crystalline silver nanostructures.}},
	url = {http://www.ncbi.nlm.nih.gov/pubmed/23187224},
	volume = {20},
	year = {2012},
	Bdsk-Url-1 = {http://www.ncbi.nlm.nih.gov/pubmed/23187224}}

@article{Lamprecht2001,
	author = {Lamprecht, B. and Krenn, J. R. and Schider, G. and Ditlbacher, H. and Salerno, M. and Felidj, N. and Leitner, a. and Aussenegg, F. R. and Weeber, J. C.},
	doi = {10.1063/1.1380236},
	file = {:C$\backslash$:/Users/sebastian.hammer/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Lamprecht et al. - 2001 - Surface plasmon propagation in microscale metal stripes.pdf:pdf},
	issn = {00036951},
	journal = {Applied Physics Letters},
	number = {1},
	pages = {51},
	title = {{Surface plasmon propagation in microscale metal stripes}},
	url = {http://scitation.aip.org/content/aip/journal/apl/79/1/10.1063/1.1380236},
	volume = {79},
	year = {2001},
	Bdsk-Url-1 = {http://scitation.aip.org/content/aip/journal/apl/79/1/10.1063/1.1380236},
	Bdsk-Url-2 = {http://dx.doi.org/10.1063/1.1380236}}

@article{Lu2012,
	abstract = {A nanolaser is a key component for on-chip optical communications and computing systems. Here, we report on the low-threshold, continuous-wave operation of a subdiffraction nanolaser based on surface plasmon amplification by stimulated emission of radiation. The plasmonic nanocavity is formed between an atomically smooth epitaxial silver film and a single optically pumped nanorod consisting of an epitaxial gallium nitride shell and an indium gallium nitride core acting as gain medium. The atomic smoothness of the metallic film is crucial for reducing the modal volume and plasmonic losses. Bimodal lasing with similar pumping thresholds was experimentally observed, and polarization properties of the two modes were used to unambiguously identify them with theoretically predicted modes. The all-epitaxial approach opens a scalable platform for low-loss, active nanoplasmonics.},
	author = {Lu, Yu-Jung and Kim, Jisun and Chen, Hung-Ying and Wu, Chihhui and Dabidian, Nima and Sanders, Charlotte E and Wang, Chun-Yuan and Lu, Ming-Yen and Li, Bo-Hong and Qiu, Xianggang and Chang, Wen-Hao and Chen, Lih-Juann and Shvets, Gennady and Shih, Chih-Kang and Gwo, Shangjr},
	doi = {10.1126/science.1223504},
	file = {:C$\backslash$:/Users/sebastian.hammer/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Lu et al. - 2012 - Plasmonic nanolaser using epitaxially grown silver film.pdf:pdf},
	issn = {1095-9203},
	journal = {Science (New York, N.Y.)},
	month = jul,
	number = {6093},
	pages = {450--3},
	pmid = {22837524},
	title = {{Plasmonic nanolaser using epitaxially grown silver film.}},
	url = {http://www.ncbi.nlm.nih.gov/pubmed/22837524},
	volume = {337},
	year = {2012},
	Bdsk-Url-1 = {http://www.ncbi.nlm.nih.gov/pubmed/22837524},
	Bdsk-Url-2 = {http://dx.doi.org/10.1126/science.1223504}}

@article{Oulton2008,
	author = {Oulton, R. F. and Sorger, V. J. and Genov, D. a. and Pile, D. F. P. and Zhang, X.},
	doi = {10.1038/nphoton.2008.131},
	file = {:C$\backslash$:/Users/sebastian.hammer/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Oulton et al. - 2008 - A hybrid plasmonic waveguide for subwavelength confinement and long-range propagation.pdf:pdf},
	issn = {1749-4885},
	journal = {Nature Photonics},
	month = jul,
	number = {8},
	pages = {496--500},
	title = {{A hybrid plasmonic waveguide for subwavelength confinement and long-range propagation}},
	url = {http://www.nature.com/doifinder/10.1038/nphoton.2008.131},
	volume = {2},
	year = {2008},
	Bdsk-Url-1 = {http://www.nature.com/doifinder/10.1038/nphoton.2008.131},
	Bdsk-Url-2 = {http://dx.doi.org/10.1038/nphoton.2008.131}}

@article{Park2012,
	abstract = {A simple route to flat, large-area, single-crystalline films for plasmonics is demonstrated by sputter deposition of silver onto mica substrates at elevated temperatures. The films exhibit improved dielectric properties and allow more precise patterning of high-quality nanostructures for plasmonic applications.},
	author = {Park, Jong Hyuk and Ambwani, Palak and Manno, Michael and Lindquist, Nathan C and Nagpal, Prashant and Oh, Sang-Hyun and Leighton, Chris and Norris, David J},
	doi = {10.1002/adma.201200812},
	file = {:C$\backslash$:/Users/sebastian.hammer/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Park et al. - 2012 - Single-crystalline silver films for plasmonics.pdf:pdf},
	issn = {1521-4095},
	journal = {Advanced materials (Deerfield Beach, Fla.)},
	keywords = {Crystallization,Electrons,Nanostructures,Nanostructures: chemistry,Silver,Silver: chemistry,Surface Plasmon Resonance,Temperature},
	month = aug,
	number = {29},
	pages = {3988--92},
	pmid = {22700389},
	title = {{Single-crystalline silver films for plasmonics.}},
	url = {http://www.ncbi.nlm.nih.gov/pubmed/22700389},
	volume = {24},
	year = {2012},
	Bdsk-Url-1 = {http://www.ncbi.nlm.nih.gov/pubmed/22700389},
	Bdsk-Url-2 = {http://dx.doi.org/10.1002/adma.201200812}}

@article{Prangsma2012,
	abstract = {Electrically connected resonant optical antennas hold promise for the realization of highly efficient nanoscale electro-plasmonic devices that rely on a combination of electric fields and local near-field intensity enhancement. Here we demonstrate the feasibility of such a concept by attaching leads to the arms of a two-wire antenna at positions of minimal near-field intensity with negligible influence on the antenna resonance. White-light scattering experiments in accordance with simulations show that the optical tunability of connected antennas is fully retained. Analysis of the electric properties demonstrates that in the antenna gaps direct current (DC) electric fields of 10(8) V/m can consistently be achieved and maintained over extended periods of time without noticeable damage.},
	author = {Prangsma, Jord C and Kern, Johannes and Knapp, Alexander G and Grossmann, Swen and Emmerling, Monika and Kamp, Martin and Hecht, Bert},
	doi = {10.1021/nl3007374},
	file = {:C$\backslash$:/Users/sebastian.hammer/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Prangsma et al. - 2012 - Electrically connected resonant optical antennas.pdf:pdf},
	issn = {1530-6992},
	journal = {Nano letters},
	keywords = {1 many exciting,can be localized to,electronic transport,fi ned to nanometallic,nano-gap,nanophotonics,optical antenna,optical fi elds,plasmonics,structures possess strongly enhanced,subwavelength scales,urface plasmon polaritons con,which},
	month = aug,
	number = {8},
	pages = {3915--9},
	pmid = {22800440},
	title = {{Electrically connected resonant optical antennas.}},
	url = {http://www.ncbi.nlm.nih.gov/pubmed/22800440},
	volume = {12},
	year = {2012},
	Bdsk-Url-1 = {http://www.ncbi.nlm.nih.gov/pubmed/22800440},
	Bdsk-Url-2 = {http://dx.doi.org/10.1021/nl3007374}}

@article{Smith1996,
	abstract = {A flat epitaxial silver film on a gallium arsenide [GaAs(110)] surface was synthesized in a two-step process. Deposition of a critical thickness of silver at low temperature led to the formation of a dense nanocluster film. Upon annealing, all atoms rearranged themselves into an atomically flat film. This silver film has a close-packed (111) structure modulated by a "silver mean" quasi-periodic sequence. The ability to grow such epitaxial overlayers of metals on semiconductors enables the testing of theoretical models and provides a connection between metal and semiconductor technologies.},
	author = {Smith, Ar and Chao, Kj and Niu, Q and Shih, Ck},
	file = {:C$\backslash$:/Users/sebastian.hammer/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Smith et al. - 1996 - Formation of Atomically Flat Silver Films on GaAs with a Silver Mean Quasi Periodicity.pdf:pdf},
	issn = {1095-9203},
	journal = {Science (New York, N.Y.)},
	month = jul,
	number = {5272},
	pages = {226--8},
	pmid = {8662503},
	title = {{Formation of Atomically Flat Silver Films on GaAs with a "Silver Mean" Quasi Periodicity}},
	url = {http://www.ncbi.nlm.nih.gov/pubmed/8662503},
	volume = {273},
	year = {1996},
	Bdsk-Url-1 = {http://www.ncbi.nlm.nih.gov/pubmed/8662503}}

@article{Stockman2011,
	author = {Stockman, Mark I.},
	doi = {10.1063/1.3554315},
	file = {:C$\backslash$:/Users/sebastian.hammer/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Stockman - 2011 - Nanoplasmonics The physics behind the applications.pdf:pdf},
	issn = {00319228},
	journal = {Physics Today},
	number = {2},
	pages = {39},
	title = {{Nanoplasmonics: The physics behind the applications}},
	url = {http://link.aip.org/link/PHTOAD/v64/i2/p39/s1\&Agg=doi},
	volume = {64},
	year = {2011},
	Bdsk-Url-1 = {http://link.aip.org/link/PHTOAD/v64/i2/p39/s1%5C&Agg=doi},
	Bdsk-Url-2 = {http://dx.doi.org/10.1063/1.3554315}}

@article{Verhagen2008,
	abstract = {We investigate the focusing of surface plasmon polaritons (SPPs) excited with 1.5 microm light in a tapered Au waveguide on a planar dielectric substrate by experiments and simulations. We find that nanofocusing can be obtained when the asymmetric bound mode at the substrate side of the metal film is excited. The propagation and concentration of this mode to the tip is demonstrated. No sign of a cutoff waveguide width is observed as the SPPs propagate along the tapered waveguide. Simulations show that such concentrating behavior is not possible for excitation of the mode at the low-index side of the film. The mode that enables the focusing exhibits a strong resemblance to the asymmetric mode responsible for focusing in conical waveguides. This work demonstrates a practical implementation of plasmonic nanofocusing on a planar substrate.},
	author = {Verhagen, Ewold and Polman, Albert and Kuipers, L Kobus},
	file = {:C$\backslash$:/Users/sebastian.hammer/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Verhagen, Polman, Kuipers - 2008 - Nanofocusing in laterally tapered plasmonic waveguides.pdf:pdf},
	issn = {1094-4087},
	journal = {Optics express},
	keywords = {Equipment Design,Equipment Failure Analysis,Gold,Image Enhancement,Image Enhancement: instrumentation,Nanoparticles,Nanotechnology,Nanotechnology: instrumentation,Particle Size,Surface Plasmon Resonance,Surface Plasmon Resonance: instrumentation,Surface Plasmon Resonance: methods},
	month = jan,
	number = {1},
	pages = {45--57},
	pmid = {18521131},
	title = {{Nanofocusing in laterally tapered plasmonic waveguides.}},
	url = {http://www.ncbi.nlm.nih.gov/pubmed/18521131},
	volume = {16},
	year = {2008},
	Bdsk-Url-1 = {http://www.ncbi.nlm.nih.gov/pubmed/18521131}}

@article{Zia2005,
	author = {Zia, Rashid and Selker, Mark and Brongersma, Mark},
	doi = {10.1103/PhysRevB.71.165431},
	file = {:C$\backslash$:/Users/sebastian.hammer/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Zia, Selker, Brongersma - 2005 - Leaky and bound modes of surface plasmon waveguides.pdf:pdf},
	issn = {1098-0121},
	journal = {Physical Review B},
	month = apr,
	number = {16},
	pages = {165431},
	title = {{Leaky and bound modes of surface plasmon waveguides}},
	url = {http://link.aps.org/doi/10.1103/PhysRevB.71.165431},
	volume = {71},
	year = {2005},
	Bdsk-Url-1 = {http://link.aps.org/doi/10.1103/PhysRevB.71.165431},
	Bdsk-Url-2 = {http://dx.doi.org/10.1103/PhysRevB.71.165431}}

@article{Bozhevolnyi2006,
	abstract = {Photonic components are superior to electronic ones in terms of operational bandwidth, but the diffraction limit of light poses a significant challenge to the miniaturization and high-density integration of optical circuits. The main approach to circumvent this problem is to exploit the hybrid nature of surface plasmon polaritons (SPPs), which are light waves coupled to free electron oscillations in a metal that can be laterally confined below the diffraction limit using subwavelength metal structures. However, the simultaneous realization of strong confinement and a propagation loss sufficiently low for practical applications has long been out of reach. Channel SPP modes--channel plasmon polaritons (CPPs)--are electromagnetic waves that are bound to and propagate along the bottom of V-shaped grooves milled in a metal film. They are expected to exhibit useful subwavelength confinement, relatively low propagation loss, single-mode operation and efficient transmission around sharp bends. Our previous experiments showed that CPPs do exist and that they propagate over tens of micrometres along straight subwavelength grooves. Here we report the design, fabrication and characterization of CPP-based subwavelength waveguide components operating at telecom wavelengths: Y-splitters, Mach-Zehnder interferometers and waveguide-ring resonators. We demonstrate that CPP guides can indeed be used for large-angle bending and splitting of radiation, thereby enabling the realization of ultracompact plasmonic components and paving the way for a new class of integrated optical circuits.},
	author = {Bozhevolnyi, Sergey I and Volkov, Valentyn S and Devaux, Elo\"{\i}se and Laluet, Jean-Yves and Ebbesen, Thomas W},
	doi = {10.1038/nature04594},
	file = {:C$\backslash$:/Users/sebastian.hammer/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Bozhevolnyi et al. - 2006 - Channel plasmon subwavelength waveguide components including interferometers and ring resonators.pdf:pdf},
	issn = {1476-4687},
	journal = {Nature},
	month = mar,
	number = {7083},
	pages = {508--11},
	pmid = {16554814},
	title = {{Channel plasmon subwavelength waveguide components including interferometers and ring resonators.}},
	url = {http://www.ncbi.nlm.nih.gov/pubmed/16554814},
	volume = {440},
	year = {2006},
	Bdsk-Url-1 = {http://www.ncbi.nlm.nih.gov/pubmed/16554814},
	Bdsk-Url-2 = {http://dx.doi.org/10.1038/nature04594}}

@article{Feature2009,
	author = {Heber, Joerg},
	file = {:C$\backslash$:/Users/sebastian.hammer/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Feature - 2009 - Small oscillations of surface electrons that manipulate light on the nanoscale could be the route to applications as disparate as faster computer chips.pdf:pdf},
	journal = {Nature},
	number = {October},
	pages = {8--10},
	title = {{Surfing the wave}},
	volume = {461},
	year = {2009}}

@article{Kumar2013a,
	archiveprefix = {arXiv},
	arxivid = {arXiv:1306.4132v1},
	author = {Kumar, Shailesh and Huck, Alexander and Chen, Yuntian and Andersen, Ulrik L},
	eprint = {arXiv:1306.4132v1},
	file = {:C$\backslash$:/Users/sebastian.hammer/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Kumar et al. - 2013 - Coupling of a Single Quantum Emitter to End-to-end Aligned Silver Nanowires.pdf:pdf},
	pages = {1--5},
	title = {{Coupling of a Single Quantum Emitter to End-to-end Aligned Silver Nanowires}},
	year = {2013}}

@article{Tame2013,
	author = {Tame, M. S. and McEnery, K. R. and \"{O}zdemir, {\c S}. K. and Lee, J. and Maier, S. a. and Kim, M. S.},
	doi = {10.1038/nphys2615},
	file = {:C$\backslash$:/Users/sebastian.hammer/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Tame et al. - 2013 - Quantum plasmonics.pdf:pdf},
	issn = {1745-2473},
	journal = {Nature Physics},
	month = jun,
	number = {6},
	pages = {329--340},
	publisher = {Nature Publishing Group},
	title = {{Quantum plasmonics}},
	url = {http://www.nature.com/doifinder/10.1038/nphys2615},
	volume = {9},
	year = {2013},
	Bdsk-Url-1 = {http://www.nature.com/doifinder/10.1038/nphys2615},
	Bdsk-Url-2 = {http://dx.doi.org/10.1038/nphys2615}}

@book{Fox2006,
	author = {Fox, M.},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/Literature/Fox, Mark - Quantum Optics.pdf:pdf},
	title = {{No Title}},
	year = {2006}}

@book{Maier2007,
	author = {Maier, Stefan A},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/Literature/S.Maier\_Plasmonics Fundamentals and Applications - S.Maier.pdf:pdf},
	isbn = {9780387331508},
	publisher = {Springer Science+Business Media LLC},
	title = {{Plasmonics: Fundamentals and Applications}},
	year = {2007}}

@article{Barnes2003,
	author = {Barnes, William L and Dereux, Alain and Ebbesen, Thomas W},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/papers/Barnes\_Nature\_424\_(2003)\_Surface plasmonsubwavelength optics.pdf:pdf},
	journal = {Nature},
	number = {August},
	pages = {824--830},
	title = {subwavelength optics},
	volume = {424},
	year = {2003}}

@article{Johnson1972,
	author = {Johnson, P. B. and Christy, R. W.},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/Literature/Johnson\_PRB\_6\_4370\_(1972)\_Optical Constants of the Noble Metals.pdf:pdf},
	journal = {Physical Review B},
	number = {12},
	pages = {4370--4379},
	title = {{Optical Constants of the Noble Metals}},
	volume = {4},
	year = {1972}}

@book{Palik1998,
	author = {Palik, Edward D.},
	publisher = {Academic Press},
	title = {{Handbook of Optical Constants of Solids}},
	year = {1998}}

@article{Reyntjens2001,
	author = {Reyntjens, Steve and Puers, Robert},
	doi = {10.1088/0960-1317/11/4/301},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/papers/Reyntjens\_JM\_11\_(2001)\_A review of focused ion beam applications.pdf:pdf},
	issn = {0960-1317},
	journal = {Journal of Micromechanics and Microengineering},
	month = jul,
	number = {4},
	pages = {287--300},
	title = {{A review of focused ion beam applications in microsystem technology}},
	url = {http://stacks.iop.org/0960-1317/11/i=4/a=301?key=crossref.eb603166dc8f0b0b38252c5fc2f55f3c},
	volume = {11},
	year = {2001},
	Bdsk-Url-1 = {http://stacks.iop.org/0960-1317/11/i=4/a=301?key=crossref.eb603166dc8f0b0b38252c5fc2f55f3c},
	Bdsk-Url-2 = {http://dx.doi.org/10.1088/0960-1317/11/4/301}}

@manual{Elphy2005,
	organisation = {Raith},
	title = {ELPHY Quantum Version 5.0},
	year = {2005}}

@manual{Nvision40,
	organisation = {Carl Zeiss SMT},
	title = {NVision 40},
	year = {2006}}

@article{Aspnes1986,
	author = {Aspnes, D.E. and Kelso, S.M. and Logan, R.A. and Bhat, R.},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/papers/Aspnes\_AP\_60\_754\_(1986)\_Optical properties of Al x Ga1−x As.pdf:pdf},
	journal = {Journal of Applied Physics},
	pages = {754},
	title = {Optical properties of $Al_x Ga_{1- x}$ As},
	volume = {60},
	year = {1986}}

@article{Otto1968,
	author = {Otto, Andreas},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/papers/Otto\_ZfP\_1968\_Excitation of Nonradiative Surface Plasma Waves....pdf:pdf},
	journal = {Z. Physik},
	pages = {398--410},
	title = {{Excitation of Nonradiative Surface Plasma Waves in Silver by the Method of Frustrated Total Reflection}},
	volume = {216},
	year = {1968}}

@article{Kretschmann1968,
	author = {Kretschmann, E. and Raether, H.},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/papers/Kretschmann\_ZNA-1968-23a-2135\_n.pdf:pdf},
	journal = {Z. Naturforschung},
	pages = {2135--2136},
	title = {{Radiative Decay of Non Radiative Surface Plasmons Excited by Light}},
	volume = {23 a},
	year = {1968}}

@book{Raether1988,
	address = {Berlin},
	author = {Raether, Heinz},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/Literature/Raether\_Surface Plasmons\_Springer\_(1986).pdf:pdf},
	publisher = {Springer-Verlag},
	title = {{Surface Plasmons}},
	year = {1988}}

@article{Kuttge2008,
	author = {Kuttge, M. and Vesseur, E. J. R. and Verhoeven, J. and Lezec, H. J. and Atwater, H. a. and Polman, a.},
	doi = {10.1063/1.2987458},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/papers/Kuttge\_(2005)\_APL\_Loss meachanisms SPR.pdf:pdf},
	issn = {00036951},
	journal = {Applied Physics Letters},
	number = {11},
	pages = {113110},
	title = {{Loss mechanisms of surface plasmon polaritons on gold probed by cathodoluminescence imaging spectroscopy.}},
	url = {http://scitation.aip.org/content/aip/journal/apl/93/11/10.1063/1.2987458},
	volume = {93},
	year = {2008},
	Bdsk-Url-1 = {http://scitation.aip.org/content/aip/journal/apl/93/11/10.1063/1.2987458},
	Bdsk-Url-2 = {http://dx.doi.org/10.1063/1.2987458}}

@article{Vieu2000,
	author = {Vieu, C and Carcenac, F and Pepin, A and Chen, Y and Mejias, M and Lebib, A and Couraud, L and Launois, H},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/papers/Vieu\_ASS\_164\_(2000)\_Electron beam lithography-Resolution limits and applications.pdf:pdf},
	journal = {Applied Surface Science},
	keywords = {data storage,electron beam lithography,molecular electronics,nanofabrication,nanolithography,single electron devices},
	pages = {111--117},
	title = {{Electron beam lithography : resolution limits and applications}},
	volume = {164},
	year = {2000}}

@book{Singh2003,
	author = {Singh, Jasprit},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/Literature/Singh - Electronic and Optoelectronic Properties of Semiconductor Structures.pdf:pdf},
	isbn = {9780521823791},
	publisher = {Cambridge University Press},
	title = {{Electronic and Optoelectronic Properties of Semiconductor Structures}},
	year = {2003}}

@book{Bimberg2008,
	address = {Berlin},
	author = {Bimberg, Dieter},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/Literature/Bimberg - Semiconductor Nanostructures.pdf:pdf},
	isbn = {9783540778981},
	publisher = {Springer-Verlag},
	title = {{Semiconductor Nanostructures}},
	year = {2008}}

@book{Hol58,
	address = {New York},
	author = {Holland, L.},
	date-modified = {2022-03-17 09:50:10 +0100},
	pages = {208, 244},
	publisher = {John Wiley \& Sons Inc},
	title = {{Vacuum Deposition of Thin Films}},
	url = {http://babel.hathitrust.org/cgi/pt?id=mdp.39076001211379;view=1up;seq=27},
	year = {1958},
	Bdsk-Url-1 = {http://babel.hathitrust.org/cgi/pt?id=mdp.39076001211379;view=1up;seq=27}}

@article{Lani2006,
	author = {Lani, S. and Bosseboeuf, A. and Belier, B. and Clerc, C. and Gousset, C. and Aubert, J.},
	journal = {Microsystems Technologies},
	number = {10-11},
	pages = {1021--1025},
	title = {{Gold metallizations for eutectic bonding of silicon wafers}},
	volume = {12},
	year = {2006}}

@book{Hecht2002,
	address = {San Francisco},
	author = {Hecht, Eugene},
	edition = {4},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/Literature/Hecht, Eugene - Optics\_4ed.pdf:pdf},
	isbn = {0321188780},
	pages = {351},
	publisher = {Addison Wesley},
	title = {{Optics}},
	year = {2002}}

@book{Kittel1996,
	address = {New York},
	author = {Kittel, Charles},
	edition = {7},
	publisher = {John Wiley \& Sons Inc},
	title = {{Introduction to Solid State Physics}},
	year = {1996}}

@article{Andrieu1996,
	author = {Andrieu, St\'{e}phane and Fr\'{e}chard, Patrick},
	doi = {10.1016/0039-6028(96)00303-2},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/papers/Andrieu\_Surface Science\_360\_(1996)\_What information can be obtained by RHEED on polycryst films.pdf:pdf},
	issn = {00396028},
	journal = {Surface Science},
	keywords = {and,diffraction,electron-solid diffraction,electron-solid interactions,growth,iron,molecular beam epitaxy,morphology,polycrystalline thin films,reflection high-energy electron diffraction,rheed,roughness,scattering,surface structure},
	month = jul,
	number = {1-3},
	pages = {289--296},
	title = {{What information can be obtained by RHEED applied on polycrystalline films?}},
	url = {http://linkinghub.elsevier.com/retrieve/pii/0039602896003032},
	volume = {360},
	year = {1996},
	Bdsk-Url-1 = {http://linkinghub.elsevier.com/retrieve/pii/0039602896003032},
	Bdsk-Url-2 = {http://dx.doi.org/10.1016/0039-6028(96)00303-2}}

@article{Neave1983,
	author = {Neave, J. H. and Joyce, B. a. and Dobson, P. J. and Norton, N.},
	doi = {10.1007/BF00617180},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/papers/Neave\_Appl Phys A\_31\_(1983)\_Dynamics of Film Growth of GaAs by MBE....pdf:pdf},
	issn = {0721-7250},
	journal = {Applied Physics A Solids and Surfaces},
	month = may,
	number = {1},
	pages = {1--8},
	title = {{Dynamics of film growth of GaAs by MBE from Rheed observations}},
	url = {http://link.springer.com/10.1007/BF00617180},
	volume = {31},
	year = {1983},
	Bdsk-Url-1 = {http://link.springer.com/10.1007/BF00617180},
	Bdsk-Url-2 = {http://dx.doi.org/10.1007/BF00617180}}

@article{Finley2001,
	author = {Finley, J. and Ashmore, a. and Lema\^{\i}tre, a. and Mowbray, D. and Skolnick, M. and Itskevich, I. and Maksym, P. and Hopkinson, M. and Krauss, T.},
	doi = {10.1103/PhysRevB.63.073307},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/papers/Finley, J. J. et al. - Charged and neutral exciton complexes in individual self-assembled In(Ga)As quantum dots (2001).pdf:pdf},
	issn = {0163-1829},
	journal = {Physical Review B},
	month = jan,
	number = {7},
	pages = {073307},
	title = {{Charged and neutral exciton complexes in individual self-assembled In(Ga)As quantum dots}},
	url = {http://link.aps.org/doi/10.1103/PhysRevB.63.073307},
	volume = {63},
	year = {2001},
	Bdsk-Url-1 = {http://link.aps.org/doi/10.1103/PhysRevB.63.073307},
	Bdsk-Url-2 = {http://dx.doi.org/10.1103/PhysRevB.63.073307}}

@article{Findeis2001,
	author = {Findeis, F. and Baier, M. and Zrenner, a. and Bichler, M. and Abstreiter, G. and Hohenester, U. and Molinari, E.},
	doi = {10.1103/PhysRevB.63.121309},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/papers/Findeis\_PRB\_63\_121309\_(2001)\_Optical excitations of s self-assembled artificial ion.pdf:pdf},
	issn = {0163-1829},
	journal = {Physical Review B},
	month = mar,
	number = {12},
	pages = {121309},
	title = {{Optical excitations of a self-assembled artificial ion}},
	url = {http://link.aps.org/doi/10.1103/PhysRevB.63.121309},
	volume = {63},
	year = {2001},
	Bdsk-Url-1 = {http://link.aps.org/doi/10.1103/PhysRevB.63.121309},
	Bdsk-Url-2 = {http://dx.doi.org/10.1103/PhysRevB.63.121309}}

@article{Grundmann1997,
	author = {Grundmann, M. and Bimberg, D.},
	doi = {10.1103/PhysRevB.55.9740},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/papers/Grundmann\_PRB\_55\_15\_(1997)\_Theory of random population for quantum dots.pdf:pdf},
	issn = {0163-1829},
	journal = {Physical Review B},
	month = apr,
	number = {15},
	pages = {9740--9745},
	title = {{Theory of random population for quantum dots}},
	url = {http://link.aps.org/doi/10.1103/PhysRevB.55.9740},
	volume = {55},
	year = {1997},
	Bdsk-Url-1 = {http://link.aps.org/doi/10.1103/PhysRevB.55.9740},
	Bdsk-Url-2 = {http://dx.doi.org/10.1103/PhysRevB.55.9740}}

@misc{Bougeard2014,
	author = {Bougeard, Dominique},
	howpublished = {discussion},
	year = {2014}}

@misc{Weiser2014,
	author = {Weiser, Peter},
	howpublished = {discussion},
	year = {2014}}

@unpublished{BracherPhD,
	author = {Bracher, Gregor},
	note = {unpublished},
	title = {PhD Thesis},
	year = {2014}}

@article{Akimov2007,
	abstract = {Control over the interaction between single photons and individual optical emitters is an outstanding problem in quantum science and engineering. It is of interest for ultimate control over light quanta, as well as for potential applications such as efficient photon collection, single-photon switching and transistors, and long-range optical coupling of quantum bits. Recently, substantial advances have been made towards these goals, based on modifying photon fields around an emitter using high-finesse optical cavities. Here we demonstrate a cavity-free, broadband approach for engineering photon-emitter interactions via subwavelength confinement of optical fields near metallic nanostructures. When a single CdSe quantum dot is optically excited in close proximity to a silver nanowire, emission from the quantum dot couples directly to guided surface plasmons in the nanowire, causing the wire's ends to light up. Non-classical photon correlations between the emission from the quantum dot and the ends of the nanowire demonstrate that the latter stems from the generation of single, quantized plasmons. Results from a large number of devices show that efficient coupling is accompanied by more than 2.5-fold enhancement of the quantum dot spontaneous emission, in good agreement with theoretical predictions.},
	author = {Akimov, A. V. and Mukherjee, A and Yu, C. L. and Chang, D E and Zibrov, a S and Hemmer, P R and Park, H and Lukin, M D},
	doi = {10.1038/nature06230},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/papers/Akimov\_nature\_450\_(2007)\_Generation of single optical plasmons in metallic nanowirs coupled to QDs.pdf:pdf},
	issn = {1476-4687},
	journal = {Nature},
	month = nov,
	number = {7168},
	pages = {402--6},
	pmid = {18004381},
	title = {{Generation of single optical plasmons in metallic nanowires coupled to quantum dots.}},
	url = {http://www.ncbi.nlm.nih.gov/pubmed/18004381},
	volume = {450},
	year = {2007},
	Bdsk-Url-1 = {http://www.ncbi.nlm.nih.gov/pubmed/18004381},
	Bdsk-Url-2 = {http://dx.doi.org/10.1038/nature06230}}

@article{Dekel2000,
	author = {Dekel, E. and Gershoni, D. and Ehrenfreund, E. and Garcia, J. and Petroff, P.},
	doi = {10.1103/PhysRevB.61.11009},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/papers/Dekel\_PRB\_61\_16\_Carrier-carrier correlations in an optically excited single semmiconductor QD.pdf:pdf},
	issn = {0163-1829},
	journal = {Physical Review B},
	month = apr,
	number = {16},
	pages = {11009--11020},
	title = {{Carrier-carrier correlations in an optically excited single semiconductor quantum dot}},
	url = {http://link.aps.org/doi/10.1103/PhysRevB.61.11009},
	volume = {61},
	year = {2000},
	Bdsk-Url-1 = {http://link.aps.org/doi/10.1103/PhysRevB.61.11009},
	Bdsk-Url-2 = {http://dx.doi.org/10.1103/PhysRevB.61.11009}}

@article{Tersoff1984,
	author = {Tersoff, J.},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/papers/Tersoff\_PRL\_52\_6\_(1984)\_Schottky Barrier Heights and the Continuum of Gap States.pdf:pdf},
	journal = {Physical Review Letters},
	number = {6},
	title = {{Schottky Barrier Heights and the Continuum of Gap States}},
	volume = {52},
	year = {1984}}

@article{Abstreiter1978,
	author = {Abstreiter, G and Bauser, E and Fischer, A and Ploog, K},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/papers/Abstreiter\_ApplPhys\_16\_345\_(1978)\_Raman Spectroscopy....pdf:pdf},
	journal = {Applied Physics},
	pages = {345--352},
	title = {{Raman Spectroscopy - A Versatile Tool for Characterization of Thin Films and Heterostructures of GaAs and Al(x)Ga(1-x)As}},
	volume = {16},
	year = {1978}}

@article{Hu2013,
	abstract = {On-chip nanophotonics serves as the foundation for the new generation of information technology, but it is challenged by the diffraction limit of light. With the capabilities of confining light into (deep) subwavelength volumes, plasmonics makes it possible to dramatically miniaturize optical devices so as to integrate them into silicon chips. Here we demonstrate that by cascading nano-corrugation gratings with different periodicities on silver nanowires atop silicon, different colors can be spatially separated and chronologically released at different grating junctions. The released light frequency depends on the grating arrangement and corrugation periodicities. Hence the nanowire acts as a spectral splitter for sorting/demultiplexing photons at different nano-scale positions with a ten-femtosecond-level interval. Such nanowires can be constructed further into compact 2D networks or circuits. We believe that this study provides a new and promising approach for realizing spatiotemporal-sensitive spectral splitting and optical signal processing on nanoscales, and for general integration of nanophotonics with microelectronics.},
	author = {Hu, Qing and Xu, Di-Hu and Zhou, Yu and Peng, Ru-Wen and Fan, Ren-Hao and Fang, Nicholas X and Wang, Qian-Jin and Huang, Xian-Rong and Wang, Mu},
	doi = {10.1038/srep03095},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/papers/Hu\_Scientific Report\_3\_3095\_(2013)\_Position-sensitive spectral splitting with a plasmonic nanowire on silicon chip.pdf:pdf},
	issn = {2045-2322},
	journal = {Scientific reports},
	month = jan,
	pages = {3095},
	pmid = {24172838},
	title = {{Position-sensitive spectral splitting with a plasmonic nanowire on silicon chip.}},
	url = {http://www.pubmedcentral.nih.gov/articlerender.fcgi?artid=3813943\&tool=pmcentrez\&rendertype=abstract},
	volume = {3},
	year = {2013},
	Bdsk-Url-1 = {http://www.pubmedcentral.nih.gov/articlerender.fcgi?artid=3813943%5C&tool=pmcentrez%5C&rendertype=abstract},
	Bdsk-Url-2 = {http://dx.doi.org/10.1038/srep03095}}

@article{Shchukin1995,
	author = {Shchukin, V.A. and Ledentsov, N.N. and Kop'ev, P.S. and Bimberg, D.},
	journal = {Physical Review Letters1},
	number = {16},
	title = {{Spontaneous Ordering of Arrays of Coherent Strained Islands}},
	volume = {75},
	year = {1995}}

@mastersthesis{Spiegl2013,
	author = {Spiegl, Matthias},
	school = {Technische Universit\"at M\"unchen},
	title = {Plasmonic Bowtie Nanoantennas for Hybrid Photonic Nanosystems},
	type = {Master's Thesis},
	year = {2013}}

@book{Bimberg1999,
	author = {Bimberg, D. and Grundmann, M. and Ledentsov, N.N.},
	pages = {37--38},
	title = {{Quantum Dot Heterostructures}},
	year = {1999}}

@article{Devaux2003,
	author = {Devaux, Eloise and Ebbesen, Thomas W. and Weeber, Jean-Claude and Dereux, Alain},
	doi = {10.1063/1.1634379},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/papers/Devaux\_APL\_83\_24\_(2003)\_Launching and decoupling surface plasmons via micro-gratings.pdf:pdf},
	issn = {00036951},
	journal = {Applied Physics Letters},
	number = {24},
	pages = {4936},
	title = {{Launching and decoupling surface plasmons via micro-gratings}},
	url = {http://scitation.aip.org/content/aip/journal/apl/83/24/10.1063/1.1634379},
	volume = {83},
	year = {2003},
	Bdsk-Url-1 = {http://scitation.aip.org/content/aip/journal/apl/83/24/10.1063/1.1634379},
	Bdsk-Url-2 = {http://dx.doi.org/10.1063/1.1634379}}

@article{Akselrod2014,
	author = {Akselrod, Gleb M. and Argyropoulos, Christos and Hoang, Thang B. and Cirac\`{\i}, Cristian and Fang, Chao and Huang, Jiani and Smith, David R. and Mikkelsen, Maiken H.},
	doi = {10.1038/nphoton.2014.228},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/papers/Akselrod\_(2014)\_Nature Photonics\_Probing the mechanisms of large purcell enhancements in plasmonic nanoantennas.pdf:pdf},
	issn = {1749-4885},
	journal = {Nature Photonics},
	month = oct,
	number = {11},
	pages = {835--840},
	publisher = {Nature Publishing Group},
	title = {{Probing the mechanisms of large Purcell enhancement in plasmonic nanoantennas}},
	url = {http://www.nature.com/doifinder/10.1038/nphoton.2014.228},
	volume = {8},
	year = {2014},
	Bdsk-Url-1 = {http://www.nature.com/doifinder/10.1038/nphoton.2014.228},
	Bdsk-Url-2 = {http://dx.doi.org/10.1038/nphoton.2014.228}}

@article{Monte2003,
	author = {a.F.G Monte and Finley, J.J and Ashmore, a and a.M Fox and Skolnick, M.S and Mowbray, D.J and Hopkins, M},
	doi = {10.1016/S1386-9477(02)00723-3},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/papers/Monte, Finley\_Science\_Direct\_E17\_109-110\_(2003)\_Carrier dynamics....pdf:pdf},
	issn = {13869477},
	journal = {Physica E: Low-dimensional Systems and Nanostructures},
	keywords = {algaas quantum dots,hopping process,inas,time-resolved photoluminescence},
	month = apr,
	pages = {109--110},
	title = {{Carrier dynamics in red-emitting self-organised InAs--AlGaAs quantum dots with indirect barriers}},
	url = {http://linkinghub.elsevier.com/retrieve/pii/S1386947702007233},
	volume = {17},
	year = {2003},
	Bdsk-Url-1 = {http://linkinghub.elsevier.com/retrieve/pii/S1386947702007233},
	Bdsk-Url-2 = {http://dx.doi.org/10.1016/S1386-9477(02)00723-3}}

@mastersthesis{Coc13,
	author = {Coca Lopez, Nicolas},
	date-modified = {2022-03-17 10:55:40 +0100},
	school = {Technische Universit\"at M\"unchen},
	title = {Towards on-chip quantum optics: Studies on InGaAs quantum dot based plasmonic hybrid systems},
	type = {Master's Thesis},
	year = {2013}}

@article{Dzhioev2001,
	author = {Dzhioev, R. I. and Zakharchenya, B. P. and Korenev, V. L. and Gammon, D. and Katzer, S.},
	doi = {10.1134/1.1410226},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/papers/Dzhioev\_JETP Letters\_74\_3\_(2001)\_Long Electron Spin Memory Times in GaAs.pdf:pdf},
	issn = {0021-3640},
	journal = {Journal of Experimental and Theoretical Physics Letters},
	month = aug,
	number = {3},
	pages = {182--185},
	title = {{Long electron spin memory times in gallium arsenide}},
	url = {http://link.springer.com/10.1134/1.1410226},
	volume = {74},
	year = {2001},
	Bdsk-Url-1 = {http://link.springer.com/10.1134/1.1410226},
	Bdsk-Url-2 = {http://dx.doi.org/10.1134/1.1410226}}

@mastersthesis{Dichtl2014,
	author = {Dichtl, Paul},
	school = {Technische Universit\"at M\"unchen},
	title = {Investigation of the coupling between "artificial semiconductor atoms" and metallic nanowires},
	type = {Bachelor's Thesis},
	year = {2013}}

@article{Ward2006,
	author = {Ward, B. W. and Notte, John a. and Economou, N. P.},
	doi = {10.1116/1.2357967},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/papers/Ward\_JVSTB\_24\_(2006)\_Helium ion microscope....pdf:pdf},
	issn = {10711023},
	journal = {Journal of Vacuum Science \& Technology B: Microelectronics and Nanometer Structures},
	number = {6},
	pages = {2871},
	title = {{Helium ion microscope: A new tool for nanoscale microscopy and metrology}},
	url = {http://scitation.aip.org/content/avs/journal/jvstb/24/6/10.1116/1.2357967},
	volume = {24},
	year = {2006},
	Bdsk-Url-1 = {http://scitation.aip.org/content/avs/journal/jvstb/24/6/10.1116/1.2357967},
	Bdsk-Url-2 = {http://dx.doi.org/10.1116/1.2357967}}

@article{Dionne2009,
	author = {Dionne, Jennifer A and Diest, Kenneth and Sweatlock, Luke A and Atwater, Harry A},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/papers/Dionne\_NL\_9\_2\_(2008)\_PlasMOStor.pdf:pdf},
	journal = {Nano letters},
	number = {2},
	pages = {897--902},
	title = {{PlasMOStor : A Metal - Oxide - Si Field Effect Plasmonic Modulator}},
	volume = {9},
	year = {2009}}

@article{Ritchie1957,
	author = {Ritchie, R.H.},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/papers/Ritchie\_PhysRev\_106\_5\_(1957)\_Plasma losses by Fast Electrons in Thin Films.pdf:pdf},
	journal = {Physical Review},
	number = {5},
	title = {{Plasma Losses by Fast Electrons in Thin Films}},
	volume = {106},
	year = {1957}}

@article{Ozbay2006,
	author = {Ozbay, Ekmel},
	file = {:C$\backslash$:/Users/sebastian.hammer/Downloads/Ozbay\_Science\_311\_(2006)\_Plasmonics Merging Photonics and Electronics at Nanoscale Dimensions.pdf:pdf},
	journal = {Science},
	number = {January},
	pages = {189--194},
	title = {{Plasmonics : Merging Photonics and}},
	volume = {311},
	year = {2006}}

@article{Sorger2012,
	author = {Sorger, Volker J. and Oulton, Rupert F. and Ma, Ren-Min and Zhang, Xiang},
	doi = {10.1557/mrs.2012.170},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/papers/Sorger\_Bulletin\_37\_(2012)\_Toward integrated plasmonic circuits.pdf:pdf},
	issn = {0883-7694},
	journal = {MRS Bulletin},
	month = aug,
	number = {08},
	pages = {728--738},
	title = {{Toward integrated plasmonic circuits}},
	url = {http://www.journals.cambridge.org/abstract\_S0883769412001704},
	volume = {37},
	year = {2012},
	Bdsk-Url-1 = {http://www.journals.cambridge.org/abstract%5C_S0883769412001704},
	Bdsk-Url-2 = {http://dx.doi.org/10.1557/mrs.2012.170}}

@article{Chang2007,
	author = {Chang, Darrick E. and S\o rensen, Anders S. and Demler, Eugene a. and Lukin, Mikhail D.},
	doi = {10.1038/nphys708},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/papers/Chang\_NaturePhys\_3\_(2007)\_A single-photon transistor using nanoscale surface plasmons.pdf:pdf},
	issn = {1745-2473},
	journal = {Nature Physics},
	month = aug,
	number = {11},
	pages = {807--812},
	title = {{A single-photon transistor using nanoscale surface plasmons}},
	url = {http://www.nature.com/doifinder/10.1038/nphys708},
	volume = {3},
	year = {2007},
	Bdsk-Url-1 = {http://www.nature.com/doifinder/10.1038/nphys708},
	Bdsk-Url-2 = {http://dx.doi.org/10.1038/nphys708}}

@article{Krasavin2004,
	author = {Krasavin, a. V. and Zheludev, N. I.},
	doi = {10.1063/1.1650904},
	file = {:/wsi/e24/Home/sebastian.hammer/My Documents/papers/Krasavin\_AIP\_84\_1416\_(2004)\_Active plasmonics....pdf:pdf},
	issn = {00036951},
	journal = {Applied Physics Letters},
	number = {8},
	pages = {1416},
	title = {{Active plasmonics: Controlling signals in Au/Ga waveguide using nanoscale structural transformations}},
	url = {http://scitation.aip.org/content/aip/journal/apl/84/8/10.1063/1.1650904},
	volume = {84},
	year = {2004},
	Bdsk-Url-1 = {http://scitation.aip.org/content/aip/journal/apl/84/8/10.1063/1.1650904},
	Bdsk-Url-2 = {http://dx.doi.org/10.1063/1.1650904}}

@article{Langford2004,
	abstract = {An in situ 'lift-out' technique for preparing transmission electron microscopy specimens, which is performed using secondary electron imaging within the chamber of a focused ion beam-SEM system is presented. The main advantage of this in situ approach, relative to the ex situ lift-out technique, is that secondary electron imaging enables higher magnifications to be used than is possible with optical microscopy. This makes the lift-out procedure more controllable and thus increases the overall success rate especially for inexperienced users. The technique is also compared with another in situ lift-out approach, the 'wedge' technique.},
	author = {Langford, R M and Clinton, C},
	doi = {10.1016/j.micron.2004.03.002},
	file = {:C$\backslash$:/Users/sebastian.hammer/Downloads/Langford\_micron\_35\_(2004)\_Iin situ lift-out using a FIB-SEMsystem.pdf:pdf},
	issn = {0968-4328},
	journal = {Micron (Oxford, England : 1993)},
	keywords = {a recent development to,electron beam,fib,focused ion beam,in situ lift-out,range of disciplines,sem,systems are versatile tools,tem cross-section,that are,the addition of an,these instruments has been,used in a wide},
	month = jan,
	number = {7},
	pages = {607--11},
	pmid = {15219907},
	title = {{In situ lift-out using a FIB-SEM system.}},
	url = {http://www.ncbi.nlm.nih.gov/pubmed/15219907},
	volume = {35},
	year = {2004},
	Bdsk-Url-1 = {http://www.ncbi.nlm.nih.gov/pubmed/15219907},
	Bdsk-Url-2 = {http://dx.doi.org/10.1016/j.micron.2004.03.002}}

@article{Wolffenbuttel1994,
	author = {Wohenbuttel, R F},
	file = {:C$\backslash$:/Users/sebastian.hammer/Downloads/Wolffenbuttel\_SaA\_43\_(1994)\_Low-temperature silicon wafer-to-wafer bonding using gold at eutectic temperatue.pdf:pdf},
	pages = {223--229},
	title = {{Low-temperature silicon wafer-to-wafer bonding using gold at eutectic temperature}},
	volume = {43},
	year = {1994}}

@online{Intel14,
	author = {Intel},
	month = {Online; accessed 18-December-2014},
	title = {Intel's Newest Microarchitecture and 14nm Manufacturing Process},
	url = {http://newsroom.intel.com/docs/DOC-5677},
	year = {2014},
	Bdsk-Url-1 = {http://newsroom.intel.com/docs/DOC-5677}}

@article{Svo16,
	author = {Svore, Krysta M and Troyer, Matthias},
	date-modified = {2022-03-17 12:11:30 +0100},
	journal = {Computer},
	keywords = {Quantum computation},
	number = {9},
	pages = {21--30},
	publisher = {IEEE},
	title = {The quantum future of computation},
	volume = {49},
	year = {2016}}

@misc{Nie02,
	author = {Nielsen, Michael A and Chuang, Isaac},
	date-modified = {2022-03-17 12:12:48 +0100},
	keywords = {Quantum encryption},
	publisher = {American Association of Physics Teachers},
	title = {Quantum computation and quantum information},
	year = {2002}}

@article{Zic19,
	title={Optimizing the stoichiometry of ultrathin NbTiN films for high-performance superconducting nanowire single-photon detectors},
	author={Zichi, Julien and Chang, Jin and Steinhauer, Stephan and Von Fieandt, Kristina and Los, Johannes WN and Visser, Gijs and Kalhor, Nima and Lettner, Thomas and Elshaari, Ali W and Zadeh, Iman Esmaeil and others},
	journal={Optics express},
	volume={27},
	number={19},
	pages={26579--26587},
	year={2019},
	publisher={Optical Society of America}
}
